A multivariate statistical analysis of spiral galaxy luminosities. I. Data and results

We have performed a multiparametric analysis of luminosity data for a sample of 234 normal spiral and irregular galaxies observed in X-rays with the {\it Einstein Observatory}. This sample is representative of S and Irr galaxies, with a good coverage of morphological types and absolute magnitudes. In addition to X-ray and optical da ta, we have compiled H-band magnitudes, IRAS near- and far-infrared, and 6cm radio co ntinuum observations for the sample from the literature. We have also performed a carefu l compilation of distance estimates. We have explored the effect of morphology by dividing the sample into early (S0/a-Sab), intermediate (Sb-Sbc), and late-type (Sc-Irr) subsamples. The data were analysed with bivariate and multiv ariate survival analysis techniques that make full use of all the information available in both detections and limits.

==> amorph_table11b.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{llrrr|llrrr}
\small
\tablenum{11B}
\tablewidth{0pc}
\tablecaption{Spearman Partial Rank Analysis on the $T = 0 - 2$ Sample ($N = 23$) (No amorphous galaxies)}
\tablehead{
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  &
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  &
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  \\
}
\startdata

 B , X &  D  &0.423 & 2.085 &0.025  & 6cm, X &  D  &0.228 & 1.046 &0.167 \nl
  &  6cm, D  &0.368 & 1.726 &0.050   &   &   H , D  &0.181 & 0.801 &0.224 \nl 
  &   H , D  &0.143 & 0.631 &0.268   &   &   B , D  & 0.047 & 0.204 & $>$ 0.400 \nl 
  &  FIR, D  &0.445 & 2.165 &0.023   &   &  FIR, D  &0.308 & 1.411 &0.090 \nl 
  &   12, D  &0.397 & 1.887 &0.039   &   &   12, D  &0.172 & 0.761 &0.233 \nl 
  &  6cm, H , D  & 0.056 & 0.240 & $>$ 0.400   &   &   H , B , D  & 0.125 & 0.533 & 0.299 \nl 
  &  6cm,FIR, D  & 0.390 & 1.798 & 0.045   &   &   H ,FIR, D  & 0.263 & 1.158 & 0.140 \nl 
  &  6cm, 12, D  & 0.372 & 1.702 & 0.053   &   &   H , 12, D  & 0.126 & 0.537 & 0.298 \nl 
  &   H ,FIR, D  & 0.167 & 0.718 & 0.243   &   &   B ,FIR, D  & 0.208 & 0.903 & 0.200 \nl 
  &   H , 12, D  & 0.087 & 0.371 & 0.359   &   &   B , 12, D  & 0.087 & 0.370 & 0.359 \nl 
  &  FIR, 12, D  & 0.418 & 1.950 & 0.035   &   &  FIR, 12, D  & 0.195 & 0.845 & 0.214 \nl 
  &  6cm, H ,FIR, D  & 0.104 & 0.430 & 0.337   &   &   H , B ,FIR, D  & 0.230 & 0.975 & 0.183 \nl 
  &  6cm, H , 12, D  & 0.062 & 0.255 & $>$ 0.400   &   &   H , B , 12, D  & 0.110 & 0.455 & 0.328 \nl 
  &  6cm,FIR, 12, D  & 0.390 & 1.745 & 0.050   &   &   H ,FIR, 12, D  & 0.150 & 0.624 & 0.271 \nl 
  &   H ,FIR, 12, D  & 0.125 & 0.519 & 0.304   &   &   B ,FIR, 12, D  & 0.109 & 0.453 & 0.328 \nl 
 H , X &  D  &0.439 & 2.186 &0.022  &  H , B &  D & 0.779& 5.548 & $<$ 0.005 \nl
  &  6cm, D  &0.420 & 2.018 &0.030   &   &  6cm, D  & 0.804 & 5.894 & $<$ 0.005 \nl 
  &   B , D  &0.193 & 0.860 &0.210   &   &   X , D  & 0.728 & 4.632 & $<$ 0.005 \nl 
  &  FIR, D  &0.439 & 2.128 &0.024   &   &  FIR, D  & 0.817 & 6.174 & $<$ 0.005 \nl 
  &   12, D  &0.432 & 2.089 &0.025   &   &   12, D  & 0.813 & 6.091 & $<$ 0.005 \nl 
  &  6cm, B , D  & 0.224 & 0.977 & 0.183   &   &  6cm, X , D  & 0.770 & 5.114 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.412 & 1.918 & 0.037   &   &  6cm,FIR, D  & 0.814 & 5.944 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.419 & 1.956 & 0.035   &   &  6cm, 12, D  & 0.811 & 5.885 & $<$ 0.005 \nl 
  &   B ,FIR, D  & 0.146 & 0.625 & 0.270   &   &   X ,FIR, D  & 0.773 & 5.162 & $<$ 0.005 \nl 
  &   B , 12, D  & 0.204 & 0.886 & 0.204   &   &   X , 12, D  & 0.775 & 5.206 & $<$ 0.005 \nl 
  &  FIR, 12, D  & 0.432 & 2.030 & 0.030   &   &  FIR, 12, D  & 0.817 & 6.006 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & 0.176 & 0.739 & 0.239   &   &  6cm, X ,FIR, D  & 0.779 & 5.115 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & 0.215 & 0.907 & 0.199   &   &  6cm, X , 12, D  & 0.777 & 5.097 & $<$ 0.005 \nl 
  &  6cm,FIR, 12, D  & 0.416 & 1.886 & 0.040   &   &  6cm,FIR, 12, D  & 0.814 & 5.782 & $<$ 0.005 \nl 
  &   B ,FIR, 12, D  & 0.173 & 0.724 & 0.242   &   &   X ,FIR, 12, D  & 0.777 & 5.082 & $<$ 0.005 \nl 
 X , 12&  D  &0.158 & 0.714 &0.244  &  B , 12&  D  &0.397 & 1.933 &0.036 \nl
  &  6cm, D  & -0.045 & -0.195 & $>$ 0.400   &   &  6cm, D  &0.066 & 0.288 &0.390 \nl 
  &   H , D  &0.133 & 0.584 &0.283   &   &   H , D  &0.525 & 2.687 &0.008 \nl 
  &   B , D  & -0.012 & -0.053 & $>$ 0.400   &   &   X , D  &0.369 & 1.730 &0.050 \nl 
  &  FIR, D  &0.288 & 1.313 &0.104   &   &  FIR, D  &0.178 & 0.788 &0.227 \nl 
  &  6cm, H , D  & -0.022 & -0.092 & $>$ 0.400   &   &  6cm, H , D  & 0.192 & 0.828 & 0.218 \nl 
  &  6cm, B , D  & -0.074 & -0.316 & 0.379   &   &  6cm, X , D  & 0.089 & 0.377 & 0.357 \nl 
  &  6cm,FIR, D  & 0.161 & 0.690 & 0.250   &   &  6cm,FIR, D  & 0.036 & 0.152 & $>$ 0.400 \nl 
  &   H , B , D  & 0.068 & 0.291 & 0.389   &   &   H , X , D  & 0.516 & 2.553 & 0.010 \nl 
  &   H ,FIR, D  & 0.276 & 1.219 & 0.126   &   &   H ,FIR, D  & 0.176 & 0.759 & 0.234 \nl 
  &   B ,FIR, D  & 0.237 & 1.037 & 0.169   &   &   X ,FIR, D  & 0.058 & 0.246 & $>$ 0.400 \nl 
  &  6cm, H , B , D  & -0.033 & -0.137 & $>$ 0.400   &   &  6cm, H , X , D  & 0.193 & 0.812 & 0.221 \nl 
  &  6cm, H ,FIR, D  & 0.172 & 0.722 & 0.243   &   &  6cm, H ,FIR, D  & 0.050 & 0.206 & $>$ 0.400 \nl 
  &  6cm, B ,FIR, D  & 0.159 & 0.665 & 0.258   &   &  6cm, X ,FIR, D  & -0.030 & -0.122 & $>$ 0.400 \nl 
  &   H , B ,FIR, D  & 0.254 & 1.084 & 0.158   &   &   H , X ,FIR, D  & 0.137 & 0.571 & 0.287 \nl 
 X ,FIR&  D & 0.022& 0.099 & $>$ 0.400  &  B ,FIR&  D  &0.362 & 1.734 &0.049 \nl
  &  6cm, D  &-0.214 & -0.955 &0.188   &   &  6cm, D  & 0.057 & 0.249 & $>$ 0.400 \nl 
  &   H , D  & 0.001 & 0.003 & $>$ 0.400   &   &   H , D  &0.515 & 2.622 &0.009 \nl 
  &   B , D  &-0.155 & -0.682 &0.253   &   &   X , D  &0.389 & 1.839 &0.042 \nl 
  &   12, D  &-0.245 & -1.104 &0.153   &   &   12, D  & 0.030 & 0.131 & $>$ 0.400 \nl 
  &  6cm, H , D  & -0.195 & -0.842 & 0.214   &   &  6cm, H , D  & 0.220 & 0.956 & 0.188 \nl 
  &  6cm, B , D  & -0.253 & -1.111 & 0.151   &   &  6cm, X , D  & 0.150 & 0.642 & 0.265 \nl 
  &  6cm, 12, D  & -0.262 & -1.151 & 0.142   &   &  6cm, 12, D  & 0.014 & 0.060 & $>$ 0.400 \nl 
  &   H , B , D  & -0.086 & -0.368 & 0.360   &   &   H , X , D  & 0.521 & 2.588 & 0.009 \nl 
  &   H , 12, D  & -0.244 & -1.069 & 0.161   &   &   H , 12, D  & 0.134 & 0.575 & 0.286 \nl 
  &   B , 12, D  & -0.281 & -1.240 & 0.121   &   &   X , 12, D  & 0.143 & 0.615 & 0.273 \nl 
  &  6cm, H , B , D  & -0.213 & -0.897 & 0.202   &   &  6cm, H , X , D  & 0.236 & 1.000 & 0.177 \nl 
  &  6cm, H , 12, D  & -0.257 & -1.096 & 0.155   &   &  6cm, H , 12, D  & 0.121 & 0.501 & 0.311 \nl 
  &  6cm, B , 12, D  & -0.288 & -1.239 & 0.121   &   &  6cm, X , 12, D  & 0.125 & 0.518 & 0.305 \nl 
  &   H , B , 12, D  & -0.259 & -1.107 & 0.152   &   &   H , X , 12, D  & 0.161 & 0.673 & 0.255 \nl 
\tablebreak 
6cm, B &  D  &0.449 & 2.249 &0.020  & FIR, 12&  D & 0.878& 8.191 & $<$ 0.005 \nl
  &   H , D  &0.533 & 2.742 &0.007   &   &  6cm, D  & 0.718 & 4.500 & $<$ 0.005 \nl 
  &   X , D  &0.400 & 1.903 &0.038   &   &   H , D  & 0.878 & 7.989 & $<$ 0.005 \nl 
  &  FIR, D  &0.291 & 1.328 &0.101   &   &   B , D  & 0.858 & 7.280 & $<$ 0.005 \nl 
  &   12, D  &0.238 & 1.070 &0.161   &   &   X , D  & 0.885 & 8.307 & $<$ 0.005 \nl 
  &   H , X , D  & 0.520 & 2.586 & 0.009   &   &  6cm, H , D  & 0.717 & 4.365 & $<$ 0.005 \nl 
  &   H ,FIR, D  & 0.267 & 1.178 & 0.136   &   &  6cm, B , D  & 0.717 & 4.367 & $<$ 0.005 \nl 
  &   H , 12, D  & 0.218 & 0.948 & 0.189   &   &  6cm, X , D  & 0.726 & 4.482 & $<$ 0.005 \nl 
  &   X ,FIR, D  & 0.181 & 0.782 & 0.229   &   &   H , B , D  & 0.833 & 6.378 & $<$ 0.005 \nl 
  &   X , 12, D  & 0.188 & 0.813 & 0.221   &   &   H , X , D  & 0.886 & 8.090 & $<$ 0.005 \nl 
  &  FIR, 12, D  & 0.237 & 1.035 & 0.169   &   &   B , X , D  & 0.867 & 7.367 & $<$ 0.005 \nl 
  &   H , X ,FIR, D  & 0.235 & 0.997 & 0.178   &   &  6cm, H , B , D  & 0.705 & 4.098 & $<$ 0.005 \nl 
  &   H , X , 12, D  & 0.210 & 0.884 & 0.204   &   &  6cm, H , X , D  & 0.727 & 4.364 & $<$ 0.005 \nl 
  &   H ,FIR, 12, D  & 0.210 & 0.887 & 0.204   &   &  6cm, B , X , D  & 0.724 & 4.327 & $<$ 0.005 \nl 
  &   X ,FIR, 12, D  & 0.174 & 0.730 & 0.241   &   &   H , B , X , D  & 0.844 & 6.479 & $<$ 0.005 \nl 
 H , 12&  D  &0.088 & 0.397 &0.349  & 6cm, 12&  D & 0.806& 6.079 & $<$ 0.005 \nl
  &  6cm, D  &-0.060 & -0.260 &0.400   &   &   H , D  & 0.805 & 5.906 & $<$ 0.005 \nl 
  &   B , D  &-0.383 & -1.807 &0.045   &   &   B , D  & 0.765 & 5.176 & $<$ 0.005 \nl 
  &   X , D  & 0.022 & 0.094 & $>$ 0.400   &   &   X , D  & 0.800 & 5.820 & $<$ 0.005 \nl 
  &  FIR, D  &0.094 & 0.412 &0.344   &   &  FIR, D  &0.510 & 2.582 &0.009 \nl 
  &  6cm, B , D  & -0.190 & -0.819 & 0.220   &   &   H , B , D  & 0.729 & 4.516 & $<$ 0.005 \nl 
  &  6cm, X , D  & -0.045 & -0.191 & $>$ 0.400   &   &   H , X , D  & 0.801 & 5.672 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.008 & 0.035 & $>$ 0.400   &   &   H ,FIR, D  & 0.503 & 2.470 & 0.013 \nl 
  &   B , X , D  & -0.388 & -1.786 & 0.046   &   &   B , X , D  & 0.766 & 5.061 & $<$ 0.005 \nl 
  &   B ,FIR, D  & -0.090 & -0.386 & 0.354   &   &   B ,FIR, D  & 0.486 & 2.361 & 0.016 \nl 
  &   X ,FIR, D  & -0.038 & -0.160 & $>$ 0.400   &   &   X ,FIR, D  & 0.462 & 2.210 & 0.021 \nl 
  &  6cm, B , X , D  & -0.178 & -0.746 & 0.237   &   &   H , B , X , D  & 0.728 & 4.374 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & -0.036 & -0.148 & $>$ 0.400   &   &   H , B ,FIR, D  & 0.481 & 2.261 & 0.020 \nl 
  &  6cm, X ,FIR, D  & -0.064 & -0.266 & 0.398   &   &   H , X ,FIR, D  & 0.464 & 2.161 & 0.023 \nl 
  &   B , X ,FIR, D  & -0.130 & -0.541 & 0.296   &   &   B , X ,FIR, D  & 0.460 & 2.135 & 0.024 \nl 
 H ,FIR&  D & 0.049& 0.221 & $>$ 0.400  & 6cm,FIR&  D & 0.727& 4.729 & $<$ 0.005 \nl
  &  6cm, D  &-0.091 & -0.398 &0.349   &   &   H , D  & 0.728 & 4.635 & $<$ 0.005 \nl 
  &   B , D  &-0.397 & -1.884 &0.039   &   &   B , D  & 0.677 & 4.013 & $<$ 0.005 \nl 
  &   X , D  & 0.044 & 0.193 & $>$ 0.400   &   &   X , D  & 0.741 & 4.813 & $<$ 0.005 \nl 
  &   12, D  & -0.059 & -0.257 & $>$ 0.400   &   &   12, D  &0.069 & 0.301 &0.385 \nl 
  &  6cm, B , D  & -0.231 & -1.005 & 0.176   &   &   H , B , D  & 0.626 & 3.405 & $<$ 0.005 \nl 
  &  6cm, X , D  & -0.001 & -0.005 & $>$ 0.400   &   &   H , X , D  & 0.741 & 4.676 & $<$ 0.005 \nl 
  &  6cm, 12, D  & -0.069 & -0.295 & 0.387   &   &   H , 12, D  & 0.078 & 0.332 & 0.373 \nl 
  &   B , X , D  & -0.378 & -1.734 & 0.050   &   &   B , X , D  & 0.694 & 4.085 & $<$ 0.005 \nl 
  &   B , 12, D  & -0.143 & -0.615 & 0.273   &   &   B , 12, D  & 0.064 & 0.271 & 0.396 \nl 
  &   X , 12, D  & 0.054 & 0.229 & $>$ 0.400   &   &   X , 12, D  & 0.116 & 0.497 & 0.312 \nl 
  &  6cm, B , X , D  & -0.184 & -0.773 & 0.231   &   &   H , B , X , D  & 0.644 & 3.472 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & -0.138 & -0.575 & 0.286   &   &   H , B , 12, D  & 0.050 & 0.208 & $>$ 0.400 \nl 
  &  6cm, X , 12, D  & 0.046 & 0.190 & $>$ 0.400   &   &   H , X , 12, D  & 0.113 & 0.469 & 0.323 \nl 
  &   B , X , 12, D  & -0.092 & -0.379 & 0.356   &   &   B , X , 12, D  & 0.092 & 0.381 & 0.355 \nl 
6cm, H &  D  &0.153 & 0.692 &0.249  & & & & & \nl
  &   B , D  &-0.351 & -1.635 &0.062   & & & & & \nl
  &   X , D  &0.061 & 0.265 &0.398   & & & & & \nl
  &  FIR, D  &0.171 & 0.755 &0.235   & & & & & \nl
  &   12, D  &0.139 & 0.610 &0.275   & & & & & \nl
  &   B , X , D  & -0.368 & -1.677 & 0.057   & & & & & \nl
  &   B ,FIR, D  & -0.122 & -0.522 & 0.303   & & & & & \nl
  &   B , 12, D  & -0.098 & -0.417 & 0.342   & & & & & \nl
  &   X ,FIR, D  & 0.042 & 0.176 & $>$ 0.400   & & & & & \nl
  &   X , 12, D  & 0.072 & 0.307 & 0.382   & & & & & \nl
  &  FIR, 12, D  & 0.143 & 0.614 & 0.274   & & & & & \nl
  &   B , X ,FIR, D  & -0.158 & -0.658 & 0.260   & & & & & \nl
  &   B , X , 12, D  & -0.119 & -0.492 & 0.314   & & & & & \nl
  &   B ,FIR, 12, D  & -0.090 & -0.372 & 0.359   & & & & & \nl
  &   X ,FIR, 12, D  & 0.067 & 0.275 & 0.394   & & & & & \nl
\enddata
\end{deluxetable}


==> amorph_table5.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{lrrrrrrrr}
\small
\tablenum{5}
\tablewidth{0pc}
\tablecaption{Correlation Tests (No amorphous galaxies)}
\tablehead{
\colhead{} &
\multicolumn{2}{c}{Total} & 
\multicolumn{2}{c}{$T = 0 - 2$} & 
\multicolumn{2}{c}{$T = 3 - 4$} & 
\multicolumn{2}{c}{$T = 5 - 10$}  \\
\colhead{Test Pair}& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}} \\ }
\startdata


$L_X$-$L_B$ & 234 & 120,0,0 &  58 & 32,0,0 &  61 & 28,0,0 &  108 & 56,0,0  \nl
& 9.75125 & 0.000000 &  4.97458 & 0.000001 &  4.29697 & 0.000017 &  6.43196 & 0.000000  \nl
& 0.63156 & 0.000000 &  0.64656 & 0.000001 &  0.55666 & 0.000016 &  0.58926 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_X$-$L_H$ & 140 & 53,0,0 &  32 & 11,0,0 &  41 & 14,0,0 &  62 & 25,0,0  \nl
& 7.05771 & 0.000000 &  2.39037 & 0.016831 &  3.29027 & 0.001001 &  4.62693 & 0.000004  \nl
& 0.59595 & 0.000000 &  0.45075 & 0.012085 &  0.49023 & 0.001932 &  0.56567 & 0.000010  \nl
&  &  &   &  &   &  &   &   \nl
$L_X$-$L_{12}$& 218 & 44,33,64 &  51 & 12,8,15 &  58 & 13,9,13 &  102 & 17,16,34  \nl
& 9.33129 & 0.000000 &  3.02355 & 0.002498 &  5.34773 & 0.000000 &  6.79409 & 0.000000  \nl
& 0.56422 & 0.000000 &  0.34145 & 0.015760 &  0.62435 & 0.000002 &  0.58729 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_X$-$L_{FIR}$& 218 & 101,2,7 &  51 & 20,2,7 &  58 & 26,0,0 &  102 & 51,0,0  \nl
& 9.25571 & 0.000000 &  2.53401 & 0.011276 &  5.41846 & 0.000000 &  7.47039 & 0.000000  \nl
& 0.59641 & 0.000000 &  0.34655 & 0.014265 &  0.71233 & 0.000000 &  0.67932 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_X$-$L_{6cm}$& 136 & 34,8,25 &  38 & 7,6,12 &  36 & 8,0,3 &  57 & 18,2,9  \nl
& 8.23522 & 0.000000 &  2.78807 & 0.005302 &  4.32718 & 0.000015 &  6.26258 & 0.000000  \nl
& 0.59459 & 0.000000 &  0.37041 & 0.024252 &  0.66916 & 0.000075 &  0.64251 & 0.000002  \nl
&  &  &   &  &   &  &   &   \nl
$L_B$-$L_H$ & 140 & 0,0,0 &  32 & 0,0,0 &  41 & 0,0,0 &  62 & 0,0,0  \nl
& 12.55309 & 0.000000 &  5.74062 & 0.000000 &  7.39062 & 0.000000 &  9.03216 & 0.000000  \nl
& 0.88156 & 0.000000 &  0.86950 & 0.000001 &  0.94216 & 0.000000 &  0.93020 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_B$-$L_{12}$ & 218 & 0,97,0 &  51 & 0,23,0 &  58 & 0,22,0 &  102 & 0,50,0  \nl
& 10.14752 & 0.000000 &  3.80753 & 0.000140 &  4.15996 & 0.000032 &  8.31032 & 0.000000  \nl
& 0.62615 & 0.000000 &  0.50178 & 0.000388 &  0.49103 & 0.000210 &  0.71452 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_B$-$L_{FIR}$ & 218 & 0,9,0 &  51 & 0,9,0 &  58 & 0,0,0 &  102 & 0,0,0  \nl
& 11.43934 & 0.000000 &  3.63036 & 0.000283 &  4.63522 & 0.000004 &  10.38866 & 0.000000  \nl
& 0.70124 & 0.000000 &  0.49978 & 0.000409 &  0.59808 & 0.000006 &  0.87139 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_B$-$L_{6cm}$ & 136 & 0,33,0 &  38 & 0,18,0 &  36 & 0,3,0 &  57 & 0,11,0  \nl
& 7.35568 & 0.000000 &  3.54014 & 0.000400 &  2.54202 & 0.011021 &  5.30613 & 0.000000  \nl
& 0.61265 & 0.000000 &  0.60167 & 0.000252 &  0.43516 & 0.010040 &  0.64744 & 0.000001  \nl
&  &  &   &  &   &  &   &   \nl
$L_H$-$L_{12}$ & 135 & 0,41,0 &  30 & 0,9,0 &  41 & 0,11,0 &  59 & 0,20,0  \nl
& 6.61906 & 0.000000 &  0.85766 & 0.391081 &  3.76223 & 0.000168 &  6.95073 & 0.000000  \nl
& 0.56200 & 0.000000 &  0.17853 & 0.336336 &  0.58141 & 0.000236 &  0.81725 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_H$-$L_{FIR}$ & 135 & 0,4,0 &  30 & 0,4,0 &  41 & 0,0,0 &  59 & 0,0,0  \nl
& 6.17389 & 0.000000 &  0.77468 & 0.438528 &  3.81886 & 0.000134 &  7.42232 & 0.000000  \nl
& 0.49702 & 0.000000 &  0.14314 & 0.440811 &  0.58328 & 0.000225 &  0.82636 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_H$-$L_{6cm}$ & 97 & 0,17,0 &  24 & 0,7,0 &  29 & 0,2,0 &  40 & 0,7,0  \nl
& 4.13407 & 0.000036 &  1.44578 & 0.148239 &  1.66752 & 0.095411 &  3.86312 & 0.000112  \nl
& 0.41224 & 0.000054 &  0.33915 & 0.103842 &  0.31874 & 0.091681 &  0.56935 & 0.000377  \nl
&  &  &   &  &   &  &   &   \nl
$L_{12}$-$L_{FIR}$& 218 & 89,1,8 &  51 & 15,1,8 &  58 & 22,0,0 &  102 & 50,0,0  \nl
& 14.70804 & 0.000000 &  6.98218 & 0.000000 &  7.47427 & 0.000000 &  10.00862 & 0.000000  \nl
& 0.83149 & 0.000000 &  0.87383 & 0.000000 &  0.83006 & 0.000000 &  0.82432 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
$L_{12}$-$L_{6cm}$& 125 & 15,11,17 &  32 & 2,6,9 &  35 & 3,1,2 &  53 & 10,3,6  \nl
& 10.39708 & 0.000000 &  5.64062 & 0.000000 &  5.82150 & 0.000000 &  5.82509 & 0.000000  \nl
& 0.77305 & 0.000000 &  0.84709 & 0.000002 &  0.82883 & 0.000001 &  0.64624 & 0.000003  \nl
&  &  &   &  &   &  &   &   \nl
$L_{FIR}$-$L_{6cm}$& 125 & 1,24,4 &  32 & 1,11,4 &  35 & 0,3,0 &  53 & 0,9,0  \nl
& 11.41265 & 0.000000 &  4.74208 & 0.000002 &  5.66011 & 0.000000 &  7.45396 & 0.000000  \nl
& 0.85204 & 0.000000 &  0.78785 & 0.000012 &  0.81729 & 0.000002 &  0.82862 & 0.000000  \nl
&  &  &   &  &   &  &   &   \nl
\tablenotetext{a}{
The values in rows 2 and 3 of each group in these columns are 
the test statistic for the Kendall's $\tau$ correlation test, 
and the Spearman's rank correlation coefficient, respectively.
} 
\tablenotetext{b}{
The three values for $N_{lim}$ in the first row of each group 
in these columns are respectively 
the number of limit points in the left-hand luminosity, 
the number in the right-hand luminosity, and the number of double limits. 
The numbers listed in rows 2 and 3 of each group are the 
probablities that the two luminosities are uncorrelated.
}
\enddata
\end{deluxetable}


==> amorph_table6.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{lrrrrrrrr}
\tablenum{6}
\tablewidth{0pc}
\tablecaption{Correlation Tests Between $L_X/L_B$ and Other Luminosity Ratios (No amorphous galaxies)}
\tablehead{
\colhead{} &
\multicolumn{2}{c}{Total} & 
\multicolumn{2}{c}{$T = 0 - 2$} & 
\multicolumn{2}{c}{$T = 3 - 4$} & 
\multicolumn{2}{c}{$T = 5 - 10$}  \\
\colhead{Ratio}& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}}
& \colhead{$N_{tot}$\tablenotemark{a}} & \colhead{$N_{lim}$\tablenotemark{b}} \\}
\startdata


$L_{60}/L_B$
& 217 & 2,100,7  & 51 & 2,20,7  & 57 & 0,25,0  & 102 & 0,51,0  \nl
& 4.91099 & 0.000001  & 0.01669 & 0.986687  & 4.19187 & 0.000028  & 4.18877 & 0.000028  \nl
& 0.32989 & 0.000001  & -0.00197 & 0.988912  & 0.57721 & 0.000016  & 0.42647 & 0.000018  \nl
&  &   &  &   &  &   &  &   \nl
    
&  &   &  &   &  &   &  &   \nl
    
    
$L_{6cm}/L_B$
& 136 & 8,34,25  & 38 & 6,7,12  & 36 & 0,8,3  & 57 & 2,18,9  \nl
& 5.66497 & 0.000000  & 0.61730 & 0.537040  & 3.64839 & 0.000264  & 5.00346 & 0.000000  \nl
& 0.41897 & 0.000001  & 0.03927 & 0.811206  & 0.61129 & 0.000299  & 0.57013 & 0.000020  \nl
&  &   &  &   &  &   &  &   \nl
    
&  &   &  &   &  &   &  &   \nl
    
    
$L_{12}/L_B$
& 218 & 33,44,64  & 51 & 8,12,15  & 58 & 9,13,13  & 102 & 16,17,34  \nl
& 4.73124 & 0.000002  & 0.67962 & 0.496746  & 3.68214 & 0.000231  & 3.29762 & 0.000975  \nl
& 0.29226 & 0.000017  & 0.06183 & 0.661981  & 0.45932 & 0.000525  & 0.31743 & 0.001422  \nl
&  &   &  &   &  &   &  &   \nl
    
&  &   &  &   &  &   &  &   \nl
    
    
$L_{60}/L_{100}$
& 212 & 1,100,3  & 46 & 1,20,3  & 58 & 0,26,0  & 101 & 0,50,0  \nl
& 4.76055 & 0.000002  & 1.33388 & 0.182243  & 3.99922 & 0.000064  & 2.99848 & 0.002713  \nl
& 0.30122 & 0.000012  & 0.16779 & 0.260355  & 0.52355 & 0.000077  & 0.27794 & 0.005446  \nl
&  &   &  &   &  &   &  &   \nl
    
&  &   &  &   &  &   &  &   \nl
    
    
$L_{H}/L_B$
& 140 & 0,53,0  & 32 & 0,11,0  & 41 & 0,14,0  & 62 & 0,25,0  \nl
& 1.80598 & 0.070921  & 0.48752 & 0.625893  & 0.38805 & 0.697983  & 0.90487 & 0.365536  \nl
& 0.17401 & 0.040214  & -0.05096 & 0.776608  & -0.03619 & 0.818938  & 0.14835 & 0.246597  \nl
&  &   &  &   &  &   &  &   \nl
    
&  &   &  &   &  &   &  &   \nl
    
    
\tablenotetext{a}{
The values in rows 2 and 3 of each group in these columns are 
the test statistic for the Kendall's $\tau$ correlation test, 
and the Spearman's rank correlation coefficient, respectively.
} 
\tablenotetext{b}{
The three values for $N_{lim}$ in the first row of each group 
in these columns are respectively 
the number of limit points in the luminosity ratio paired with $L_X/L_B$, 
the number in $L_X/L_B$, and the number of double limits. 
The numbers listed in rows 2 and 3 of each group are the 
probablities that the two variables are uncorrelated.
}
\enddata
\end{deluxetable}


==> amorph_table7.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{ccrrrrrrrrrrrr}
\small
\tablenum{7}
\tablewidth{0pc}
\tablecaption{Schmitt's Method Regression Bisectors (No amorphous galaxies) }
\tablehead{
\colhead{} & \colhead{} &
\multicolumn{3}{c}{Total} & 
\multicolumn{3}{c}{$T = 0 - 2$} & 
\multicolumn{3}{c}{$T = 3 - 4$} & 
\multicolumn{3}{c}{$T = 5 - 10$}  \\
\colhead{X} & \colhead{Y} &
\colhead{Slope} & \colhead{$\sigma_{Slope}$} & \colhead{Int.}  & 
\colhead{Slope} & \colhead{$\sigma_{Slope}$} & \colhead{Int.}  & 
\colhead{Slope} & \colhead{$\sigma_{Slope}$} & \colhead{Int.}  & 
\colhead{Slope} & \colhead{$\sigma_{Slope}$} & \colhead{Int.}  \\
 }

\startdata



$L_B$ & $L_X$ &   1.50 &   0.10 & -24.34 &    1.45 &   0.15 & -22.03 &    1.53 &   0.17 & -26.03 &    1.48 &   0.13 & -23.61 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_H$ & $L_X$ &   1.17 &   0.08 & -10.67 &    1.41 &   0.47 & -21.38 &    1.10 &   0.22 &  -7.87 &    1.20 &   0.13 & -12.03 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{12}$ & $L_X$ &   0.74 &   0.07 &   8.53 &    1.22 &   0.16 & -11.64 &    1.07 &   0.09 &  -5.17 &    0.66 &   0.06 &  12.26 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{FIR}$ & $L_X$ &   1.00 &   0.06 &  -3.16 &    0.84 &   0.14 &   4.18 &    1.10 &   0.10 &  -7.51 &    0.96 &   0.06 &  -1.60 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{6cm}$ & $L_X$ &   0.90 &   0.07 &   7.77 &    0.65 &   0.13 &  17.19 &    0.96 &   0.12 &   5.75 &    0.90 &   0.07 &   7.70 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_H$ & $L_B$ &   0.73 &   0.03 &  11.46 &    1.00 &   0.11 &  -0.49 &    0.83 &   0.06 &   6.78 &    0.73 &   0.04 &  11.34 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{12}$ & $L_B$ &   0.49 &   0.04 &  22.51 &    0.75 &   0.09 &  11.27 &    0.76 &   0.09 &  10.92 &    0.45 &   0.04 &  23.99 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{FIR}$ & $L_B$ &   0.65 &   0.04 &  14.95 &    0.64 &   0.13 &  15.61 &    0.78 &   0.14 &   9.36 &    0.66 &   0.04 &  14.34 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{6cm}$ & $L_B$ &   0.53 &   0.05 &  24.18 &    0.50 &   0.12 &  25.27 &    0.65 &   0.16 &  19.74 &    0.62 &   0.07 &  20.64 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{12}$ & $L_H$ &   0.67 &   0.06 &  15.02 &    0.82 &   0.28 &   9.04 &    0.84 &   0.12 &   7.91 &    0.60 &   0.05 &  17.89 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_H$ & $L_{FIR}$ &   1.16 &   0.13 &  -7.24 &    1.30 &   0.66 & -14.01 &    1.20 &   0.24 &  -8.77 &    1.19 &   0.09 &  -7.99 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_H$ & $L_{6cm}$ &   1.38 &   0.21 & -24.17 &    2.32 &   1.03 & -66.37 &    1.43 &   0.56 & -26.54 &    1.25 &   0.23 & -18.27 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{12}$ & $L_{FIR}$ &   0.76 &   0.04 &  10.95 &    1.23 &   0.12 &  -9.23 &    0.98 &   0.07 &   1.84 &    0.74 &   0.03 &  11.99 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{12}$ & $L_{6cm}$ &   0.99 &   0.07 &  -6.08 &    1.79 &   0.21 & -40.60 &    1.15 &   0.12 & -13.03 &    0.88 &   0.07 &  -1.37 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
$L_{6cm}$ & $L_{FIR}$ &   0.82 &   0.05 &  14.16 &    0.72 &   0.13 &  17.30 &    0.92 &   0.09 &  10.56 &    0.91 &   0.06 &  10.67 \nl
  &  &  &  &  &   &  &  &   &  &  &   &  &  \nl
  
\enddata
\end{deluxetable}


==> amorph_table8.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\ptlandscape
\begin{deluxetable}{llrrrrrrrrrrrr}
\small
\tablenum{8}
\tablewidth{0pc}
\tablecaption{Spearman Partial Rank Analysis}
\tablehead{
\colhead{} & \colhead{} &
\multicolumn{3}{c}{Total ($N = 94$)} & 
\multicolumn{3}{c}{$T = 0 - 2$ ($N = 23$)} & 
\multicolumn{3}{c}{$T = 3 - 4$ ($N = 29$)} & 
\multicolumn{3}{c}{$T = 5 - 10$ ($N = 38$)}  \\
\colhead{Test} & \colhead{Held } &
\multicolumn{1}{c}{Partial } & \multicolumn{1}{c}{Test Stat.} & \multicolumn{1}{c}{Prob.}  &
\multicolumn{1}{c}{Partial } & \multicolumn{1}{c}{Test Stat.} & \multicolumn{1}{c}{Prob.}  &
\multicolumn{1}{c}{Partial } & \multicolumn{1}{c}{Test Stat.} & \multicolumn{1}{c}{Prob.}  &
\multicolumn{1}{c}{Partial } & \multicolumn{1}{c}{Test Stat.} & \multicolumn{1}{c}{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\multicolumn{1}{c}{Rank} & \multicolumn{1}{c}{(T)} & \colhead{}  &
\multicolumn{1}{c}{Rank} & \multicolumn{1}{c}{(T)} & \colhead{}  &
\multicolumn{1}{c}{Rank} & \multicolumn{1}{c}{(T)} & \colhead{}  &
\multicolumn{1}{c}{Rank} & \multicolumn{1}{c}{(T)} & \colhead{}  \\
}
\startdata


 B , X & 6cm, H ,FIR, 12, D  & -0.007 & -0.068 & $>$ 0.400 &   0.097 & 0.388 & 0.354 &   -0.095 & -0.449 & 0.330 &   0.239 & 1.368 & 0.093 \nl 
 & & & & & & & & & & & & &  \nl
 H , X & 6cm, B ,FIR, 12, D  & 0.210 & 2.005 & 0.025 &   0.185 & 0.751 & 0.236 &   0.104 & 0.491 & 0.314 &   -0.275 & -1.594 & 0.064 \nl 
 & & & & & & & & & & & & &  \nl
 X , 12& 6cm, H , B ,FIR, D  & 0.060 & 0.563 & 0.289 &   0.168 & 0.683 & 0.252 &   0.232 & 1.121 & 0.147 &   0.077 & 0.428 & 0.338 \nl 
 & & & & & & & & & & & & &  \nl
 X ,FIR& 6cm, H , B , 12, D  & -0.021 & -0.197 & $>$ 0.400 &   -0.267 & -1.108 & 0.154 &   0.214 & 1.026 & 0.170 &   0.258 & 1.487 & 0.077 \nl 
 & & & & & & & & & & & & &  \nl
6cm, X &  H , B ,FIR, 12, D  & 0.250 & 2.404 & 0.010 &   0.127 & 0.513 & 0.310 &   -0.023 & -0.110 & $>$ 0.400 &   0.141 & 0.795 & 0.223 \nl 
 & & & & & & & & & & & & &  \nl
 H , B & 6cm, X ,FIR, 12, D  & 0.819 & 13.307 & $<$ 0.005 &   0.779 & 4.963 & $<$ 0.005 &   0.934 & 12.253 & $<$ 0.005 &   0.870 & 9.846 & $<$ 0.005 \nl 
 & & & & & & & & & & & & &  \nl
 B , 12& 6cm, H , X ,FIR, D  & 0.007 & 0.069 & $>$ 0.400 &   0.033 & 0.131 & $>$ 0.400 &   0.113 & 0.536 & 0.298 &   -0.144 & -0.811 & 0.219 \nl 
 & & & & & & & & & & & & &  \nl
 B ,FIR& 6cm, H , X , 12, D  & 0.293 & 2.863 & $<$ 0.005 &   0.141 & 0.572 & 0.289 &   0.166 & 0.789 & 0.226 &   0.081 & 0.455 & 0.328 \nl 
 & & & & & & & & & & & & &  \nl
6cm, B &  H , X ,FIR, 12, D  & -0.012 & -0.114 & $>$ 0.400 &   0.195 & 0.796 & 0.225 &   -0.129 & -0.610 & 0.275 &   -0.040 & -0.225 & $>$ 0.400 \nl 
 & & & & & & & & & & & & &  \nl
 H , 12& 6cm, B , X ,FIR, D  & 0.143 & 1.352 & 0.093 &   -0.066 & -0.264 & 0.399 &   0.036 & 0.171 & $>$ 0.400 &   0.311 & 1.824 & 0.041 \nl 
 & & & & & & & & & & & & &  \nl
 H ,FIR& 6cm, B , X , 12, D  & -0.255 & -2.464 & 0.009 &   -0.082 & -0.328 & 0.376 &   -0.137 & -0.646 & 0.264 &   0.124 & 0.697 & 0.246 \nl 
 & & & & & & & & & & & & &  \nl
6cm, H &  B , X ,FIR, 12, D  & -0.108 & -1.009 & 0.170 &   -0.111 & -0.447 & 0.333 &   -0.023 & -0.109 & $>$ 0.400 &   -0.068 & -0.378 & 0.356 \nl 
 & & & & & & & & & & & & &  \nl
FIR, 12& 6cm, H , B , X , D  & 0.632 & 7.602 & $<$ 0.005 &   0.715 & 4.086 & $<$ 0.005 &   0.370 & 1.868 & 0.039 &   0.509 & 3.288 & $<$ 0.005 \nl 
 & & & & & & & & & & & & &  \nl
6cm, 12&  H , B , X ,FIR, D  & 0.241 & 2.318 & 0.013 &   0.449 & 2.008 & 0.033 &   0.665 & 4.177 & $<$ 0.005 &   -0.046 & -0.259 & $>$ 0.400 \nl 
 & & & & & & & & & & & & &  \nl
6cm,FIR&  H , B , X , 12, D  & 0.359 & 3.589 & $<$ 0.005 &   0.082 & 0.329 & 0.375 &   0.157 & 0.747 & 0.237 &   0.503 & 3.241 & $<$ 0.005 \nl 
 & & & & & & & & & & & & &  \nl
\enddata
\end{deluxetable}


==> table1.tex <==
\begin{deluxetable}{lllrrrrrrrrrrr}
\tablenum{1}
\small
\tablewidth{0pc}
\tablecaption{Flux Data }
\tablehead{
\colhead{Name} & \colhead{RA} &
\colhead{DEC} & \colhead{T} &
\colhead{Dist.}  &
\colhead{$f_X$\tablenotemark{a}} & \colhead{$B$} &
\colhead{$H$} &
\colhead{$f_{\nu (12)}$\tablenotemark{a}} & \colhead{$f_{\nu (25)}$\tablenotemark{a}} &
\colhead{$f_{\nu (60)}$\tablenotemark{a}} &
\colhead{$f_{\nu (100)}$\tablenotemark{a}} &
\colhead{$f_{\nu (6cm)}$\tablenotemark{a}} &
\colhead{Refs.\tablenotemark{b}} \\
\colhead{} & \colhead{(1950)} &
\colhead{(1950)} & \colhead{} &
\colhead{(Mpc)}  &
\colhead{($10^{-13}$ cgs)} & \colhead{(mag)} &
\colhead{(mag)} &
\colhead{(mJy)\tablenotemark{c}} & \colhead{(mJy)\tablenotemark{c}} &
\colhead{(mJy)\tablenotemark{c}} &
\colhead{(mJy)\tablenotemark{c}} &
\colhead{(mJy)} &
\colhead{} \\
 }

\startdata


N0125 & 0 26 16 & 2 33 42 & 0 &  73.20& $<$ 4.28 & 13.22 & \nodata & \nodata & \nodata & \nodata & \nodata & $<$ 60 & 	21 \nl	 
N0224 & 0 40 0 & 40 59 42 & 3 &  0.77&  500. & 3.36 &  0.47 &  160\tablenotemark{c} &  110\tablenotemark{c} &  540\tablenotemark{c} &  2930\tablenotemark{c} &  2460 & 	3,8,43,45 \nl	 
N0247 & 0 44 40 & -21 2 0 & 5 &  3.00&  13.71 & 8.93 &  7.31 & $<$ 120 & $<$ 160 &  7930 &  27320 & \nodata & 	8,45 \nl	 
N0253 & 0 45 8 & -25 33 42 & 5 &  3.10&  68.81 & 7.09 &  4.24 &  60\tablenotemark{c} &  160\tablenotemark{c} &  1000\tablenotemark{c} &  1860\tablenotemark{c} &  2080 & 	10,26,45 \nl	 
SMC & 0 51 0 & -73 6 0 & 9 &  0.06&  2105. & 2.28 & \nodata &  70\tablenotemark{c}  &  270\tablenotemark{c} &  6690\tablenotemark{c} &  15020\tablenotemark{c} & \nodata & 	3,8 \nl	 
N0309 & 0 54 13 & -10 11 18 & 5 &  77.10& $<$ 2.87 & 12.11 & \nodata & $<$ 260 & $<$ 320 &  1940 &  6320 & \nodata & 	10 \nl	 
I1613 & 1 2 13 & 1 51 0 & 10 &  0.76&  21.95 & 9.82 & \nodata & $<$ 60 & $<$ 140 &  1420 &  3690 & \nodata & 	2,8 \nl	 
N0449 & 1 13 19 & 32 49 30 & 5 &  67.80& $<$ 4.77 & 14.45 &  12.62 & $<$ 1790 &  800 &  2300 &  2850 &  28 & 	10,30,65 \nl	 
N0520 & 1 22 0 & 3 31 53 & 0 &  37.80& $<$ 3.06 & 11.77 &  8.98 &  780 &  2830 &  31520 &  48400 &  72 & 	10,28,45 \nl	 
N0521  \tablenotemark{e}& 1 22 0 & 1 28 12 & 5 &  69.30& $<$ 4.39 & 12.29 & \nodata & $<$ 800 & $<$ 340 &  540 &  3450 & \nodata & 	10 \nl	 
N0524  \tablenotemark{e}& 1 22 10 & 9 16 42 & 0 &  34.80&  7.01 & 11.17 &  8.05 &  230 & $<$ 147 &  780 &  1820 &  4.1 & 	6,18,58 \nl	 
N0523 & 1 22 30 & 33 46 0 & 10 &  66.80& $<$ 2.49 & 12.43 &  10.32 & $<$ 250 &  270 &  2050 &  4700 & $<$ 18 & 	4,10,23,45 \nl	 
N0578 & 1 28 5 & -22 55 30 & 5 &  22.30& $<$ 3.46 & 11.17 &  9.46 &  230 & $<$ 320 &  3070 &  12550 & \nodata & 	10,45 \nl	 
N0598 & 1 31 3 & 30 23 53 & 5 &  0.84&  210.00 & 5.75 &  4.00 &  30\tablenotemark{c} &  40\tablenotemark{c} &  420\tablenotemark{c} &  1260\tablenotemark{c} &  1300 & 	3,8,43,45 \nl	 
N0625 & 1 32 55 & -41 41 24 & 0 &  4.90& $<$ 2.84 & 11.21 & \nodata & $<$ 260 &  900 &  5660 &  8700 & \nodata & 	10 \nl	 
N0628 & 1 34 1 & 15 31 36 & 5 &  7.30&  3.39 & 9.76 &  7.77 &  2070 &  1900 &  20860 &  65640 &  38 & 	8,24,45 \nl	 
I1727  \tablenotemark{e}& 1 44 40 & 27 5 6 & 9 &  7.60& $<$ 2.05 & 11.33 & \nodata & $<$ 250 & $<$ 250 &  390 &  1890 & \nodata & 	10 \nl	 
N0672 & 1 45 5 & 27 11 6 & 5 &  7.90& $<$ 2.14 & 10.50 & \nodata & $<$ 250 &  370 &  3370 &  8340 & $<$ 4.8 & 	10,42 \nl	 
N0772  \tablenotemark{e}& 1 56 35 & 18 46 0 & 3 &  32.80& $<$ 6.04 & 10.55 &  7.91 &  290 &  530 &  4950 &  21660 &  27 & 	10,43,45 \nl	 
N0871 & 2 14 27 & 14 19 0 & 5 &  52.20& $<$ 2.51 & 13.04 & \nodata & $<$ 250 &  310 &  3880 &  7550 &  41 & 	10,24 \nl	 
N0877 & 2 15 16 & 14 18 53 & 5 &  54.50&  2.37 & 11.96 &  9.68 &  370 &  550 &  9050 &  24370 &  40 & 	10,43,51 \nl	 
N0936 & 2 25 5 & -1 22 42 & 0 &  19.30&  4.35 & 10.98 &  7.74 & $<$ 70 & $<$ 135 & $<$ 132 & $<$ 270 &  3.7 & 	6,20,45 \nl	 
N0941 & 2 25 55 & -1 22 30 & 6 &  22.90& $<$ 14.90 & 12.67 & \nodata & $<$ 250 & $<$ 250 &  830 &  2530 & \nodata & 	10 \nl	 
N0945 & 2 26 10 & -10 45 36 & 5 &  60.70& $<$ 1.61 & 12.60 & \nodata & $<$ 250 & $<$ 250 &  950 &  3810 & \nodata & 	10 \nl	 
N0985 \tablenotemark{d} & 2 32 11 & -9 0 18 & 10 &  173.30&  200.75 & 13.89 & \nodata & $<$ 270 &  550 &  1440 &  2000 & \nodata & 	10 \nl	 
N1042 & 2 37 56 & -8 38 47 & 5 &  19.20&  5.78 & 11.36 & \nodata & $<$ 250 & $<$ 260 &  1190 &  6560 & \nodata & 	10 \nl	 
N1068 \tablenotemark{d} & 2 40 7 & -0 13 30 & 3 &  16.50&  206.50 & 9.47 &  6.04 &  40\tablenotemark{c} &  90\tablenotemark{c} &  190\tablenotemark{c} &  240\tablenotemark{c} &  2190 & 	10,23,45 \nl	 
N1073 & 2 41 5 & 1 9 53 & 5 &  17.60&  3.82 & 11.36 & \nodata & $<$ 250 & $<$ 250 &  1150 &  6050 &  110 & 	2,10,26 \nl	 
N1087 & 2 43 52 & -0 42 30 & 5 &  21.50& $<$ 7.13 & 10.97 & \nodata &  590 &  830 &  9270 &  29550 &  45 & 	10,44 \nl	 
N1090 & 2 44 1 & -0 27 23 & 5 &  38.10& $<$ 4.29 & 11.83 &  9.73 & $<$ 250 & $<$ 330 &  870 &  3780 & \nodata & 	10,45 \nl	 
N1097 & 2 44 11 & -30 29 6 & 4 &  16.50&  30.30 & 9.92 &  6.79 &  2880 &  7700 &  46730 &  116340 &  130 & 	8,26,58 \nl	 
N1218 \tablenotemark{d} & 3 5 49 & 3 55 12 & 0 &  116.60&  25.84 & 13.16 &  10.34 & $<$ 80 &  110 & $<$ 72 &  420 & $<$ 3000 & 	6,31,59 \nl	 
N1300 & 3 17 25 & -19 35 30 & 3 &  20.80&  1.65 & 10.77 &  8.76 & $<$ 250 & $<$ 300 &  2410 &  11180 & \nodata & 	10,45 \nl	 
N1313 & 3 17 39 & -66 40 42 & 5 &  4.50&  18.91 & 9.29 & \nodata &  950 &  3490 &  35970 &  92000 &  59 & 	8,26 \nl	 
N1317 & 3 20 51 & -37 16 53 & 1 &  18.40& $<$ 2.66 & 11.81 & \nodata &  280 &  270 &  3690 &  9530 & \nodata & 	6 \nl	 
N1350 & 3 29 10 & -33 47 54 & 1 &  18.40& $<$ 4.77 & 10.87 &  8.05 & $<$ 250 & $<$ 250 & $<$ 570 &  3970 & \nodata & 	10,45 \nl	 
N1358  \tablenotemark{e}& 3 31 11 & -5 15 23 & 1 &  54.10&  1.40 & 12.70 &  9.70 & $<$ 82.86 & $<$ 123.6 &  378 &  925 &  1.2 & 	39,17,58 \nl	 
N1365 & 3 31 42 & -36 18 17 & 3 &  18.40&  17.12 & 9.93 &  6.84 &  4420 &  13070 &  84200 &  185400 &  210 & 	8,26,45 \nl	 
N1380 & 3 34 31 & -35 8 23 & 0 &  15.80&  6.84 & 10.92 &  7.65 &  170 &  70 &  1070 &  3060 &  1.9 & 	6,18,63 \nl	 
N1386 & 3 34 52 & -36 9 53 & 1 &  18.40&  5.97 & 12.12 &  8.79 &  530 &  1500 &  5650 &  8890 &  30.0 & 	6,20,57 \nl	 
N1398 & 3 36 45 & -26 29 53 & 2 &  18.00&  3.60 & 10.39 &  7.09 & $<$ 250 & $<$ 250 &  930 &  7820 & \nodata & 	10,45 \nl	 
N1421 & 3 40 9 & -13 38 54 & 5 &  27.80&  6.41 & 11.00 &  9.37 &  370 &  400 &  7440 &  21790 & \nodata & 	2,10,45 \nl	 
I0342 & 3 41 57 & 67 56 24 & 6 &  3.60&  49.27 & 6.04 &  5.73 &  23660 &  45200 &  255960 &  661680 &  80 & 	8,29,50 \nl	 
N1512 & 4 2 16 & -43 29 12 & 3 &  10.20& $<$ 3.71 & 10.96 &  8.59 & $<$ 400 & $<$ 250 &  890 &  1130 & $<$ 12.6 & 	11,37,56 \nl	 
N1533 & 4 8 50 & -56 15 0 & 0 &  15.50&  2.76 & 11.74 & \nodata & $<$ 93 &  60 &  330 &  1240 & $<$ 26.4 & 	6,38 \nl	 
N1559 & 4 17 1 & -62 54 17 & 5 &  16.00&  9.80 & 10.81 &  8.83 &  890 &  1650 &  23830 &  58330 &  120 & 	10,26,45 \nl	 
N1566 \tablenotemark{d} & 4 18 53 & -55 3 24 & 5 &  15.50&  82.68 & 10.16 &  7.39 &  530 &  890 &  12700 &  42200 &  76 & 	10,26,45 \nl	 
N1569 & 4 26 5 & 64 44 24 & 9 &  1.70&  19.31 & 9.42 &  8.23 &  680 &  6840 &  46680 &  51710 &  278 & 	10,23,60 \nl	 
N1614 & 4 31 36 & -8 40 54 & 5 &  63.40&  6.50 & 13.28 &  10.31 &  1380 &  7550 &  33540 &  32380 & \nodata & 	10,57 \nl	 
N1625 & 4 34 35 & -3 24 12 & 4 &  62.60& $<$ 2.77 & 12.08 & \nodata & $<$ 250 & $<$ 250 &  1070 &  3740 & \nodata & 	10 \nl	 
N1672 & 4 44 58 & -59 19 36 & 3 &  15.30&  7.65 & 10.25 &  7.97 &  1470 &  4030 &  34800 &  69460 &  100 & 	10,26,58 \nl	 
N1784 & 5 3 7 & -11 56 24 & 4 &  30.10& $<$ 2.62 & 11.63 &  9.07 & $<$ 250 & $<$ 350 &  2440 &  9300 & \nodata & 	10,45 \nl	 
LMC & 5 24 0 & -69 48 0 & 9 &  0.05&  8563. & 0.57 & \nodata &  2780\tablenotemark{c} &  7820\tablenotemark{c} &  82920\tablenotemark{c} &  184690\tablenotemark{c} & \nodata & 	3,8 \nl	 
N1961  \tablenotemark{e}& 5 36 34 & 69 21 17 & 3 &  75.40&  2.77 & 11.01 &  8.34 &  510 &  470 &  6600 &  22070 &  64 & 	10,42,45 \nl	 
U3691 & 7 5 6 & 15 15 0 & 6 &  28.90& $<$ 3.48 & 11.43 &  11.38 & $<$ 250 & $<$ 250 &  1360 &  3790 & \nodata & 	10,47 \nl	 
N2276 & 7 10 31 & 85 50 54 & 5 &  17.10& $<$ 6.82 & 11.75 & \nodata &  580 &  1130 &  11800 &  29500 &  104 & 	10,36 \nl	 
N2366 & 7 23 37 & 69 19 6 & 9 &  3.40& $<$ 2.39 & 10.95 &  10.60 & $<$ 250 &  720 &  3300 &  4580 &  20 & 	10,42,45 \nl	 
N2403 & 7 32 3 & 65 42 42 & 5 &  3.20&  19.12 & 8.43 &  6.21 &  3340 &  6290 &  51550 &  148490 &  53 & 	8,24,45 \nl	 
N2441 & 7 46 20 & 73 9 23 & 5 &  56.50& $<$ 3.34 & 12.57 & \nodata & $<$ 250 & $<$ 250 &  830 &  3590 & $<$ 5.7 & 	10,42 \nl	 
N2525 & 8 3 15 & -11 17 6 & 5 &  18.60& $<$ 2.86 & 11.55 & \nodata & $<$ 250 &  570 &  6080 &  16760 & \nodata & 	10 \nl	 
N2608 & 8 32 15 & 28 38 47 & 4 &  28.20&  1.15 & 12.53 & \nodata & $<$ 250 &  250 &  2300 &  5970 &  27 & 	2,10,23 \nl	 
N2642 & 8 38 14 & -3 56 35 & 3 &  55.50& $<$ 3.47 & 13.02 & \nodata & $<$ 250 & $<$ 260 &  810 &  3200 & \nodata & 	10 \nl	 
N2683  \tablenotemark{e}& 8 49 35 & 33 36 30 & 3 &  5.40& $<$ 8.24 & 9.62 &  6.71 &  930 &  520 &  8330 &  34020 &  20 & 	8,19,45 \nl	 
N2763 & 9 4 29 & -15 17 53 & 5 &  22.20& $<$ 2.26 & 12.35 & \nodata & $<$ 290 & $<$ 260 &  2060 &  5990 & \nodata & 	10 \nl	 
N2773 & 9 6 58 & 7 23 6 & 5 &  70.20&  2.59 & 14.27 & \nodata & $<$ 270 &  390 &  2840 &  5260 & \nodata & 	10 \nl	 
N2775 & 9 7 41 & 7 14 30 & 1 &  17.10&  4.22 & 10.81 &  7.83 & $<$ 250 & $<$ 280 &  1740 &  10470 & $<$ 10 & 	10,22,45 \nl	 
N2777 & 9 8 2 & 7 24 42 & 2 &  17.10& $<$ 1.63 & 13.88 & \nodata & $<$ 250 & $<$ 320 &  750 &  1290 & $<$ 10 & 	10,22 \nl	 
N2782 & 9 10 54 & 40 19 17 & 1 &  34.50& $<$ 5.40 & 12.01 &  9.54 &  510 &  1470 &  8470 &  13810 &  55.0 & 	10,20,64 \nl	 
N2835 & 9 15 37 & -22 8 48 & 5 &  8.50&  2.03 & 10.31 &  8.92 & $<$ 250 & $<$ 250 &  2560 &  14400 & \nodata & 	2,10,45 \nl	 
N2848 & 9 17 49 & -16 18 47 & 5 &  24.10& $<$ 2.08 & 11.95 & \nodata & $<$ 250 & $<$ 250 &  1180 &  5000 & \nodata & 	10 \nl	 
N2841  \tablenotemark{e}& 9 18 35 & 51 11 18 & 3 &  24.90&  4.71 & 9.58 &  6.75 &  900 &  830 &  4410 &  24210 &  14 & 	8,19,45 \nl	 
N2903 & 9 29 20 & 21 43 12 & 5 &  6.40&  14.34 & 9.11 &  6.52 &  5000 &  7640 &  52380 &  147360 &  148 & 	8,24,45 \nl	 
N2914 & 9 31 21 & 10 19 54 & 2 &  40.20& $<$ 4.03 & 13.71 & \nodata & $<$ 84 & $<$ 108 &  290 &  560 & $<$ 36 & 	13,23 \nl	 
N2992 \tablenotemark{d} & 9 43 18 & -14 5 41 & 1 &  28.40&  204.80 & 12.16 &  9.09 &  590 &  1360 &  6870 &  14440 &  8.5 & 	10,20,57 \nl	 
N2993 & 9 43 23 & -14 8 6 & 2 &  28.40& $<$ 10.02 & 12.65 &  10.90 &  470 &  1600 &  10230 &  15510 & \nodata & 	1,10,67 \nl	 
N3031  \tablenotemark{e}& 9 51 30 & 69 18 17 & 3 &  3.60&  92.92 & 7.39 &  4.18 &  5860 &  5420 &  44730 &  174020 &  118 & 	8,24,45 \nl	 
N3034 & 9 51 41 & 69 54 54 & 0 &  3.60&  235.45 & 8.83 &  4.68 &  70\tablenotemark{c} &  290\tablenotemark{c} &  1270\tablenotemark{c} &  1350\tablenotemark{c} &  4078 & 	8,23,45 \nl	 
N3067 & 9 55 26 & 32 36 30 & 3 &  19.30& $<$ 4.94 & 12.22 & \nodata &  670 &  1020 &  9140 &  19130 & $<$ 252 & 	10,42 \nl	 
N3081 & 9 57 11 & -22 35 5 & 1 &  28.00&  8.09 & 12.59 &  9.81 & \nodata & \nodata & \nodata & \nodata &  0.9 & 	7,39,57 \nl	 
N3066 & 9 57 51 & 72 21 54 & 4 &  29.60& $<$ 8.19 & 13.27 &  11.39 & $<$ 360 &  540 &  3030 &  5680 & \nodata & 	10,49 \nl	 
N3079  \tablenotemark{e}& 9 58 35 & +55 55 24 & 5 &  19.40& $<$ 11.47 & 10.41 &  7.63 &  1240 &  2030 &  42860 &  88950 &  330 & 	10,24,45 \nl	 
N3077 & 9 59 22 & 68 58 30 & 0 &  3.60& $<$ 3.10 & 10.41 &  8.21 &  520 &  1890 &  14800 &  25110 & $<$ 24 & 	10,24,45 \nl	 
N3125 & 10 4 18 & -29 41 30 & 0 &  10.60& $<$ 6.76 & 13.11 &  11.36 & $<$ 250 & $<$ 790 &  4970 &  6480 & \nodata & 	10,58 \nl	 
N3166  \tablenotemark{e}& 10 11 10 & 3 40 30 & 1 &  8.80&  3.04 & 11.01 & \nodata &  310 &  420 &  5900 &  13570 & $<$ 10 & 	6,20 \nl	 
N3169  \tablenotemark{e}& 10 11 38 & 3 43 12 & 3 &  8.80& $<$ 4.12 & 10.96 & \nodata &  550 &  600 &  6780 &  19940 &  23 & 	10,22 \nl	 
N3175 & 10 12 24 & -28 37 12 & 5 &  11.10& $<$ 6.10 & 11.23 & \nodata &  690 &  1210 &  12400 &  31440 & \nodata & 	10 \nl	 
N3184 & 10 15 17 & 41 40 0 & 5 &  7.20& $<$ 47.16 & 10.34 & \nodata & $<$ 250 & $<$ 540 &  2350 &  15380 &  13 & 	1,10,19 \nl	 
N3227 \tablenotemark{d} & 10 20 47 & 20 7 5 & 3 &  14.20&  140.34 & 11.18 &  8.35 &  670 &  1740 &  7980 &  17460 &  34 & 	10,30,64 \nl	 
I2574 & 10 24 40 & 68 40 6 & 9 &  3.60&  1.44 & 10.33 &  9.98 & $<$ 51 &  80 &  2410 &  10620 & \nodata & 	8,45 \nl	 
N3281 & 10 29 36 & -34 36 0 & 1 &  41.90& $<$ 7.22 & 11.92 &  9.35 &  880 &  2560 &  6760 &  7680 &  26.7 & 	10,39,57 \nl	 
N3310 & 10 35 39 & 53 45 54 & 4 &  14.20&  10.92 & 10.95 &  9.05 &  1240 &  4640 &  33290 &  41760 &  146 & 	10,23,49 \nl	 
N3346 & 10 40 59 & 15 8 6 & 5 &  15.20& $<$ 1.99 & 12.24 & \nodata & $<$ 250 & $<$ 360 &  1340 &  5520 & \nodata & 	10 \nl	 
N3351 & 10 41 19 & 11 58 5 & 3 &  10.10& $<$ 7.80 & 10.26 &  7.29 &  570 &  1910 &  17370 &  35300 &  41 & 	10,36,45 \nl	 
N3353 & 10 42 17 & 56 13 36 & 3 &  13.90&  1.73 & 13.00 &  11.24 & $<$ 250 &  920 &  5180 &  6650 & \nodata & 	10,66 \nl	 
N3368  \tablenotemark{e}& 10 44 8 & 12 5 5 & 2 &  11.30& $<$ 5.51 & 9.80 &  6.72 &  370 & $<$ 560 &  9160 &  27440 & $<$ 24 & 	10,26,45 \nl	 
N3389 & 10 45 50 & 12 47 54 & 5 &  29.90& $<$ 6.79 & 11.83 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 	7 \nl	 
N3395 & 10 47 2 & 33 14 41 & 5 &  21.20&  3.72 & 12.09 &  11.66 & $<$ 250 &  510 &  8160 &  16800 &  41 & 	11,23,53 \nl	 
N3430 & 10 49 25 & 33 12 53 & 4 &  20.80& $<$ 2.87 & 11.72 &  9.48 & $<$ 360 & $<$ 250 &  2870 &  8320 & \nodata & 	10,45 \nl	 
N3445 & 10 51 34 & 57 15 18 & 5 &  28.30& $<$ 3.33 & 12.84 & \nodata & $<$ 250 & $<$ 260 &  2200 &  4460 & \nodata & 	10 \nl	 
N3448 & 10 51 40 & 54 34 30 & 0 &  19.20&  3.81 & 11.84 & \nodata &  350 &  580 &  5620 &  11160 &  39 & 	10,24 \nl	 
N3455 & 10 51 52 & 17 33 5 & 5 &  13.30& $<$ 2.63 & 12.51 & \nodata & $<$ 300 & $<$ 390 &  1020 &  0 & \nodata & 	10 \nl	 
N3489  \tablenotemark{e}& 10 57 41 & 14 10 11 & 0 &  11.60& $<$ 4.60 & 11.15 & \nodata & \nodata & \nodata & \nodata & \nodata &  1.5 & 	7,18 \nl	 
N3504 & 11 0 29 & 28 14 30 & 3 &  19.80&  4.03 & 11.65 &  8.63 &  1040 &  3720 &  19170 &  32890 &  115 & 	10,19,49 \nl	 
N3512 & 11 1 20 & 28 18 17 & 5 &  17.60& $<$ 3.72 & 12.87 & \nodata & $<$ 250 & $<$ 410 &  1390 &  4100 & \nodata & 	10 \nl	 
N3593 & 11 12 0 & 13 5 24 & 1 &  6.60&  2.37 & 11.45 & \nodata &  1310 &  2090 &  18870 &  35600 &  67.0 & 	6,20 \nl	 
N3628  \tablenotemark{e}& 11 17 40 & 13 52 5 & 4 &  11.90&  16.41 & 9.31 &  6.73 &  3080 &  5300 &  48510 &  122170 &  224 & 	8,24,45 \nl	 
N3690 & 11 25 42 & 58 50 0 & 9 &  43.20&  4.80 & 11.85 &  9.23 &  3710 &  21510 &  105820 &  111160 &  346 & 	1,11,23,48 \nl	 
N3718  \tablenotemark{e}& 11 29 50 & 53 20 42 & 1 &  14.30& $<$ 8.69 & 11.19 &  7.62 &  150 &  110 &  760 &  2520 & $<$ 90 & 	6,21,68 \nl	 
N3729 & 11 31 4 & 53 24 0 & 1 &  15.50& $<$ 3.57 & 11.91 & \nodata & $<$ 290 &  370 &  2660 &  7760 & \nodata & 	10 \nl	 
N3783 \tablenotemark{d} & 11 36 33 & -37 27 42 & 1 &  35.10&  416.29 & 12.04 &  9.44 &  770 &  2430 &  3370 &  5120 &  13.0 & 	10,40,57 \nl	 
N3884  \tablenotemark{e}& 11 43 36 & 20 41 4 & 1 &  91.50&  11.81 & 13.26 &  8.93 & \nodata & \nodata & \nodata & \nodata & \nodata & 	52 \nl	 
N3887 & 11 44 33 & -16 34 35 & 3 &  12.80& $<$ 2.36 & 11.19 & \nodata & $<$ 290 & $<$ 420 &  4490 &  15930 & \nodata & 	10 \nl	 
N3888 & 11 44 55 & 56 14 53 & 5 &  33.40& $<$ 1.79 & 12.55 &  10.23 &  320 &  470 &  4810 &  11390 & $<$ 30 & 	10,24,48 \nl	 
N3893 & 11 46 1 & 48 59 24 & 5 &  15.50& $<$ 2.92 & 10.68 &  8.65 &  820 &  1130 &  13800 &  35070 &  45 & 	10,24,45 \nl	 
N3896 & 11 46 18 & 48 57 12 & 0 &  15.50& $<$ 1.99 & 13.75 & \nodata & \nodata & \nodata & \nodata & \nodata & $<$ 24 & 	33 \nl	 
N3991 & 11 54 55 & 32 36 48 & 10 &  42.10&  4.82 & 13.32 &  12.71 & $<$ 250 & $<$ 290 &  2550 &  4840 &  36 & 	10,23,53 \nl	 
N3994 & 11 55 1 & 32 33 18 & 5 &  42.10& $<$ 3.39 & 13.18 & \nodata & $<$ 270 & $<$ 520 &  2750 &  10430 &  25 & 	11,43 \nl	 
N3995 & 11 55 10 & 32 34 17 & 5 &  42.10& $<$ 3.35 & 12.32 & \nodata & \nodata & \nodata & \nodata & \nodata &  41 & 	11,24 \nl	 
I0749 & 11 56 0 & 43 0 48 & 5 &  15.50& $<$ 1.82 & 12.81 & \nodata & \nodata & \nodata & \nodata & \nodata & $<$ 27 & 	7,33 \nl	 
I0750 & 11 56 17 & 43 0 6 & 3 &  15.50& $<$ 1.86 & 12.39 & \nodata & \nodata & \nodata & \nodata & \nodata &  63 & 	7,24 \nl	 
N4036  \tablenotemark{e}& 11 58 54 & 62 10 30 & 0 &  20.30& $<$ 4.10 & 11.49 &  8.16 &  110 & $<$ 75 &  580 &  1450 &  3.0 & 	6,20,68 \nl	 
N4038 & 11 59 19 & -18 35 5 & 5 &  23.30&  14.16 & 10.62 & \nodata &  1220 &  3910 &  39220 &  75970 &  210 & 	11,27 \nl	 
N4041 & 11 59 39 & 62 25 0 & 5 &  18.20& $<$ 5.79 & 11.76 & \nodata &  820 &  1400 &  13870 &  31490 &  38 & 	10,24 \nl	 
N4051 \tablenotemark{d} & 12 0 37 & 44 48 42 & 4 &  15.50&  220.45 & 10.74 &  9.21 &  770 &  1400 &  8280 &  20940 &  45 & 	10,24,64 \nl	 
N4151 \tablenotemark{d} & 12 8 0 & 39 40 54 & 2 &  13.50&  97.00 & 10.71 &  7.81 & \nodata & \nodata & \nodata & \nodata &  158 & 	7,24,64 \nl	 
N4156 & 12 8 17 & 39 44 54 & 3 &  90.20&  5.37 & 13.79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 	7 \nl	 
N4178 & 12 10 14 & 11 8 48 & 5 &  12.60& $<$ 2.79 & 11.35 &  9.85 & $<$ 450 &  520 &  4300 &  9890 & \nodata & 	12,45 \nl	 
N4190 & 12 11 13 & 36 54 35 & 9 &  3.50&  5.92 & 13.36 & \nodata & $<$ 121.1 & $<$ 123.2 &  400 &  1490 &  5.0 & 	14,41,17 \nl	 
N4192  \tablenotemark{e}& 12 11 15 & 15 10 48 & 3 &  14.50&  1.33 & 10.02 &  7.53 &  650 &  360 &  7190 &  23180 &  33 & 	8,43,45 \nl	 
N4206 & 12 12 44 & 13 18 12 & 4 &  19.70& $<$ 2.03 & 11.73 &  9.88 & $<$ 300 & $<$ 420 &  1150 &  2490 & \nodata & 	12,45 \nl	 
N4212 & 12 13 7 & 14 10 48 & 5 &  18.70&  1.91 & 11.35 & \nodata &  770 &  1170 &  7500 &  16940 & \nodata & 	12 \nl	 
N4214 & 12 13 8 & 36 36 30 & 9 &  4.10& $<$ 39.96 & 10.14 &  8.53 &  390 &  1750 &  14470 &  25470 &  46 & 	1,10,36,45 \nl	 
N4216  \tablenotemark{e}& 12 13 21 & 13 25 23 & 3 &  16.80&  1.14 & 9.95 &  7.05 & $<$ 120 & $<$ 200 &  2270 &  12790 & \nodata & 	8,45 \nl	 
N4224 & 12 14 1 & 7 44 24 & 1 &  45.70& $<$ 3.90 & 12.52 & \nodata & $<$ 200 & $<$ 180 &  170 &  860 & \nodata & 	12 \nl	 
N4236 & 12 14 22 & 69 45 0 & 7 &  3.60&  1.02 & 9.53 &  8.66 &  110 &  570 &  3980 &  10020 & \nodata & 	2,5,8,45 \nl	 
N4235 \tablenotemark{d} & 12 14 37 & 7 28 6 & 1 &  19.80&  40.61 & 11.89 &  9.69 & $<$ 110 & $<$ 210 &  320 &  640 &  5.3 & 	12,40,67 \nl	 
N4244 & 12 15 0 & 38 5 11 & 6 &  4.50&  2.20 & 9.28 &  8.43 & $<$ 51 & $<$ 70 &  4200 &  16060 & \nodata & 	2,8,45 \nl	 
N4245 & 12 15 5 & 29 52 54 & 1 &  11.40& $<$ 2.91 & 12.01 & \nodata & $<$ 110 & $<$ 120 &  810 &  2680 & \nodata & 	6 \nl	 
N4246 & 12 15 25 & 7 27 54 & 5 &  36.80& $<$ 3.54 & 12.91 &  11.25 & \nodata & \nodata & \nodata & \nodata & \nodata & 	45 \nl	 
N4254 & 12 16 17 & 14 41 42 & 5 &  12.90&  4.56 & 10.10 & \nodata &  4020 &  4600 &  44000 &  96320 &  135 & 	12,24 \nl	 
N4258  \tablenotemark{e}& 12 16 29 & 47 35 0 & 3 &  7.20&  45.66 & 8.53 &  5.95 &  2250 &  2810 &  21600 &  78390 &  246 & 	1,5,8,24,45 \nl	 
N4260 & 12 16 49 & 6 22 36 & 1 &  42.40& $<$ 5.86 & 12.31 & \nodata & $<$ 500 & $<$ 230 &  200 &  950 & \nodata & 	12 \nl	 
N4298 & 12 19 0 & 14 53 5 & 5 &  16.10&  2.22 & 11.62 & \nodata &  610 &  880 &  3400 &  11440 & \nodata & 	12 \nl	 
N4303 & 12 19 22 & 4 45 5 & 5 &  10.60&  9.42 & 10.12 &  7.83 &  3650 &  5060 &  41000 &  77400 &  120 & 	12,26,45 \nl	 
N4321  \tablenotemark{e}& 12 20 23 & 16 6 0 & 5 &  16.10&  8.43 & 9.98 &  7.80 &  2830 &  3430 &  31000 &  70520 &  82 & 	12,24,45 \nl	 
N4351 & 12 21 29 & 12 28 54 & 2 &  12.90& $<$ 3.86 & 12.79 & \nodata & $<$ 100 & $<$ 180 &  740 &  2060 & \nodata & 	12 \nl	 
N4378  \tablenotemark{e}& 12 22 45 & 5 12 6 & 1 &  49.10&  3.28 & 12.22 & \nodata & $<$ 200 & $<$ 280 & $<$ 900 &  1460 & \nodata & 	2,12 \nl	 
N4385 & 12 23 12 & 0 50 54 & 4 &  26.20& $<$ 7.43 & 12.90 &  10.56 &  270 &  1150 &  4550 &  5910 & \nodata & 	6,48 \nl	 
N4388  \tablenotemark{e}& 12 23 14 & 12 56 17 & 2 &  16.70&  6.60 & 10.79 &  8.48 &  1120 &  3500 &  11500 &  18060 &  97 & 	12,24,45 \nl	 
N4394  \tablenotemark{e}& 12 23 25 & 18 29 23 & 3 &  24.30& $<$ 1.43 & 11.51 &  8.76 &  280 &  270 &  1150 &  4990 & \nodata & 	12,53 \nl	 
N4424 & 12 24 40 & 9 41 47 & 1 &  4.00&  0.44 & 11.94 & \nodata &  180 &  370 &  3000 &  5500 & \nodata & 	12 \nl	 
N4429  \tablenotemark{e}& 12 24 54 & 11 23 6 & 0 &  13.00&  3.20 & 10.97 &  7.50 &  200 & $<$ 120 &  1600 &  4580 & $<$ 8.4 & 	2,6,38,45 \nl	 
N4438  \tablenotemark{e}& 12 25 14 & 13 17 6 & 3 &  12.30&  5.89 & 10.49 &  7.78 &  170 & $<$ 150 &  4280 &  12050 &  77 & 	8,26,61 \nl	 
N4449 & 12 25 47 & 44 22 17 & 9 &  2.90&  12.72 & 9.94 &  8.09 & \nodata & \nodata & \nodata & \nodata &  136 & 	7,24,45 \nl	 
N4450  \tablenotemark{e}& 12 25 59 & 17 21 42 & 2 &  14.20&  11.48 & 10.75 &  7.96 &  150 & $<$ 270 &  1800 &  7910 & \nodata & 	12,45 \nl	 
N4461 & 12 26 31 & 13 27 42 & 1 &  12.00& $<$ 3.44 & 11.95 & \nodata &  130 & $<$ 100 & $<$ 50 & $<$ 225 & $<$ 8.1 & 	6,38 \nl	 
N4464 & 12 26 49 & 8 26 6 & 0 &  18.40& $<$ 4.48 & 13.39 &  10.26 & $<$ 132 & $<$ 140 & $<$ 93 &  310 & \nodata & 	6,54 \nl	 
N4477  \tablenotemark{e}& 12 27 31 & 13 54 42 & 0 &  16.40&  7.07 & 11.30 &  8.06 &  160 & $<$ 132 &  590 &  1250 & $<$ 0.27 & 	6,18,45 \nl	 
N4501  \tablenotemark{e}& 12 29 28 & 14 41 42 & 4 &  17.40&  7.53 & 9.86 &  7.09 &  2340 &  3020 &  21000 &  59340 &  74 & 	12,24,45 \nl	 
N4503 & 12 29 34 & 11 27 12 & 1 &  11.70& $<$ 1.29 & 12.05 & \nodata & $<$ 75 & $<$ 84 & $<$ 120 & $<$ 507 & $<$ 7.5 & 	6,38 \nl	 
N4522 & 12 31 8 & 9 27 0 & 4 &  16.30& $<$ 6.16 & 11.99 &  10.35 & $<$ 210 &  230 &  1700 &  3960 & \nodata & 	12,45 \nl	 
N4527  \tablenotemark{e}& 12 31 35 & 2 55 42 & 3 &  13.70& $<$ 5.52 & 10.66 & \nodata &  1010 &  1870 &  25820 &  63520 &  151 & 	10,44 \nl	 
N4535 & 12 31 48 & 8 28 36 & 5 &  12.40& $<$ 2.79 & 10.32 &  8.58 &  1190 &  1520 &  14000 &  31820 &  38 & 	12,43,45 \nl	 
N4536 & 12 31 54 & 2 27 42 & 5 &  16.60&  5.90 & 10.58 &  8.11 &  1410 &  3470 &  30330 &  44980 &  85 & 	10,26,45 \nl	 
I3528 \tablenotemark{d} & 12 32 25 & 15 50 30 & 3 &  182.20&  26.49 & 15.12 & \nodata & $<$ 290 & $<$ 460 &  1350 &  5740 & \nodata & 	11 \nl	 
N4548  \tablenotemark{e}& 12 32 55 & 14 46 24 & 3 &  14.50& $<$ 4.85 & 10.79 & \nodata &  390 &  270 &  2800 &  10920 & \nodata & 	12 \nl	 
N4565  \tablenotemark{e}& 12 33 52 & 26 15 36 & 3 &  10.60&  7.85 & 9.10 &  6.22 &  1530 &  1700 &  9830 &  47230 &  45 & 	8,24,45 \nl	 
N4567 & 12 34 1 & 11 32 0 & 5 &  22.30&  4.68 & 11.79 &  10.55 &  580 &  980 &  15530 &  47590 &  46 & 	11,24,53 \nl	 
N4569  \tablenotemark{e}& 12 34 19 & 13 26 23 & 2 &  9.00&  6.00 & 9.79 &  7.33 &  750 &  1280 &  9190 &  27330 &  41 & 	8,26,45 \nl	 
N4571 & 12 34 25 & 14 29 36 & 5 &  14.90& $<$ 3.41 & 11.73 & \nodata & $<$ 250 & $<$ 250 &  950 &  6530 & \nodata & 	10 \nl	 
N4579  \tablenotemark{e}& 12 35 12 & 12 5 35 & 2 &  20.00&  78.64 & 10.29 &  7.28 &  940 &  720 &  6700 &  18920 &  57 & 	12,24,45 \nl	 
N4594  \tablenotemark{e}& 12 37 23 & -11 21 0 & 2 &  9.40&  29.24 & 8.38 &  5.55 &  740 &  500 &  4260 &  22860 &  170 & 	8,26,45 \nl	 
N4603 & 12 38 11 & -40 42 5 & 5 &  30.30&  2.21 & 11.53 &  9.26 & $<$ 250 & $<$ 250 &  2220 &  11410 & \nodata & 	10,45 \nl	 
N4631 & 12 39 41 & 32 48 47 & 5 &  3.50&  13.81 & 8.61 &  6.16 &  5480 &  9650 &  82900 &  208660 &  168 & 	8,19,45 \nl	 
N4639  \tablenotemark{e}& 12 40 21 & 13 31 53 & 3 &  25.10&  12.95 & 11.85 & \nodata & $<$ 300 & $<$ 270 &  1850 &  4470 & \nodata & 	12 \nl	 
N4643  \tablenotemark{e}& 12 40 48 & 2 15 6 & 0 &  16.00&  2.35 & 11.54 &  8.09 & $<$ 80 & $<$ 144 &  640 &  1830 & $<$ 0.57 & 	2,6,18,45 \nl	 
N4647 & 12 41 1 & 11 51 12 & 5 &  19.80& $<$ 7.58 & 11.81 &  10.56 &  960 &  900 &  6100 &  15570 & $<$ 9 & 	1,12,33,53 \nl	 
N4651  \tablenotemark{e}& 12 41 13 & 16 40 5 & 5 &  20.70& $<$ 3.43 & 11.04 &  8.53 &  630 &  720 &  6300 &  14190 & \nodata & 	12,45 \nl	 
N4654 & 12 41 26 & 13 24 0 & 5 &  13.00& $<$ 3.16 & 10.75 &  8.69 &  1260 &  1730 &  14700 &  34400 &  48 & 	12,43,45 \nl	 
N4665 & 12 42 33 & 3 19 47 & 0 &  16.00& $<$ 3.10 & 11.36 & \nodata & $<$ 63 & $<$ 144 & $<$ 81 & $<$ 132 & $<$ 0.33 & 	6,18 \nl	 
N4689 & 12 45 15 & 14 2 5 & 5 &  14.10&  8.77 & 11.39 & \nodata &  480 &  370 &  3900 &  9630 & \nodata & 	12 \nl	 
N4698  \tablenotemark{e}& 12 45 52 & 8 45 35 & 1 &  36.30&  2.38 & 11.24 &  8.36 &  280 & $<$ 460 &  630 &  1890 & \nodata & 	2,12,45 \nl	 
N4736  \tablenotemark{e}& 12 48 32 & 41 23 36 & 2 &  5.90&  20.42 & 8.75 &  5.15 &  4770 &  6830 &  62410 &  135340 &  90 & 	1,8,24,45 \nl	 
N4826  \tablenotemark{e}& 12 54 17 & 21 57 5 & 2 &  4.60&  7.89 & 8.82 &  5.99 &  1710 &  2000 &  33860 &  77380 &  58 & 	8,24,45 \nl	 
N4845 & 12 55 28 & 1 50 47 & 1 &  30.50& $<$ 2.52 & 11.42 & \nodata &  440 &  680 &  9450 &  23670 & \nodata & 	10 \nl	 
N4861 & 12 56 40 & 35 7 54 & 9 &  11.40&  7.42 & 12.17 &  10.86 & $<$ 250 &  390 &  1840 &  2390 & $<$ 30 & 	11,23,53 \nl	 
I4182 & 13 3 30 & 37 52 30 & 9 &  4.70& $<$ 20.89 & 11.73 & \nodata & $<$ 91.9 & $<$ 75.47 &  567 &  1693 & \nodata & 	1,17 \nl	 
N5033  \tablenotemark{e}& 13 11 8 & 36 51 47 & 4 &  12.00&  77.37 & 10.21 &  7.34 &  1380 &  1770 &  17200 &  51050 &  54 & 	8,24,45 \nl	 
N5037 & 13 12 22 & -16 19 36 & 2 &  20.20& $<$ 6.84 & 12.56 & \nodata & $<$ 250 & $<$ 280 &  710 &  2890 & \nodata & 	10 \nl	 
N5068 & 13 16 13 & -20 46 35 & 5 &  5.90& $<$ 6.37 & 10.09 & \nodata & $<$ 300 & $<$ 950 &  2340 &  17120 & \nodata & 	10 \nl	 
N5088 & 13 17 42 & -12 18 47 & 5 &  16.40& $<$ 2.21 & 12.33 & \nodata & $<$ 250 & $<$ 460 &  1770 &  4100 & \nodata & 	10 \nl	 
N5101 & 13 19 1 & -27 10 6 & 1 &  21.50& $<$ 5.90 & 11.21 & \nodata &  110 &  110 &  780 &  5600 & \nodata & 	6 \nl	 
N5135 & 13 22 56 & -29 34 17 & 3 &  51.50&  3.35 & 12.37 &  9.78 &  670 &  2480 &  16180 &  30830 &  58.8 & 	10,39,57 \nl	 
N5204 & 13 27 44 & 58 40 42 & 7 &  7.20&  9.58 & 11.48 &  10.15 & $<$ 250 & $<$ 290 &  2350 &  5360 & \nodata & 	10,45 \nl	 
N5194  \tablenotemark{e}& 13 27 46 & 47 27 17 & 4 &  8.40&  34.12 & 8.67 &  6.52 &  11020 &  17470 &  108680 &  292080 &  360 & 	1,8,33,45 \nl	 
N5236 & 13 34 10 & -29 36 47 & 5 &  4.50&  50.98 & 7.98 &  5.75 &  26280 &  47720 &  266030 &  638630 &  490 & 	8,26,45 \nl	 
N5248 & 13 35 3 & 9 8 30 & 4 &  14.00&  3.17 & 10.63 &  7.99 &  960 &  1490 &  17720 &  43970 &  77 & 	10,26,55 \nl	 
N5253 & 13 37 5 & -31 23 23 & 0 &  4.20&  2.17 & 10.47 &  8.78 &  2580 &  12210 &  30840 &  27490 &  65 & 	6,26,45 \nl	 
I4329A \tablenotemark{d} & 13 46 28 & -30 3 42 & 0 &  60.70&  494.50 & 13.67 &  9.97 &  1050 &  2250 &  2040 &  1620 & \nodata & 	1,10,57 \nl	 
N5313 & 13 47 37 & 40 14 0 & 3 &  34.50& $<$ 2.12 & 12.50 & \nodata & $<$ 340 &  250 &  3090 &  10530 & \nodata & 	10 \nl	 
N5326 & 13 48 42 & 39 49 12 & 1 &  34.00& $<$ 2.01 & 12.58 & \nodata & \nodata & \nodata & \nodata & \nodata & $<$ 20 & 	15,20 \nl	 
N5350 & 13 51 14 & 40 36 42 & 4 &  31.50& $<$ 3.30 & 11.99 & \nodata & $<$ 640 &  340 &  2250 &  8600 & \nodata & 	10 \nl	 
N5364 & 13 53 42 & 5 15 36 & 5 &  15.10& $<$ 7.59 & 10.79 & \nodata & $<$ 250 & $<$ 800 &  2070 &  11420 & \nodata & 	10 \nl	 
N5410 & 13 58 48 & 41 13 0 & 5 &  50.70& $<$ 3.62 & 13.53 &  12.32 & $<$ 270 & $<$ 250 &  790 &  1890 & \nodata & 	53 \nl	 
N5457 & 14 1 28 & 54 35 35 & 5 &  7.20&  19.35 & 8.21 &  6.35 &  6200 &  11780 &  88040 &  252840 &  150 & 	3,8,23,45 \nl	 
N5474 & 14 3 15 & 53 54 0 & 6 &  7.20& $<$ 1.74 & 11.30 &  11.09 & $<$ 250 & $<$ 250 &  1120 &  4780 & $<$ 3 & 	10,41,68 \nl	 
N5477 & 14 3 47 & 54 42 6 & 9 &  7.20& $<$ 2.13 & 14.20 & \nodata & $<$ 50.77 & $<$ 85.13 &  287 &  504 & $<$ 3 & 	41,17 \nl	 
N5506 \tablenotemark{d} & 14 10 38 & -2 58 30 & 1 &  22.40&  111.83 & 12.26 &  9.27 &  1300 &  4090 &  8790 &  8310 &  132 & 	6,28,57 \nl	 
N5548 \tablenotemark{d} & 14 15 43 & +25 22 0 & 1 &  68.60&  365.19 & 12.81 &  10.06 &  360 &  760 &  1040 &  1730 &  8 & 	10,32,64 \nl	 
N5566  \tablenotemark{e}& 14 17 49 & 4 9 41 & 1 &  18.80&  2.87 & 10.78 &  7.86 & $<$ 250 & $<$ 280 &  1070 &  5610 & \nodata & 	2,10,58 \nl	 
N5585 & 14 18 12 & 56 57 30 & 7 &  7.20& $<$ 3.16 & 11.05 &  9.97 & $<$ 250 & $<$ 250 &  850 &  3740 &  5.0 & 	10,41,45 \nl	 
N5645 & 14 28 10 & 7 29 47 & 5 &  17.20& $<$ 4.40 & 12.45 & \nodata & $<$ 340 & $<$ 250 &  2040 &  4720 & \nodata & 	10 \nl	 
N5643 & 14 29 28 & -43 57 12 & 5 &  12.70&  10.46 & 10.23 &  8.41 &  860 &  3350 &  18710 &  44190 &  64 & 	10,35,57 \nl	 
N5674 & 14 31 21 & 5 39 35 & 3 &  98.50&  2.52 & 13.57 & \nodata & $<$ 250 & $<$ 360 &  1500 &  3500 & \nodata & 	10 \nl	 
N5683 \tablenotemark{d} & 14 33 6 & 48 52 54 & 0 &  144.60&  49.62 & 14.98 &  12.58 & $<$ 250 & $<$ 250 &  470 &  1340 & \nodata & 	11,49 \nl	 
N5689 & 14 33 44 & 48 57 35 & 1 &  30.30& $<$ 3.56 & 12.03 & \nodata & $<$ 250 & $<$ 250 &  440 &  1420 & $<$ 100 & 	10,20 \nl	 
N5728 & 14 39 37 & -17 2 17 & 3 &  34.90&  5.46 & 11.65 &  9.19 & $<$ 320 &  810 &  8400 &  15170 &  4.6 & 	10,39,57 \nl	 
N5850  \tablenotemark{e}& 15 4 35 & 1 44 12 & 3 &  33.00&  0.91 & 11.39 & \nodata & $<$ 250 & $<$ 250 &  730 &  4430 & \nodata & 	10 \nl	 
N5879  \tablenotemark{e}& 15 8 29 & 57 11 23 & 3 &  12.40& $<$ 3.90 & 11.38 &  9.11 &  280 &  250 &  3350 &  9210 & \nodata & 	10,45 \nl	 
N5907 & 15 14 37 & 56 30 23 & 5 &  11.80& $<$ 2.99 & 9.70 &  7.35 &  1220 &  1350 &  8780 &  45760 &  30 & 	8,24,45 \nl	 
N5985  \tablenotemark{e}& 15 38 36 & 59 29 36 & 3 &  36.00& $<$ 8.49 & 11.38 & \nodata & $<$ 250 & $<$ 250 &  980 &  6200 & \nodata & 	10 \nl	 
N6052 & 16 3 1 & 20 40 30 & 5 &  63.50& $<$ 10.40 & 13.40 &  11.70 &  240 &  870 &  7040 &  10100 &  48 & 	10,24,48 \nl	 
N6300 & 17 12 18 & -62 45 47 & 3 &  12.00& $<$ 5.14 & 10.20 & \nodata &  740 &  2150 &  14050 &  40250 &  42 & 	10,26 \nl	 
N6454 \tablenotemark{d} & 17 44 0 & 55 43 0 & 5 &  125.30&  10.78 & 14.06 &  10.89 & $<$ 57 & $<$ 30 & $<$ 87 & $<$ 190 &  588 & 	59 \nl	 
N6503  \tablenotemark{e}& 17 49 58 & 70 9 30 & 5 &  5.20& $<$ 5.46 & 10.11 &  7.65 &  600 &  450 &  7160 &  25390 &  21 & 	10,42,45 \nl	 
N6744 & 19 5 2 & -63 56 17 & 4 &  8.90&  7.17 & 8.82 &  6.89 &  2860 &  4180 &  22210 &  85800 & \nodata & 	8,45 \nl	 
N6814 \tablenotemark{d} & 19 39 55 & -10 26 36 & 4 &  21.90&  27.72 & 11.32 &  8.65 &  330 &  590 &  5690 &  18160 &  2.2 & 	10,40,45 \nl	 
N6822 & 19 42 7 & -14 55 42 & 10 &  0.50&  8.56 & 8.38 & \nodata &  250 &  2460 &  47630 &  95420 &  72 & 	1,9,26 \nl	 
N6872 & 20 11 40 & -70 55 30 & 3 &  61.80&  8.66 & 11.49 & \nodata & $<$ 550 & $<$ 250 &  1570 &  7520 &  38 & 	10,26 \nl	 
N6890 & 20 14 50 & -44 57 24 & 2 &  32.10& $<$ 3.96 & 12.82 &  9.93 &  410 &  750 &  3710 &  8930 &  4.2 & 	10,39,58 \nl	 
N6946 & 20 33 48 & 59 59 0 & 5 &  5.50&  32.05 & 7.78 &  5.86 &  12130 &  21180 &  136690 &  344370 &  130 & 	8,19,45 \nl	 
N6951  \tablenotemark{e}& 20 36 37 & 65 55 54 & 3 &  22.80& $<$ 5.81 & 10.71 &  8.39 &  450 &  1170 &  13490 &  37140 &  36 & 	10,24,49 \nl	 
N6962 & 20 44 45 & 0 8 0 & 2 &  58.30& $<$ 3.03 & 12.43 & \nodata & $<$ 250 & $<$ 250 & $<$ 400 &  2020 & \nodata & 	10 \nl	 
I5063 & 20 48 12 & -57 15 11 & 0 &  43.50& $<$ 8.82 & 12.58 &  9.62 &  1220 &  3990 &  6530 &  3920 &  430.0 & 	6,20,57 \nl	 
N7213 \tablenotemark{d} & 22 6 12 & -47 25 0 & 1 &  23.20&  932.75 & 11.13 &  8.14 &  520 &  840 &  2570 &  8130 &  228.0 & 	6,20,57 \nl	 
N7314 & 22 33 0 & -26 18 30 & 5 &  19.80& $<$ 10.54 & 11.09 &  9.06 & $<$ 270 &  650 &  3390 &  14890 & \nodata & 	1,10,45 \nl	 
N7320 & 22 33 45 & 33 41 24 & 7 &  15.10&  8.64 & 12.55 &  11.06 & $<$ 250 & $<$ 290 &  640 &  3010 & \nodata & 	11,45 \nl	 
N7331  \tablenotemark{e}& 22 34 47 & 34 9 30 & 3 &  15.10&  8.81 & 9.38 &  6.08 &  3360 &  4200 &  35290 &  115070 &  94 & 	8,24,45 \nl	 
N7339 & 22 35 23 & 23 31 30 & 4 &  17.00& $<$ 6.74 & 12.09 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 	7 \nl	 
N7469 \tablenotemark{d} & 23 0 44 & 8 36 17 & 2 &  29.50&  390.08 & 12.64 &  9.72 &  1300 &  5480 &  26950 &  35220 &  78 & 	11,26,57 \nl	 
I5283 & 23 0 46 & 8 37 24 & 6 &  29.50& $<$ 2.22 & 14.34 &  11.59 & \nodata & \nodata & \nodata & \nodata & $<$ 33 & 	1,11,33,53 \nl	 
N7496 & 23 6 59 & -43 42 0 & 5 &  21.10& $<$ 4.45 & 11.84 &  9.71 &  270 &  1520 &  8550 &  15330 & \nodata & 	10,46 \nl	 
N7552 & 23 13 25 & -42 51 30 & 4 &  21.10&  8.74 & 11.13 &  8.39 &  2980 &  11960 &  72930 &  100890 &  140 & 	10,26,58 \nl	 
N7582 \tablenotemark{d} & 23 15 38 & -42 38 42 & 2 &  21.10&  11.09 & 10.83 &  8.32 &  1350 &  6330 &  48010 &  72760 &  110 & 	10,26,46 \nl	 
N7590 & 23 16 11 & -42 30 42 & 5 &  21.10&  2.83 & 11.46 &  9.28 &  520 &  840 &  7390 &  18020 & \nodata & 	10,57 \nl	 
N7599 & 23 16 36 & -42 31 47 & 5 &  21.10&  2.07 & 11.22 &  9.66 &  520 &  620 &  6130 &  18280 & \nodata & 	10,56 \nl	 
N7611 & 23 17 4 & 7 47 24 & 0 &  47.30& $<$ 3.85 & 13.44 &  10.12 & $<$ 105 & $<$ 170 & $<$ 140 & $<$ 735 & $<$ 1500 & 	6,21,62 \nl	 
N7673 & 23 25 12 & 23 18 54 & 5 &  48.90&  2.78 & 12.86 & \nodata & $<$ 250 &  500 &  5250 &  6980 & \nodata & 	10 \nl	 
N7677 & 23 25 36 & 23 15 18 & 4 &  50.80& $<$ 3.68 & 13.38 & \nodata &  280 &  750 &  3900 &  6140 & \nodata & 	10 \nl	 
N7679 & 23 26 14 & 3 14 11 & 5 &  71.20&  10.72 & 12.89 &  9.81 &  490 &  1080 &  7790 &  10500 & $<$ 60 & 	6,21,49 \nl	 
N7682 & 23 26 30 & 3 15 30 & 2 &  71.00& $<$ 11.82 & 13.67 & \nodata & \nodata & \nodata & \nodata & \nodata &  26 & 	16,34 \nl	 
N7714 & 23 33 40 & 1 52 42 & 3 &  39.90&  2.82 & 12.62 &  10.29 &  500 &  2800 &  11230 &  11290 &  22 & 	10,34,57 \nl	 
N7769 & 23 48 31 & 19 52 17 & 4 &  59.60& $<$ 3.09 & 12.59 &  9.98 & $<$ 410 &  590 &  4770 &  11580 & $<$ 27 & 	10,33,49 \nl	 
N7771 \tablenotemark{d} & 23 48 52 & 19 50 0 & 1 &  60.60&  7.24 & 12.50 &  9.77 &  680 &  1720 &  18150 &  38780 &  47 & 	11,25,53 \nl	 
N7793 & 23 55 15 & -32 52 5 & 7 &  4.00&  6.81 & 9.37 &  7.82 &  1540 &  2090 &  19620 &  56340 & \nodata & 	8,45 \nl	 

\tablenotetext{a} {The values listed as upper limits are 3$\sigma$.}
\tablenotetext{b} {References are given in Table 2. }
\tablenotetext{c} {NGC 224,SMC,NGC 598,LMC,NGC 3034,NGC 253, NGC 1068 {\it IRAS} data in Janskys.  All other {\it IRAS} data in milliJanskys}
\tablenotetext{d} {Galaxies known as AGN, and excluded from the statistical analysis.}
\tablenotetext{e} {Galaxies exhibiting evidence
for some kind of non-stellar ionizing continuum giving rise to
nuclear emission, but at a lower level than those flagged with 
``d'' (Ho et al. 1997). These galaxies were included in the statictical analysis.}

\enddata
\end{deluxetable}



==> table10.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.


\begin{deluxetable}{lccrrc}
\tablenum{10}
\small
\tablewidth{0pc}
\tablecaption{Distances }
\tablehead{
\colhead{Galaxy} & \colhead{Dist. Mod.} &
\colhead{Distance} & 
\colhead{$V_0$}  &  \colhead{$V_{yts}$} & \colhead{D($H_0 = 75$)}
\\
\colhead{} &\colhead{from lit.} &
\colhead{(Mpc)} &
\colhead{(km/s)}
& \colhead{(km/s)} &
\colhead{(Mpc)} \\
}

\startdata
N0125 & \nodata & \nodata & 5306 & 5491.2 & 73.2 \nl
N0224 & 24.44 & 0.77 & -300 & -13.2 & \nodata \nl
N0247 & 27.40 & 3.0 & 159 & 228.7 & \nodata \nl
N0253 & 27.45 & 3.1 & 251 & 297.8 & \nodata \nl
SMC & 18.90 & 0.060 & 175 & -8.6 & \nodata \nl
N0309 & \nodata & \nodata & 5662 & 5780.4 & 77.1 \nl
I1613 & 24.42 & 0.76 & -230 & -62.0 & \nodata \nl
N0449 & \nodata & \nodata & 4824 & 5085.5 & 67.8 \nl
N0520 & 32.88 & 37.8 & 2217 & 2382.3 & \nodata \nl
N0521 & \nodata & \nodata & 5040 & 5196.8 & 69.3 \nl
N0523 & \nodata & \nodata & 4750 & 5009.6 & 66.8 \nl
N0524 & \nodata & \nodata & 2421 & 2608.6 & 34.8 \nl
N0578 & \nodata & \nodata & 1630 & 1671.6 & 22.3 \nl
N0598 & 24.63 & 0.84 & -179 & 69.3 & \nodata \nl
N0625 & 28.46 & 4.9 & 386 & 333.2 & \nodata \nl
N0628 & 29.32 & 7.3 & 656 & 859.8 & \nodata \nl
I1727 & \nodata & \nodata & 338 & 571.3 & 7.6 \nl
N0672 & 29.50 & 7.9 & 421 & 654.4 & \nodata \nl
N0772 & 32.58 & 32.8 & 2458 & 2660.1 & \nodata \nl
N0871 & \nodata & \nodata & 3736 & 3912.1 & 52.2 \nl
N0877 & \nodata & \nodata & 3913 & 4088.6 & 54.5 \nl
N0936 & \nodata & \nodata & 1340 & 1447.1 & 19.3 \nl
N0941 & \nodata & \nodata & 1608 & 1714.6 & 22.9 \nl
N0945 & \nodata & \nodata & 4484 & 4549.1 & 60.7 \nl
N0985 & \nodata & \nodata & 12929 & 12997.9 & 173.3 \nl
N1042 & \nodata & \nodata & 1373 & 1439.6 & 19.2 \nl
N1068 & \nodata & \nodata & 1137 & 1238.7 & 16.5 \nl
N1073 & \nodata & \nodata & 1211 & 1317.8 & 17.6 \nl
N1087 & \nodata & \nodata & 1519 & 1616.0 & 21.5 \nl
N1090 & \nodata & \nodata & 2758 & 2855.9 & 38.1 \nl
N1097 & \nodata & \nodata & 1275 & 1238.2 & 16.5 \nl
N1218 & \nodata & \nodata & 8644 & 8744.3 & 116.6 \nl
N1300 & \nodata & \nodata & 1568 & 1557.6 & 20.8 \nl
N1313 & 28.27 & 4.5 & 457 & 264.4 & \nodata \nl
N1317 & 31.32 & 18.4 & 1941 & 1852.1 & \nodata \nl
N1350 & 31.32 & 18.4 & 1890 & 1810.2 & \nodata \nl
N1358 & \nodata & \nodata & 4013 & 4055.0 & 54.1 \nl
N1365 & 31.32 & 18.4 & 1662 & 1570.3 & \nodata \nl
N1380 & 31.00 & 15.8 & 1841 & 1752.2 & \nodata \nl
N1386 & 31.32 & 18.4 & 864 & 770.9 & \nodata \nl
N1398 & \nodata & \nodata & 1407 & 1352.7 & 18.0 \nl
N1421 & \nodata & \nodata & 2090 & 2088.6 & 27.8 \nl
I0342 & 27.78 & 3.6 & 34 & 279.3 & \nodata \nl
N1512 & \nodata & \nodata & 901 & 763.1 & 10.2 \nl
N1533 & \nodata & \nodata & 1342 & 1159.7 & 15.5 \nl
N1559 & 31.02 & 16.0 & 1292 & 1089.0 & \nodata \nl
N1566 & \nodata & \nodata & 1342 & 1159.7 & 15.5 \nl
N1569 & 26.15 & 1.7 & -89 & 138.4 & \nodata \nl
N1614 & \nodata & \nodata & 4778 & 4756.6 & 63.4 \nl
N1625 & \nodata & \nodata & 4700 & 4698.4 & 62.6 \nl
N1672 & \nodata & \nodata & 1350 & 1143.9 & 15.3 \nl
N1784 & \nodata & \nodata & 2316 & 2255.2 & 30.1 \nl
LMC & 18.50 & 0.050 & 324 & 87.1 & \nodata \nl
N1961 & 34.39 & 75.4 & 3930 & 4142.9 & \nodata \nl
U3691 & \nodata & \nodata & 2203 & 2164.0 & 28.9 \nl
N2276 & 31.16 & 17.1 & 2417 & 2650.4 & \nodata \nl
N2366 & 27.68 & 3.4 & 100 & 284.5 & \nodata \nl
N2403 & 27.51 & 3.2 & 131 & 300.5 & \nodata \nl
N2441 & 33.76 & 56.5 & 3470 & 3663.1 & \nodata \nl
N2525 & \nodata & \nodata & 1581 & 1393.5 & 18.6 \nl
N2608 & \nodata & \nodata & 2135 & 2112.6 & 28.2 \nl
N2642 & \nodata & \nodata & 4342 & 4165.2 & 55.5 \nl
N2683 & \nodata & \nodata & 410 & 406.2 & 5.4 \nl
N2763 & \nodata & \nodata & 1893 & 1663.9 & 22.2 \nl
N2773 & \nodata & \nodata & 5406 & 5266.2 & 70.2 \nl
N2775 & \nodata & \nodata & 1421 & 1280.4 & 17.1 \nl
N2777 & \nodata & \nodata & 1421 & 1280.4 & 17.1 \nl
N2782 & \nodata & \nodata & 2562 & 2586.2 & 34.5 \nl
N2835 & \nodata & \nodata & 888 & 634.4 & 8.5 \nl
N2841 & 31.98 & 24.9 & 638 & 716.1 & \nodata \nl
N2848 & \nodata & \nodata & 2044 & 1807.1 & 24.1 \nl
N2903 & \nodata & \nodata & 556 & 478.8 & 6.4 \nl
N2914 & \nodata & \nodata & 3151 & 3017.2 & 40.2 \nl
N2992 & \nodata & \nodata & 2367 & 2130.4 & 28.4 \nl
N2993 & \nodata & \nodata & 2367 & 2130.4 & 28.4 \nl
N3031 & 27.80 & 3.6 & -34 & 127.0 & \nodata \nl
N3034 & 27.80 & 3.6 & 203 & 366.7 & \nodata \nl
N3067 & \nodata & \nodata & 1476 & 1449.9 & 19.3 \nl
N3066 & \nodata & \nodata & 2049 & 2223.2 & 29.6 \nl
N3077 & 27.80 & 3.6 & 14 & 173.0 & \nodata \nl
N3079 & 31.44 & 19.4 & 1125 & 1221.0 & \nodata \nl
N3081 & \nodata & \nodata & 2367 & 2102.1 & 28.0 \nl
N3125 & \nodata & \nodata & 1080 & 797.3 & 10.6 \nl
N3166 & 29.72 & 8.8 & 1345 & 1172.4 & \nodata \nl
N3169 & 29.72 & 8.8 & 1233 & 1060.5 & \nodata \nl
N3175 & \nodata & \nodata & 1111 & 829.4 & 11.1 \nl
N3184 & 29.30 & 7.2 & 593 & 612.7 & \nodata \nl
N3227 & \nodata & \nodata & 1157 & 1062.1 & 14.2 \nl
I2574 & 27.80 & 3.6 & 47 & 203.3 & \nodata \nl
N3281 & \nodata & \nodata & 3439 & 3144.8 & 41.9 \nl
N3310 & \nodata & \nodata & 980 & 1062.4 & 14.2 \nl
N3346 & \nodata & \nodata & 1260 & 1138.7 & 15.2 \nl
N3351 & 30.01 & 10.1 & 778 & 641.2 & \nodata \nl
N3353 & \nodata & \nodata & 944 & 1038.9 & 13.9 \nl
N3368 & 30.27 & 11.3 & 897 & 760.7 & \nodata \nl
N3389 & 32.38 & 29.9 & 1301 & 1168.1 & \nodata \nl
N3395 & \nodata & \nodata & 1620 & 1592.8 & 21.2 \nl
N3430 & \nodata & \nodata & 1585 & 1557.6 & 20.8 \nl
N3445 & \nodata & \nodata & 2023 & 2123.1 & 28.3 \nl
N3448 & \nodata & \nodata & 1350 & 1436.4 & 19.2 \nl
N3455 & \nodata & \nodata & 1107 & 997.7 & 13.3 \nl
N3489 & 30.32 & 11.6 & 708 & 581.9 & \nodata \nl
N3504 & \nodata & \nodata & 1539 & 1485.2 & 19.8 \nl
N3512 & \nodata & \nodata & 1376 & 1322.6 & 17.6 \nl
N3593 & \nodata & \nodata & 628 & 497.4 & 6.6 \nl
N3628 & 30.37 & 11.9 & 847 & 720.7 & \nodata \nl
N3660 & \nodata & \nodata & 3678 & 3455.2 & 46.1 \nl
N3690 & \nodata & \nodata & 3132 & 3241.4 & 43.2 \nl
N3718 & \nodata & \nodata & 994 & 1075.7 & 14.3 \nl
N3729 & 30.95 & 15.5 & 1024 & 1106.1 & \nodata \nl
N3783 & \nodata & \nodata & 2926 & 2630.1 & 35.1 \nl
N3884 & \nodata & \nodata & 6948 & 6859.4 & 91.5 \nl
N3887 & \nodata & \nodata & 1209 & 961.8 & 12.8 \nl
N3888 & \nodata & \nodata & 2408 & 2506.0 & 33.4 \nl
N3893 & 30.95 & 15.5 & 973 & 1033.9 & \nodata \nl
N3896 & 30.95 & 15.5 & 869 & 929.7 & \nodata \nl
N3991 & \nodata & \nodata & 3192 & 3167.8 & 42.1 \nl
N3994 & \nodata & \nodata & 3096 & 3071.5 & 42.1 \nl
N3995 & \nodata & \nodata & 3254 & 3229.6 & 42.1 \nl
I0749 & 30.95 & 15.5 & 784 & 815.0 & \nodata \nl
I0750 & 30.95 & 15.5 & 703 & 734.0 & \nodata \nl
N4036 & \nodata & \nodata & 1397 & 1525.8 & 20.3 \nl
N4038 & 31.83 & 23.3 & 1624 & 1373.8 & \nodata \nl
N4041 & \nodata & \nodata & 1234 & 1364.0 & 18.2 \nl
N4051 & 30.95 & 15.5 & 725 & 766.3 & \nodata \nl
N4151 & \nodata & \nodata & 995 & 1010.8 & 13.5 \nl
N4156 & \nodata & \nodata & 6750 & 6766.2 & 90.2 \nl
N4178 & 30.51 & 12.6 & 378 & 248.5 & \nodata \nl
N4190 & 27.75 & 3.5 & 230 & 232.0 & \nodata \nl
N4192 & 30.80 & 14.5 & -142 & -251.7 & \nodata \nl
N4206 & 31.48 & 19.7 & 702 & 583.6 & \nodata \nl
N4212 & 31.36 & 18.7 & -81 & -195.0 & \nodata \nl
N4214 & 28.06 & 4.1 & 291 & 291.8 & \nodata \nl
N4216 & 31.13 & 16.8 & 131 & 13.4 & \nodata \nl
N4224 & 33.30 & 45.7 & 2603 & 2458.7 & \nodata \nl
N4235 & 31.48 & 19.8 & 2410 & 2264.6 & \nodata \nl
N4236 & 27.80 & 3.6 & -5 & 160.3 & \nodata \nl
N4244 & 28.28 & 4.5 & 243 & 252.0 & \nodata \nl
N4245 & \nodata & \nodata & 890 & 856.1 & 11.4 \nl
N4246 & 32.83 & 36.8 & 3725 & 3579.9 & \nodata \nl
N4254 & 30.56 & 12.9 & 2407 & 2296.4 & \nodata \nl
N4258 & 29.29 & 7.2 & 448 & 506.8 & \nodata \nl
N4260 & 33.14 & 42.4 & 1958 & 1808.3 & \nodata \nl
N4298 & 31.03 & 16.1 & 1141 & 1032.1 & \nodata \nl
N4303 & 30.12 & 10.6 & 1569 & 1412.8 & \nodata \nl
N4321 & 31.04 & 16.1 & 1586 & 1483.5 & \nodata \nl
N4351 & 30.16 & 12.9 & 2310 & 2190.3 & \nodata \nl
N4378 & 33.45 & 49.1 & 2551 & 2397.9 & \nodata \nl
N4385 & \nodata & \nodata & 2140 & 1968.0 & 26.2 \nl
N4388 & 31.11 & 16.7 & 2517 & 2400.0 & \nodata \nl
N4394 & 31.93 & 24.3 & 922 & 832.3 & \nodata \nl
N4424 & 28.00 & 4.0 & 439 & 307.1 & \nodata \nl
N4429 & 30.57 & 13.0 & 1137 & 1013.2 & \nodata \nl
N4438 & 30.45 & 12.3 & 69 & -45.6 & \nodata \nl
N4449 & 27.33 & 2.9 & 201 & 245.3 & \nodata \nl
N4450 & 30.77 & 14.2 & 1956 & 1861.5 & \nodata \nl
N4461 & 30.40 & 12.0 & 1918 & 1804.6 & \nodata \nl
N4464 & 31.32 & 18.4 & 1255 & 1118.0 & \nodata \nl
N4477 & 31.08 & 16.4 & 1353 & 1242.1 & \nodata \nl
N4501 & 31.20 & 17.4 & 2280 & 2173.6 & \nodata \nl
N4503 & 30.35 & 11.7 & 1364 & 1242.1 & \nodata \nl
N4522 & 31.06 & 16.3 & 2324 & 2193.2 & \nodata \nl
N4527 & 30.68 & 13.7 & 1734 & 1573.9 & \nodata \nl
N4535 & 30.47 & 12.4 & 1957 & 1821.9 & \nodata \nl
N4536 & 31.10 & 16.6 & 1804 & 1641.9 & \nodata \nl
I3528 & \nodata & \nodata & 13764 & 13664.2 & 182.2 \nl
N4548 & 30.81 & 14.5 & 486 & 381.2 & \nodata \nl
N4565 & 30.13 & 10.6 & 1227 & 1179.9 & \nodata \nl
N4567 & 31.74 & 22.3 & 2268 & 2148.0 & \nodata \nl
N4569 & 29.77 & 9.0 & -235 & -345.8 & \nodata \nl
N4571 & 30.87 & 14.9 & 342 & 236.3 & \nodata \nl
N4579 & 31.51 & 20.0 & 1519 & 1402.1 & \nodata \nl
N4594 & 29.86 & 9.4 & 1091 & 876.1 & \nodata \nl
N4603 & \nodata & \nodata & 2562 & 2275.1 & 30.3 \nl
N4631 & 27.69 & 3.5 & 606 & 594.5 & \nodata \nl
N4639 & 32.00 & 25.1 & 1010 & 901.9 & \nodata \nl
N4643 & 31.02 & 16.0 & 1399 & 1239.3 & \nodata \nl
N4647 & 31.48 & 19.8 & 1415 & 1299.1 & \nodata \nl
N4651 & 31.57 & 20.7 & 805 & 712.4 & \nodata \nl
N4654 & 30.56 & 13.0 & 1035 & 926.6 & \nodata \nl
N4665 & 31.02 & 16.0 & 785 & 630.7 & \nodata \nl
N4689 & 30.75 & 14.1 & 1619 & 1515.2 & \nodata \nl
N4698 & 32.80 & 36.3 & 999 & 870.5 & \nodata \nl
N4736 & 28.85 & 5.9 & 310 & 345.4 & \nodata \nl
N4826 & \nodata & \nodata & 408 & 346.6 & 4.6 \nl
N4845 & 32.42 & 30.5 & 1232 & 1076.6 & \nodata \nl
N4861 & \nodata & \nodata & 846 & 852.2 & 11.4 \nl
I4182 & 28.36 & 4.7 & 321 & 343.5 & \nodata \nl
N5033 & \nodata & \nodata & 878 & 898.3 & 12.0 \nl
N5037 & 31.52 & 20.2 & 1904 & 1686.7 & \nodata \nl
N5068 & \nodata & \nodata & 672 & 442.5 & 5.9 \nl
N5079 & \nodata & \nodata & 2870 & 2668.3 & 35.6 \nl
N5088 & \nodata & \nodata & 1434 & 1233.1 & 16.4 \nl
N5101 & \nodata & \nodata & 1861 & 1615.1 & 21.5 \nl
N5135 & \nodata & \nodata & 4112 & 3861.9 & 51.5 \nl
N5194 & 29.62 & 8.4 & 463 & 541.5 & \nodata \nl
N5204 & 29.28 & 7.2 & 204 & 334.0 & \nodata \nl
N5236 & 28.27 & 4.5 & 516 & 271.1 & \nodata \nl
N5248 & \nodata & \nodata & 1153 & 1049.6 & 14.0 \nl
N5253 & 28.10 & 4.2 & 404 & 156.2 & \nodata \nl
I4329A & \nodata & \nodata & 4793 & 4553.0 & 60.7 \nl
N5313 & \nodata & \nodata & 2538 & 2590.1 & 34.5 \nl
N5326 & \nodata & \nodata & 2501 & 2551.6 & 34.0 \nl
N5350 & \nodata & \nodata & 2304 & 2359.5 & 31.5 \nl
N5364 & \nodata & \nodata & 1241 & 1130.8 & 15.1 \nl
N5410 & \nodata & \nodata & 3738 & 3799.8 & 50.7 \nl
N5457 & 29.28 & 7.2 & 241 & 363.9 & \nodata \nl
N5474 & 29.28 & 7.2 & 277 & 397.7 & \nodata \nl
N5477 & 29.28 & 7.2 & 304 & 428.3 & \nodata \nl
N5506 & \nodata & \nodata & 1815 & 1680.1 & 22.4 \nl
N5548 & \nodata & \nodata & 5149 & 5145.0 & 68.6 \nl
N5566 & \nodata & \nodata & 1507 & 1407.1 & 18.8 \nl
N5585 & 29.28 & 7.2 & 305 & 443.8 & \nodata \nl
N5643 & \nodata & \nodata & 1199 & 951.8 & 12.7 \nl
N5645 & \nodata & \nodata & 1367 & 1288.6 & 17.2 \nl
N5674 & \nodata & \nodata & 7472 & 7387.8 & 98.5 \nl
N5683 & \nodata & \nodata & 10732 & 10843.6 & 144.6 \nl
N5689 & \nodata & \nodata & 2160 & 2272.2 & 30.3 \nl
N5728 & \nodata & \nodata & 2788 & 2618.6 & 34.9 \nl
N5850 & \nodata & \nodata & 2556 & 2478.6 & 33.0 \nl
N5879 & \nodata & \nodata & 772 & 931.0 & 12.4 \nl
N5907 & 30.36 & 11.8 & 667 & 826.2 & \nodata \nl
N5985 & \nodata & \nodata & 2520 & 2698.8 & 36.0 \nl
N6052 & \nodata & \nodata & 4716 & 4765.1 & 63.5 \nl
N6300 & \nodata & \nodata & 1110 & 903.3 & 12.0 \nl
N6454 & \nodata & \nodata & 9169 & 9394.2 & 125.3 \nl
N6503 & 28.58 & 5.2 & 44 & 288.5 & \nodata \nl
N6744 & \nodata & \nodata & 841 & 670.3 & 8.9 \nl
N6814 & \nodata & \nodata & 1563 & 1646.2 & 21.9 \nl
N6822 & 23.50 & 0.50 & -56 & 7.8 & \nodata \nl
N6872 & \nodata & \nodata & 4818 & 4637.5 & 61.8 \nl
N6890 & \nodata & \nodata & 2471 & 2405.5 & 32.1 \nl
N6946 & 28.71 & 5.5 & 52 & 340.9 & \nodata \nl
N6951 & \nodata & \nodata & 1426 & 1712.2 & 22.8 \nl
N6962 & \nodata & \nodata & 4211 & 4375.0 & 58.3 \nl
I5063 & \nodata & \nodata & 3380 & 3265.6 & 43.5 \nl
N7213 & \nodata & \nodata & 1792 & 1740.9 & 23.2 \nl
N7314 & \nodata & \nodata & 1422 & 1485.7 & 19.8 \nl
N7320 & 30.89 & 15.1 & 776 & 1069.0 & \nodata \nl
N7331 & 30.89 & 15.1 & 821 & 1114.8 & \nodata \nl
N7339 & 31.15 & 17.0 & 1346 & 1617.6 & \nodata \nl
N7469 & 32.35 & 29.5 & 4916 & 5141.1 & \nodata \nl
I5283 & 32.35 & 29.5 & 4894 & 5119.2 & \nodata \nl
N7496 & \nodata & \nodata & 1612 & 1582.7 & 21.1 \nl
N7552 & \nodata & \nodata & 1612 & 1582.7 & 21.1 \nl
N7582 & \nodata & \nodata & 1612 & 1582.7 & 21.1 \nl
N7590 & \nodata & \nodata & 1612 & 1582.7 & 21.1 \nl
N7599 & \nodata & \nodata & 1612 & 1582.7 & 21.1 \nl
N7611 & \nodata & \nodata & 3330 & 3551.0 & 47.3 \nl
N7673 & \nodata & \nodata & 3401 & 3670.3 & 48.9 \nl
N7677 & \nodata & \nodata & 3539 & 3808.1 & 50.8 \nl
N7679 & \nodata & \nodata & 5138 & 5340.2 & 71.2 \nl
N7682 & \nodata & \nodata & 5120 & 5322.3 & 71.0 \nl
N7714 & \nodata & \nodata & 2799 & 2994.6 & 39.9 \nl
N7769 & \nodata & \nodata & 4214 & 4470.3 & 59.6 \nl
N7771 & \nodata & \nodata & 4287 & 4543.1 & 60.6 \nl
N7793 & 28.03 & 4.0 & 230 & 252.8 & \nodata \nl
\enddata
\end{deluxetable}



==> table11a.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{llrrr|llrrr}
\small
\tablenum{11A}
\tablewidth{0pc}
\tablecaption{Spearman Partial Rank Analysis on the Total Sample ($N = 94$)}
\tablehead{
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  &
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  &
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  \\
}
\startdata

 B , X &  D & 0.451& 4.823 & $<$ 0.005  & 6cm, X &  D & 0.458& 4.919 & $<$ 0.005 \nl
  &  6cm, D  & 0.338 & 3.413 & $<$ 0.005   &   &   H , D  & 0.423 & 4.429 & $<$ 0.005 \nl 
  &   H , D  &0.172 & 1.658 &0.053   &   &   B , D  & 0.349 & 3.533 & $<$ 0.005 \nl 
  &  FIR, D  & 0.302 & 3.005 & $<$ 0.005   &   &  FIR, D  &0.235 & 2.294 &0.014 \nl 
  &   12, D  &0.266 & 2.623 &0.006   &   &   12, D  &0.194 & 1.881 &0.035 \nl 
  &  6cm, H , D  & 0.002 & 0.016 & $>$ 0.400   &   &   H , B , D  & 0.392 & 4.024 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.323 & 3.225 & $<$ 0.005   &   &   H ,FIR, D  & 0.273 & 2.675 & 0.005 \nl 
  &  6cm, 12, D  & 0.286 & 2.814 & $<$ 0.005   &   &   H , 12, D  & 0.259 & 2.534 & 0.008 \nl 
  &   H ,FIR, D  & -0.010 & -0.096 & $>$ 0.400   &   &   B ,FIR, D  & 0.263 & 2.573 & 0.007 \nl 
  &   H , 12, D  & 0.014 & 0.127 & $>$ 0.400   &   &   B , 12, D  & 0.221 & 2.138 & 0.020 \nl 
  &  FIR, 12, D  & 0.264 & 2.581 & 0.007   &   &  FIR, 12, D  & 0.193 & 1.859 & 0.036 \nl 
  &  6cm, H ,FIR, D  & -0.007 & -0.065 & $>$ 0.400   &   &   H , B ,FIR, D  & 0.273 & 2.659 & 0.005 \nl 
  &  6cm, H , 12, D  & -0.014 & -0.133 & $>$ 0.400   &   &   H , B , 12, D  & 0.259 & 2.520 & 0.008 \nl 
  &  6cm,FIR, 12, D  & 0.294 & 2.881 & $<$ 0.005   &   &   H ,FIR, 12, D  & 0.250 & 2.419 & 0.010 \nl 
  &   H ,FIR, 12, D  & -0.011 & -0.100 & $>$ 0.400   &   &   B ,FIR, 12, D  & 0.234 & 2.253 & 0.016 \nl 
 H , X &  D & 0.436& 4.621 & $<$ 0.005  &  H , B &  D & 0.845& 15.059 & $<$ 0.005 \nl
  &  6cm, D  & 0.398 & 4.113 & $<$ 0.005   &   &  6cm, D  & 0.849 & 15.240 & $<$ 0.005 \nl 
  &   B , D  &0.115 & 1.096 &0.149   &   &   X , D  & 0.807 & 12.959 & $<$ 0.005 \nl 
  &  FIR, D  & 0.362 & 3.681 & $<$ 0.005   &   &  FIR, D  & 0.848 & 15.211 & $<$ 0.005 \nl 
  &   12, D  & 0.316 & 3.155 & $<$ 0.005   &   &   12, D  & 0.821 & 13.656 & $<$ 0.005 \nl 
  &  6cm, B , D  & 0.222 & 2.148 & 0.020   &   &  6cm, X , D  & 0.827 & 13.899 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.385 & 3.940 & $<$ 0.005   &   &  6cm,FIR, D  & 0.848 & 15.100 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.357 & 3.601 & $<$ 0.005   &   &  6cm, 12, D  & 0.823 & 13.644 & $<$ 0.005 \nl 
  &   B ,FIR, D  & 0.209 & 2.019 & 0.025   &   &   X ,FIR, D  & 0.832 & 14.137 & $<$ 0.005 \nl 
  &   B , 12, D  & 0.176 & 1.686 & 0.050   &   &   X , 12, D  & 0.806 & 12.847 & $<$ 0.005 \nl 
  &  FIR, 12, D  & 0.321 & 3.201 & $<$ 0.005   &   &  FIR, 12, D  & 0.838 & 14.510 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & 0.221 & 2.130 & 0.020   &   &  6cm, X ,FIR, D  & 0.829 & 13.881 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & 0.223 & 2.146 & 0.020   &   &  6cm, X , 12, D  & 0.805 & 12.724 & $<$ 0.005 \nl 
  &  6cm,FIR, 12, D  & 0.356 & 3.570 & $<$ 0.005   &   &  6cm,FIR, 12, D  & 0.836 & 14.294 & $<$ 0.005 \nl 
  &   B ,FIR, 12, D  & 0.190 & 1.819 & 0.039   &   &   X ,FIR, 12, D  & 0.825 & 13.696 & $<$ 0.005 \nl 
 X , 12&  D & 0.459& 4.932 & $<$ 0.005  &  B , 12&  D & 0.553& 6.329 & $<$ 0.005 \nl
  &  6cm, D  &0.197 & 1.909 &0.033   &   &  6cm, D  & 0.441 & 4.667 & $<$ 0.005 \nl 
  &   H , D  & 0.350 & 3.550 & $<$ 0.005   &   &   H , D  & 0.459 & 4.902 & $<$ 0.005 \nl 
  &   B , D  & 0.282 & 2.791 & $<$ 0.005   &   &   X , D  & 0.436 & 4.596 & $<$ 0.005 \nl 
  &  FIR, D  &0.216 & 2.100 &0.022   &   &  FIR, D  &0.240 & 2.342 &0.012 \nl 
  &  6cm, H , D  & 0.059 & 0.557 & 0.291   &   &  6cm, H , D  & 0.260 & 2.538 & 0.008 \nl 
  &  6cm, B , D  & 0.057 & 0.535 & 0.298   &   &  6cm, X , D  & 0.406 & 4.193 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.169 & 1.622 & 0.058   &   &  6cm,FIR, D  & 0.260 & 2.538 & 0.008 \nl 
  &   H , B , D  & 0.310 & 3.078 & $<$ 0.005   &   &   H , X , D  & 0.432 & 4.522 & $<$ 0.005 \nl 
  &   H ,FIR, D  & 0.128 & 1.219 & 0.120   &   &   H ,FIR, D  & 0.003 & 0.031 & $>$ 0.400 \nl 
  &   B ,FIR, D  & 0.155 & 1.483 & 0.076   &   &   X ,FIR, D  & 0.187 & 1.800 & 0.041 \nl 
  &  6cm, H , B , D  & 0.061 & 0.569 & 0.287   &   &  6cm, H , X , D  & 0.260 & 2.527 & 0.008 \nl 
  &  6cm, H ,FIR, D  & 0.060 & 0.566 & 0.288   &   &  6cm, H ,FIR, D  & 0.007 & 0.065 & $>$ 0.400 \nl 
  &  6cm, B ,FIR, D  & 0.093 & 0.880 & 0.202   &   &  6cm, X ,FIR, D  & 0.220 & 2.114 & 0.021 \nl 
  &   H , B ,FIR, D  & 0.128 & 1.212 & 0.121   &   &   H , X ,FIR, D  & 0.005 & 0.043 & $>$ 0.400 \nl 
 X ,FIR&  D & 0.417& 4.374 & $<$ 0.005  &  B ,FIR&  D & 0.520& 5.807 & $<$ 0.005 \nl
  &  6cm, D  &0.109 & 1.038 &0.163   &   &  6cm, D  & 0.390 & 4.022 & $<$ 0.005 \nl 
  &   H , D  & 0.337 & 3.392 & $<$ 0.005   &   &   H , D  & 0.535 & 6.012 & $<$ 0.005 \nl 
  &   B , D  &0.239 & 2.335 &0.012   &   &   X , D  & 0.409 & 4.254 & $<$ 0.005 \nl 
  &   12, D  &0.042 & 0.400 &0.346   &   &   12, D  &0.098 & 0.935 &0.188 \nl 
  &  6cm, H , D  & 0.021 & 0.197 & $>$ 0.400   &   &  6cm, H , D  & 0.385 & 3.930 & $<$ 0.005 \nl 
  &  6cm, B , D  & -0.027 & -0.254 & 0.399   &   &  6cm, X , D  & 0.378 & 3.851 & $<$ 0.005 \nl 
  &  6cm, 12, D  & -0.036 & -0.344 & 0.366   &   &  6cm, 12, D  & 0.135 & 1.286 & 0.103 \nl 
  &   H , B , D  & 0.294 & 2.901 & $<$ 0.005   &   &   H , X , D  & 0.515 & 5.662 & $<$ 0.005 \nl 
  &   H , 12, D  & 0.076 & 0.722 & 0.240   &   &   H , 12, D  & 0.310 & 3.074 & $<$ 0.005 \nl 
  &   B , 12, D  & 0.017 & 0.157 & $>$ 0.400   &   &   X , 12, D  & 0.090 & 0.854 & 0.208 \nl 
  &  6cm, H , B , D  & 0.022 & 0.206 & $>$ 0.400   &   &  6cm, H , X , D  & 0.385 & 3.908 & $<$ 0.005 \nl 
  &  6cm, H , 12, D  & -0.024 & -0.228 & $>$ 0.400   &   &  6cm, H , 12, D  & 0.294 & 2.882 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & -0.079 & -0.744 & 0.234   &   &  6cm, X , 12, D  & 0.152 & 1.442 & 0.081 \nl 
  &   H , B , 12, D  & 0.076 & 0.714 & 0.242   &   &   H , X , 12, D  & 0.310 & 3.056 & $<$ 0.005 \nl 
\tablebreak 
6cm, B &  D & 0.376& 3.874 & $<$ 0.005  & FIR, 12&  D & 0.867& 16.593 & $<$ 0.005 \nl
  &   H , D  & 0.404 & 4.184 & $<$ 0.005   &   &  6cm, D  & 0.684 & 8.892 & $<$ 0.005 \nl 
  &   X , D  &0.214 & 2.075 &0.023   &   &   H , D  & 0.855 & 15.640 & $<$ 0.005 \nl 
  &  FIR, D  &-0.051 & -0.487 &0.315   &   &   B , D  & 0.814 & 13.300 & $<$ 0.005 \nl 
  &   12, D  &-0.068 & -0.646 &0.261   &   &   X , D  & 0.837 & 14.487 & $<$ 0.005 \nl 
  &   H , X , D  & 0.371 & 3.763 & $<$ 0.005   &   &  6cm, H , D  & 0.663 & 8.357 & $<$ 0.005 \nl 
  &   H ,FIR, D  & -0.013 & -0.124 & $>$ 0.400   &   &  6cm, B , D  & 0.619 & 7.440 & $<$ 0.005 \nl 
  &   H , 12, D  & 0.104 & 0.990 & 0.175   &   &  6cm, X , D  & 0.680 & 8.742 & $<$ 0.005 \nl 
  &   X ,FIR, D  & -0.132 & -1.255 & 0.111   &   &   H , B , D  & 0.812 & 13.121 & $<$ 0.005 \nl 
  &   X , 12, D  & -0.127 & -1.204 & 0.123   &   &   H , X , D  & 0.836 & 14.356 & $<$ 0.005 \nl 
  &  FIR, 12, D  & -0.115 & -1.094 & 0.150   &   &   B , X , D  & 0.802 & 12.646 & $<$ 0.005 \nl 
  &   H , X ,FIR, D  & -0.011 & -0.101 & $>$ 0.400   &   &  6cm, H , B , D  & 0.632 & 7.646 & $<$ 0.005 \nl 
  &   H , X , 12, D  & 0.104 & 0.985 & 0.176   &   &  6cm, H , X , D  & 0.663 & 8.311 & $<$ 0.005 \nl 
  &   H ,FIR, 12, D  & -0.014 & -0.136 & $>$ 0.400   &   &  6cm, B , X , D  & 0.622 & 7.451 & $<$ 0.005 \nl 
  &   X ,FIR, 12, D  & -0.176 & -1.674 & 0.051   &   &   H , B , X , D  & 0.793 & 12.218 & $<$ 0.005 \nl 
 H , 12&  D & 0.386& 3.994 & $<$ 0.005  & 6cm, 12&  D & 0.748& 10.764 & $<$ 0.005 \nl
  &  6cm, D  & 0.370 & 3.775 & $<$ 0.005   &   &   H , D  & 0.744 & 10.566 & $<$ 0.005 \nl 
  &   B , D  &-0.181 & -1.749 &0.045   &   &   B , D  & 0.700 & 9.298 & $<$ 0.005 \nl 
  &   X , D  &0.233 & 2.269 &0.015   &   &   X , D  & 0.681 & 8.830 & $<$ 0.005 \nl 
  &  FIR, D  & 0.281 & 2.773 & $<$ 0.005   &   &  FIR, D  &0.239 & 2.339 &0.012 \nl 
  &  6cm, B , D  & -0.011 & -0.100 & $>$ 0.400   &   &   H , B , D  & 0.687 & 8.931 & $<$ 0.005 \nl 
  &  6cm, X , D  & 0.324 & 3.229 & $<$ 0.005   &   &   H , X , D  & 0.702 & 9.302 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.302 & 2.991 & $<$ 0.005   &   &   H ,FIR, D  & 0.265 & 2.593 & 0.007 \nl 
  &   B , X , D  & -0.224 & -2.170 & 0.019   &   &   B , X , D  & 0.669 & 8.492 & $<$ 0.005 \nl 
  &   B ,FIR, D  & 0.150 & 1.433 & 0.082   &   &   B ,FIR, D  & 0.260 & 2.536 & 0.008 \nl 
  &   X ,FIR, D  & 0.222 & 2.151 & 0.020   &   &   X ,FIR, D  & 0.199 & 1.913 & 0.032 \nl 
  &  6cm, B , X , D  & -0.024 & -0.224 & $>$ 0.400   &   &   H , B , X , D  & 0.647 & 7.961 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & 0.160 & 1.520 & 0.071   &   &   H , B ,FIR, D  & 0.265 & 2.579 & 0.007 \nl 
  &  6cm, X ,FIR, D  & 0.261 & 2.531 & 0.008   &   &   H , X ,FIR, D  & 0.241 & 2.331 & 0.013 \nl 
  &   B , X ,FIR, D  & 0.122 & 1.151 & 0.136   &   &   B , X ,FIR, D  & 0.229 & 2.212 & 0.017 \nl 
 H ,FIR&  D & 0.291& 2.903 & $<$ 0.005  & 6cm,FIR&  D & 0.777& 11.757 & $<$ 0.005 \nl
  &  6cm, D  &0.227 & 2.207 &0.017   &   &   H , D  & 0.767 & 11.346 & $<$ 0.005 \nl 
  &   B , D  & -0.324 & -3.249 & $<$ 0.005   &   &   B , D  & 0.734 & 10.254 & $<$ 0.005 \nl 
  &   X , D  &0.134 & 1.281 &0.105   &   &   X , D  & 0.725 & 9.979 & $<$ 0.005 \nl 
  &   12, D  &-0.095 & -0.904 &0.196   &   &   12, D  & 0.386 & 3.974 & $<$ 0.005 \nl 
  &  6cm, B , D  & -0.215 & -2.080 & 0.022   &   &   H , B , D  & 0.713 & 9.597 & $<$ 0.005 \nl 
  &  6cm, X , D  & 0.201 & 1.936 & 0.031   &   &   H , X , D  & 0.732 & 10.142 & $<$ 0.005 \nl 
  &  6cm, 12, D  & -0.039 & -0.365 & 0.359   &   &   H , 12, D  & 0.378 & 3.852 & $<$ 0.005 \nl 
  &   B , X , D  & -0.364 & -3.691 & $<$ 0.005   &   &   B , X , D  & 0.715 & 9.648 & $<$ 0.005 \nl 
  &   B , 12, D  & -0.309 & -3.064 & $<$ 0.005   &   &   B , 12, D  & 0.396 & 4.067 & $<$ 0.005 \nl 
  &   X , 12, D  & -0.114 & -1.084 & 0.152   &   &   X , 12, D  & 0.386 & 3.946 & $<$ 0.005 \nl 
  &  6cm, B , X , D  & -0.215 & -2.063 & 0.023   &   &   H , B , X , D  & 0.680 & 8.699 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & -0.266 & -2.587 & 0.007   &   &   H , B , 12, D  & 0.366 & 3.684 & $<$ 0.005 \nl 
  &  6cm, X , 12, D  & -0.028 & -0.258 & 0.397   &   &   H , X , 12, D  & 0.372 & 3.759 & $<$ 0.005 \nl 
  &   B , X , 12, D  & -0.317 & -3.134 & $<$ 0.005   &   &   B , X , 12, D  & 0.402 & 4.121 & $<$ 0.005 \nl 
6cm, H &  D  &0.195 & 1.893 &0.034  & & & & & \nl
  &   B , D  &-0.248 & -2.434 &0.009   & & & & & \nl
  &   X , D  & -0.006 & -0.061 & $>$ 0.400   & & & & & \nl
  &  FIR, D  &-0.052 & -0.496 &0.312   & & & & & \nl
  &   12, D  &-0.154 & -1.482 &0.076   & & & & & \nl
  &   B , X , D  & -0.310 & -3.076 & $<$ 0.005   & & & & & \nl
  &   B ,FIR, D  & -0.017 & -0.156 & $>$ 0.400   & & & & & \nl
  &   B , 12, D  & -0.173 & -1.658 & 0.053   & & & & & \nl
  &   X ,FIR, D  & -0.151 & -1.446 & 0.081   & & & & & \nl
  &   X , 12, D  & -0.232 & -2.247 & 0.016   & & & & & \nl
  &  FIR, 12, D  & -0.128 & -1.219 & 0.120   & & & & & \nl
  &   B , X ,FIR, D  & -0.076 & -0.714 & 0.242   & & & & & \nl
  &   B , X , 12, D  & -0.221 & -2.124 & 0.021   & & & & & \nl
  &   B ,FIR, 12, D  & -0.058 & -0.547 & 0.294   & & & & & \nl
  &   X ,FIR, 12, D  & -0.205 & -1.963 & 0.029   & & & & & \nl
\enddata
\end{deluxetable}


==> table11c.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{llrrr|llrrr}
\small
\tablenum{11C}
\tablewidth{0pc}
\tablecaption{Spearman Partial Rank Analysis on the $T = 3 - 4$ Sample ($N = 29$)}
\tablehead{
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  &
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  &
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  \\
}
\startdata

 B , X &  D  &0.249 & 1.310 &0.102  & 6cm, X &  D & 0.486& 2.839 & $<$ 0.005 \nl
  &  6cm, D  &0.240 & 1.234 &0.120   &   &   H , D  & 0.488 & 2.795 & $<$ 0.005 \nl 
  &   H , D  & 0.046 & 0.228 & $>$ 0.400   &   &   B , D  &0.483 & 2.756 &0.006 \nl 
  &  FIR, D  &0.081 & 0.406 &0.346   &   &  FIR, D  &0.162 & 0.819 &0.217 \nl 
  &   12, D  & 0.028 & 0.138 & $>$ 0.400   &   &   12, D  & -0.005 & -0.025 & $>$ 0.400 \nl 
  &  6cm, H , D  & 0.004 & 0.017 & $>$ 0.400   &   &   H , B , D  & 0.486 & 2.727 & 0.006 \nl 
  &  6cm,FIR, D  & 0.117 & 0.577 & 0.284   &   &   H ,FIR, D  & 0.187 & 0.931 & 0.191 \nl 
  &  6cm, 12, D  & 0.028 & 0.138 & $>$ 0.400   &   &   H , 12, D  & 0.017 & 0.085 & $>$ 0.400 \nl 
  &   H ,FIR, D  & -0.086 & -0.423 & 0.340   &   &   B ,FIR, D  & 0.182 & 0.907 & 0.197 \nl 
  &   H , 12, D  & -0.064 & -0.313 & 0.381   &   &   B , 12, D  & 0.007 & 0.035 & $>$ 0.400 \nl 
  &  FIR, 12, D  & 0.018 & 0.088 & $>$ 0.400   &   &  FIR, 12, D  & -0.031 & -0.152 & $>$ 0.400 \nl 
  &  6cm, H ,FIR, D  & -0.071 & -0.343 & 0.369   &   &   H , B ,FIR, D  & 0.181 & 0.881 & 0.205 \nl 
  &  6cm, H , 12, D  & -0.062 & -0.299 & 0.386   &   &   H , B , 12, D  & 0.011 & 0.051 & $>$ 0.400 \nl 
  &  6cm,FIR, 12, D  & 0.005 & 0.026 & $>$ 0.400   &   &   H ,FIR, 12, D  & -0.011 & -0.054 & $>$ 0.400 \nl 
  &   H ,FIR, 12, D  & -0.093 & -0.449 & 0.330   &   &   B ,FIR, 12, D  & -0.026 & -0.124 & $>$ 0.400 \nl 
 H , X &  D  &0.247 & 1.302 &0.104  &  H , B &  D & 0.950& 15.592 & $<$ 0.005 \nl
  &  6cm, D  &0.251 & 1.296 &0.106   &   &  6cm, D  & 0.951 & 15.296 & $<$ 0.005 \nl 
  &   B , D  & 0.036 & 0.180 & $>$ 0.400   &   &   X , D  & 0.947 & 14.774 & $<$ 0.005 \nl 
  &  FIR, D  &0.114 & 0.576 &0.285   &   &  FIR, D  & 0.947 & 14.752 & $<$ 0.005 \nl 
  &   12, D  & 0.052 & 0.258 & $>$ 0.400   &   &   12, D  & 0.944 & 14.261 & $<$ 0.005 \nl 
  &  6cm, B , D  & 0.077 & 0.378 & 0.356   &   &  6cm, X , D  & 0.947 & 14.503 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.148 & 0.734 & 0.237   &   &  6cm,FIR, D  & 0.945 & 14.191 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.054 & 0.266 & 0.398   &   &  6cm, 12, D  & 0.933 & 12.658 & $<$ 0.005 \nl 
  &   B ,FIR, D  & 0.118 & 0.583 & 0.282   &   &   X ,FIR, D  & 0.947 & 14.461 & $<$ 0.005 \nl 
  &   B , 12, D  & 0.077 & 0.379 & 0.356   &   &   X , 12, D  & 0.944 & 13.999 & $<$ 0.005 \nl 
  &  FIR, 12, D  & 0.051 & 0.252 & $>$ 0.400   &   &  FIR, 12, D  & 0.945 & 14.093 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & 0.116 & 0.560 & 0.291   &   &  6cm, X ,FIR, D  & 0.945 & 13.825 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & 0.078 & 0.373 & 0.358   &   &  6cm, X , 12, D  & 0.933 & 12.413 & $<$ 0.005 \nl 
  &  6cm,FIR, 12, D  & 0.042 & 0.204 & $>$ 0.400   &   &  6cm,FIR, 12, D  & 0.933 & 12.463 & $<$ 0.005 \nl 
  &   B ,FIR, 12, D  & 0.105 & 0.505 & 0.309   &   &   X ,FIR, 12, D  & 0.945 & 13.861 & $<$ 0.005 \nl 
 X , 12&  D & 0.604& 3.863 & $<$ 0.005  &  B , 12&  D  &0.378 & 2.084 &0.024 \nl
  &  6cm, D  &0.409 & 2.244 &0.019   &   &  6cm, D  & 0.532 & 3.143 & $<$ 0.005 \nl 
  &   H , D  & 0.570 & 3.470 & $<$ 0.005   &   &   H , D  &0.170 & 0.864 &0.207 \nl 
  &   B , D  & 0.569 & 3.455 & $<$ 0.005   &   &   X , D  &0.295 & 1.546 &0.071 \nl 
  &  FIR, D  &0.305 & 1.599 &0.064   &   &  FIR, D  &0.211 & 1.078 &0.157 \nl 
  &  6cm, H , D  & 0.338 & 1.760 & 0.046   &   &  6cm, H , D  & 0.181 & 0.901 & 0.198 \nl 
  &  6cm, B , D  & 0.343 & 1.789 & 0.044   &   &  6cm, X , D  & 0.490 & 2.754 & 0.006 \nl 
  &  6cm,FIR, D  & 0.263 & 1.337 & 0.098   &   &  6cm,FIR, D  & 0.426 & 2.309 & 0.016 \nl 
  &   H , B , D  & 0.571 & 3.410 & $<$ 0.005   &   &   H , X , D  & 0.176 & 0.875 & 0.204 \nl 
  &   H ,FIR, D  & 0.288 & 1.476 & 0.080   &   &   H ,FIR, D  & 0.011 & 0.053 & $>$ 0.400 \nl 
  &   B ,FIR, D  & 0.295 & 1.513 & 0.075   &   &   X ,FIR, D  & 0.196 & 0.979 & 0.180 \nl 
  &  6cm, H , B , D  & 0.343 & 1.752 & 0.047   &   &  6cm, H , X , D  & 0.191 & 0.932 & 0.192 \nl 
  &  6cm, H ,FIR, D  & 0.224 & 1.102 & 0.152   &   &  6cm, H ,FIR, D  & 0.094 & 0.454 & 0.328 \nl 
  &  6cm, B ,FIR, D  & 0.238 & 1.173 & 0.135   &   &  6cm, X ,FIR, D  & 0.413 & 2.174 & 0.021 \nl 
  &   H , B ,FIR, D  & 0.290 & 1.456 & 0.083   &   &   H , X ,FIR, D  & 0.037 & 0.180 & $>$ 0.400 \nl 
 X ,FIR&  D & 0.573& 3.564 & $<$ 0.005  &  B ,FIR&  D  &0.325 & 1.751 &0.047 \nl
  &  6cm, D  &0.378 & 2.042 &0.026   &   &  6cm, D  &0.367 & 1.975 &0.031 \nl 
  &   H , D  & 0.542 & 3.225 & $<$ 0.005   &   &   H , D  &0.214 & 1.097 &0.152 \nl 
  &   B , D  & 0.537 & 3.184 & $<$ 0.005   &   &   X , D  &0.230 & 1.179 &0.133 \nl 
  &   12, D  &0.202 & 1.031 &0.168   &   &   12, D  & 0.050 & 0.249 & $>$ 0.400 \nl 
  &  6cm, H , D  & 0.325 & 1.681 & 0.054   &   &  6cm, H , D  & 0.214 & 1.074 & 0.158 \nl 
  &  6cm, B , D  & 0.321 & 1.661 & 0.056   &   &  6cm, X , D  & 0.308 & 1.586 & 0.066 \nl 
  &  6cm, 12, D  & 0.204 & 1.022 & 0.170   &   &  6cm, 12, D  & 0.112 & 0.552 & 0.293 \nl 
  &   H , B , D  & 0.545 & 3.189 & $<$ 0.005   &   &   H , X , D  & 0.226 & 1.136 & 0.143 \nl 
  &   H , 12, D  & 0.202 & 1.010 & 0.173   &   &   H , 12, D  & 0.133 & 0.655 & 0.258 \nl 
  &   B , 12, D  & 0.201 & 1.005 & 0.174   &   &   X , 12, D  & 0.045 & 0.221 & $>$ 0.400 \nl 
  &  6cm, H , B , D  & 0.332 & 1.685 & 0.053   &   &  6cm, H , X , D  & 0.225 & 1.109 & 0.150 \nl 
  &  6cm, H , 12, D  & 0.201 & 0.986 & 0.179   &   &  6cm, H , 12, D  & 0.150 & 0.726 & 0.241 \nl 
  &  6cm, B , 12, D  & 0.202 & 0.991 & 0.178   &   &  6cm, X , 12, D  & 0.109 & 0.523 & 0.302 \nl 
  &   H , B , 12, D  & 0.213 & 1.044 & 0.166   &   &   H , X , 12, D  & 0.149 & 0.721 & 0.243 \nl 
\tablebreak 
6cm, B &  D  &0.083 & 0.422 &0.340  & FIR, 12&  D & 0.783& 6.416 & $<$ 0.005 \nl
  &   H , D  &0.087 & 0.437 &0.335   &   &  6cm, D  & 0.541 & 3.212 & $<$ 0.005 \nl 
  &   X , D  & -0.045 & -0.228 & $>$ 0.400   &   &   H , D  & 0.763 & 5.893 & $<$ 0.005 \nl 
  &  FIR, D  &-0.199 & -1.015 &0.171   &   &   B , D  & 0.754 & 5.737 & $<$ 0.005 \nl 
  &   12, D  &-0.411 & -2.257 &0.018   &   &   X , D  & 0.669 & 4.498 & $<$ 0.005 \nl 
  &   H , X , D  & 0.074 & 0.365 & 0.361   &   &  6cm, H , D  & 0.463 & 2.559 & 0.009 \nl 
  &   H ,FIR, D  & -0.087 & -0.426 & 0.339   &   &  6cm, B , D  & 0.438 & 2.388 & 0.014 \nl 
  &   H , 12, D  & -0.106 & -0.524 & 0.302   &   &  6cm, X , D  & 0.457 & 2.515 & 0.010 \nl 
  &   X ,FIR, D  & -0.216 & -1.082 & 0.156   &   &   H , B , D  & 0.754 & 5.628 & $<$ 0.005 \nl 
  &   X , 12, D  & -0.411 & -2.211 & 0.020   &   &   H , X , D  & 0.657 & 4.267 & $<$ 0.005 \nl 
  &  FIR, 12, D  & -0.421 & -2.277 & 0.017   &   &   B , X , D  & 0.646 & 4.149 & $<$ 0.005 \nl 
  &   H , X ,FIR, D  & -0.072 & -0.346 & 0.368   &   &  6cm, H , B , D  & 0.442 & 2.361 & 0.015 \nl 
  &   H , X , 12, D  & -0.106 & -0.509 & 0.308   &   &  6cm, H , X , D  & 0.397 & 2.074 & 0.025 \nl 
  &   H ,FIR, 12, D  & -0.127 & -0.615 & 0.273   &   &  6cm, B , X , D  & 0.369 & 1.902 & 0.037 \nl 
  &   X ,FIR, 12, D  & -0.421 & -2.227 & 0.020   &   &   H , B , X , D  & 0.644 & 4.032 & $<$ 0.005 \nl 
 H , 12&  D  &0.346 & 1.879 &0.038  & 6cm, 12&  D & 0.809& 7.029 & $<$ 0.005 \nl
  &  6cm, D  & 0.509 & 2.957 & $<$ 0.005   &   &   H , D  & 0.843 & 7.821 & $<$ 0.005 \nl 
  &   B , D  & -0.048 & -0.240 & $>$ 0.400   &   &   B , D  & 0.844 & 7.854 & $<$ 0.005 \nl 
  &   X , D  &0.254 & 1.314 &0.101   &   &   X , D  & 0.740 & 5.509 & $<$ 0.005 \nl 
  &  FIR, D  &0.219 & 1.122 &0.146   &   &  FIR, D  & 0.608 & 3.828 & $<$ 0.005 \nl 
  &  6cm, B , D  & 0.012 & 0.059 & $>$ 0.400   &   &   H , B , D  & 0.843 & 7.683 & $<$ 0.005 \nl 
  &  6cm, X , D  & 0.460 & 2.538 & 0.009   &   &   H , X , D  & 0.787 & 6.248 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & 0.422 & 2.277 & 0.017   &   &   H ,FIR, D  & 0.675 & 4.480 & $<$ 0.005 \nl 
  &   B , X , D  & -0.083 & -0.410 & 0.345   &   &   B , X , D  & 0.790 & 6.311 & $<$ 0.005 \nl 
  &   B ,FIR, D  & 0.062 & 0.302 & 0.384   &   &   B ,FIR, D  & 0.678 & 4.523 & $<$ 0.005 \nl 
  &   X ,FIR, D  & 0.195 & 0.972 & 0.182   &   &   X ,FIR, D  & 0.594 & 3.621 & $<$ 0.005 \nl 
  &  6cm, B , X , D  & -0.015 & -0.073 & $>$ 0.400   &   &   H , B , X , D  & 0.788 & 6.145 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & 0.063 & 0.301 & 0.385   &   &   H , B ,FIR, D  & 0.678 & 4.429 & $<$ 0.005 \nl 
  &  6cm, X ,FIR, D  & 0.401 & 2.099 & 0.024   &   &   H , X ,FIR, D  & 0.660 & 4.215 & $<$ 0.005 \nl 
  &   B , X ,FIR, D  & 0.028 & 0.135 & $>$ 0.400   &   &   B , X ,FIR, D  & 0.665 & 4.269 & $<$ 0.005 \nl 
 H ,FIR&  D  &0.274 & 1.454 &0.083  & 6cm,FIR&  D & 0.679& 4.722 & $<$ 0.005 \nl
  &  6cm, D  &0.320 & 1.690 &0.053   &   &   H , D  & 0.691 & 4.780 & $<$ 0.005 \nl 
  &   B , D  &-0.117 & -0.589 &0.280   &   &   B , D  & 0.692 & 4.798 & $<$ 0.005 \nl 
  &   X , D  &0.167 & 0.846 &0.211   &   &   X , D  & 0.560 & 3.376 & $<$ 0.005 \nl 
  &   12, D  & 0.006 & 0.031 & $>$ 0.400   &   &   12, D  &0.125 & 0.631 &0.266 \nl 
  &  6cm, B , D  & -0.100 & -0.494 & 0.313   &   &   H , B , D  & 0.691 & 4.683 & $<$ 0.005 \nl 
  &  6cm, X , D  & 0.251 & 1.273 & 0.111   &   &   H , X , D  & 0.582 & 3.502 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.062 & 0.305 & 0.383   &   &   H , 12, D  & 0.140 & 0.690 & 0.248 \nl 
  &   B , X , D  & -0.162 & -0.803 & 0.221   &   &   B , X , D  & 0.586 & 3.546 & $<$ 0.005 \nl 
  &   B , 12, D  & -0.123 & -0.608 & 0.274   &   &   B , 12, D  & 0.160 & 0.794 & 0.223 \nl 
  &   X , 12, D  & -0.004 & -0.021 & $>$ 0.400   &   &   X , 12, D  & 0.129 & 0.637 & 0.264 \nl 
  &  6cm, B , X , D  & -0.132 & -0.641 & 0.265   &   &   H , B , X , D  & 0.581 & 3.426 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & -0.118 & -0.568 & 0.288   &   &   H , B , 12, D  & 0.156 & 0.757 & 0.234 \nl 
  &  6cm, X , 12, D  & 0.052 & 0.251 & $>$ 0.400   &   &   H , X , 12, D  & 0.139 & 0.673 & 0.255 \nl 
  &   B , X , 12, D  & -0.142 & -0.688 & 0.251   &   &   B , X , 12, D  & 0.162 & 0.787 & 0.227 \nl 
6cm, H &  D  &0.058 & 0.299 &0.386  & & & & & \nl
  &   B , D  &-0.065 & -0.324 &0.376   & & & & & \nl
  &   X , D  &-0.073 & -0.366 &0.361   & & & & & \nl
  &  FIR, D  &-0.181 & -0.921 &0.193   & & & & & \nl
  &   12, D  &-0.402 & -2.194 &0.020   & & & & & \nl
  &   B , X , D  & -0.094 & -0.461 & 0.326   & & & & & \nl
  &   B ,FIR, D  & 0.023 & 0.112 & $>$ 0.400   & & & & & \nl
  &   B , 12, D  & -0.045 & -0.220 & $>$ 0.400   & & & & & \nl
  &   X ,FIR, D  & -0.204 & -1.019 & 0.170   & & & & & \nl
  &   X , 12, D  & -0.402 & -2.151 & 0.022   & & & & & \nl
  &  FIR, 12, D  & -0.406 & -2.175 & 0.021   & & & & & \nl
  &   B , X ,FIR, D  & 0.001 & 0.007 & $>$ 0.400   & & & & & \nl
  &   B , X , 12, D  & -0.046 & -0.219 & $>$ 0.400   & & & & & \nl
  &   B ,FIR, 12, D  & -0.026 & -0.124 & $>$ 0.400   & & & & & \nl
  &   X ,FIR, 12, D  & -0.405 & -2.124 & 0.023   & & & & & \nl
\enddata
\end{deluxetable}


==> table11d.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{llrrr|llrrr}
\small
\tablenum{11D}
\tablewidth{0pc}
\tablecaption{Spearman Partial Rank Analysis on the $T = 5 - 10$ Sample ($N = 38$)}
\tablehead{
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  &
\colhead{Test} & \colhead{Held} &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  &
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  \\
}
\startdata

 B , X &  D & 0.445& 2.936 & $<$ 0.005  & 6cm, X &  D & 0.528& 3.677 & $<$ 0.005 \nl
  &  6cm, D  &0.277 & 1.681 &0.052   &   &   H , D  & 0.431 & 2.781 & $<$ 0.005 \nl 
  &   H , D  &0.260 & 1.567 &0.067   &   &   B , D  &0.412 & 2.638 &0.007 \nl 
  &  FIR, D  &-0.045 & -0.265 &0.398   &   &  FIR, D  &0.174 & 1.029 &0.167 \nl 
  &   12, D  &0.102 & 0.598 &0.277   &   &   12, D  &0.338 & 2.095 &0.023 \nl 
  &  6cm, H , D  & 0.249 & 1.479 & 0.078   &   &   H , B , D  & 0.425 & 2.699 & 0.006 \nl 
  &  6cm,FIR, D  & -0.005 & -0.028 & $>$ 0.400   &   &   H ,FIR, D  & 0.134 & 0.778 & 0.227 \nl 
  &  6cm, 12, D  & 0.099 & 0.574 & 0.285   &   &   H , 12, D  & 0.338 & 2.060 & 0.024 \nl 
  &   H ,FIR, D  & 0.228 & 1.347 & 0.095   &   &   B ,FIR, D  & 0.168 & 0.979 & 0.179 \nl 
  &   H , 12, D  & 0.285 & 1.710 & 0.049   &   &   B , 12, D  & 0.337 & 2.059 & 0.024 \nl 
  &  FIR, 12, D  & -0.037 & -0.213 & $>$ 0.400   &   &  FIR, 12, D  & 0.171 & 0.996 & 0.175 \nl 
  &  6cm, H ,FIR, D  & 0.231 & 1.341 & 0.096   &   &   H , B ,FIR, D  & 0.138 & 0.790 & 0.224 \nl 
  &  6cm, H , 12, D  & 0.270 & 1.584 & 0.065   &   &   H , B , 12, D  & 0.325 & 1.943 & 0.032 \nl 
  &  6cm,FIR, 12, D  & -0.002 & -0.011 & $>$ 0.400   &   &   H ,FIR, 12, D  & 0.136 & 0.775 & 0.227 \nl 
  &   H ,FIR, 12, D  & 0.235 & 1.371 & 0.092   &   &   B ,FIR, 12, D  & 0.167 & 0.957 & 0.184 \nl 
 H , X &  D  &0.390 & 2.506 &0.009  &  H , B &  D & 0.952& 18.346 & $<$ 0.005 \nl
  &  6cm, D  &0.206 & 1.228 &0.119   &   &  6cm, D  & 0.940 & 16.070 & $<$ 0.005 \nl 
  &   B , D  &-0.120 & -0.706 &0.244   &   &   X , D  & 0.944 & 16.629 & $<$ 0.005 \nl 
  &  FIR, D  &-0.174 & -1.031 &0.166   &   &  FIR, D  & 0.878 & 10.708 & $<$ 0.005 \nl 
  &   12, D  & -0.037 & -0.217 & $>$ 0.400   &   &   12, D  & 0.881 & 10.880 & $<$ 0.005 \nl 
  &  6cm, B , D  & -0.166 & -0.965 & 0.182   &   &  6cm, X , D  & 0.939 & 15.692 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & -0.135 & -0.781 & 0.226   &   &  6cm,FIR, D  & 0.871 & 10.165 & $<$ 0.005 \nl 
  &  6cm, 12, D  & -0.031 & -0.178 & $>$ 0.400   &   &  6cm, 12, D  & 0.883 & 10.779 & $<$ 0.005 \nl 
  &   B ,FIR, D  & -0.281 & -1.682 & 0.052   &   &   X ,FIR, D  & 0.885 & 10.904 & $<$ 0.005 \nl 
  &   B , 12, D  & -0.270 & -1.613 & 0.061   &   &   X , 12, D  & 0.890 & 11.239 & $<$ 0.005 \nl 
  &  FIR, 12, D  & -0.175 & -1.021 & 0.169   &   &  FIR, 12, D  & 0.868 & 10.055 & $<$ 0.005 \nl 
  &  6cm, B ,FIR, D  & -0.265 & -1.556 & 0.068   &   &  6cm, X ,FIR, D  & 0.878 & 10.374 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & -0.254 & -1.483 & 0.078   &   &  6cm, X , 12, D  & 0.890 & 11.067 & $<$ 0.005 \nl 
  &  6cm,FIR, 12, D  & -0.141 & -0.807 & 0.220   &   &  6cm,FIR, 12, D  & 0.862 & 9.621 & $<$ 0.005 \nl 
  &   B ,FIR, 12, D  & -0.288 & -1.703 & 0.050   &   &   X ,FIR, 12, D  & 0.876 & 10.271 & $<$ 0.005 \nl 
 X , 12&  D & 0.510& 3.505 & $<$ 0.005  &  B , 12&  D & 0.760& 6.924 & $<$ 0.005 \nl
  &  6cm, D  &0.302 & 1.847 &0.039   &   &  6cm, D  & 0.690 & 5.553 & $<$ 0.005 \nl 
  &   H , D  &0.358 & 2.237 &0.018   &   &   H , D  & -0.019 & -0.112 & $>$ 0.400 \nl 
  &   B , D  &0.295 & 1.802 &0.043   &   &   X , D  & 0.693 & 5.597 & $<$ 0.005 \nl 
  &  FIR, D  & -0.034 & -0.201 & $>$ 0.400   &   &  FIR, D  &0.294 & 1.791 &0.043 \nl 
  &  6cm, H , D  & 0.228 & 1.343 & 0.096   &   &  6cm, H , D  & -0.056 & -0.322 & 0.377 \nl 
  &  6cm, B , D  & 0.160 & 0.928 & 0.191   &   &  6cm, X , D  & 0.662 & 5.068 & $<$ 0.005 \nl 
  &  6cm,FIR, D  & -0.011 & -0.062 & $>$ 0.400   &   &  6cm,FIR, D  & 0.271 & 1.619 & 0.060 \nl 
  &   H , B , D  & 0.376 & 2.331 & 0.015   &   &   H , X , D  & -0.124 & -0.720 & 0.240 \nl 
  &   H ,FIR, D  & 0.039 & 0.223 & $>$ 0.400   &   &   H ,FIR, D  & -0.130 & -0.752 & 0.233 \nl 
  &   B ,FIR, D  & -0.022 & -0.127 & $>$ 0.400   &   &   X ,FIR, D  & 0.292 & 1.757 & 0.046 \nl 
  &  6cm, H , B , D  & 0.250 & 1.460 & 0.081   &   &  6cm, H , X , D  & -0.120 & -0.681 & 0.250 \nl 
  &  6cm, H ,FIR, D  & 0.044 & 0.249 & $>$ 0.400   &   &  6cm, H ,FIR, D  & -0.130 & -0.741 & 0.235 \nl 
  &  6cm, B ,FIR, D  & -0.010 & -0.056 & $>$ 0.400   &   &  6cm, X ,FIR, D  & 0.271 & 1.594 & 0.064 \nl 
  &   H , B ,FIR, D  & 0.071 & 0.402 & 0.347   &   &   H , X ,FIR, D  & -0.142 & -0.814 & 0.218 \nl 
 X ,FIR&  D & 0.606& 4.509 & $<$ 0.005  &  B ,FIR&  D & 0.771& 7.168 & $<$ 0.005 \nl
  &  6cm, D  &0.387 & 2.446 &0.010   &   &  6cm, D  & 0.724 & 6.118 & $<$ 0.005 \nl 
  &   H , D  & 0.526 & 3.606 & $<$ 0.005   &   &   H , D  &0.127 & 0.748 &0.234 \nl 
  &   B , D  & 0.462 & 3.037 & $<$ 0.005   &   &   X , D  & 0.704 & 5.785 & $<$ 0.005 \nl 
  &   12, D  &0.383 & 2.416 &0.012   &   &   12, D  &0.350 & 2.179 &0.020 \nl 
  &  6cm, H , D  & 0.358 & 2.202 & 0.019   &   &  6cm, H , D  & 0.098 & 0.566 & 0.288 \nl 
  &  6cm, B , D  & 0.281 & 1.683 & 0.052   &   &  6cm, X , D  & 0.696 & 5.569 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.254 & 1.508 & 0.075   &   &  6cm, 12, D  & 0.399 & 2.498 & 0.009 \nl 
  &   H , B , D  & 0.515 & 3.448 & $<$ 0.005   &   &   H , X , D  & -0.011 & -0.065 & $>$ 0.400 \nl 
  &   H , 12, D  & 0.414 & 2.614 & 0.007   &   &   H , 12, D  & 0.180 & 1.051 & 0.162 \nl 
  &   B , 12, D  & 0.372 & 2.305 & 0.016   &   &   X , 12, D  & 0.338 & 2.066 & 0.024 \nl 
  &  6cm, H , B , D  & 0.346 & 2.086 & 0.023   &   &  6cm, H , X , D  & 0.010 & 0.055 & $>$ 0.400 \nl 
  &  6cm, H , 12, D  & 0.287 & 1.693 & 0.051   &   &  6cm, H , 12, D  & 0.152 & 0.873 & 0.204 \nl 
  &  6cm, B , 12, D  & 0.235 & 1.366 & 0.093   &   &  6cm, X , 12, D  & 0.388 & 2.383 & 0.013 \nl 
  &   H , B , 12, D  & 0.385 & 2.358 & 0.014   &   &   H , X , 12, D  & 0.071 & 0.402 & 0.347 \nl 
\tablebreak 
6cm, B &  D & 0.442& 2.919 & $<$ 0.005  & FIR, 12&  D & 0.864& 10.136 & $<$ 0.005 \nl
  &   H , D  &0.082 & 0.478 &0.319   &   &  6cm, D  & 0.796 & 7.676 & $<$ 0.005 \nl 
  &   X , D  &0.273 & 1.656 &0.056   &   &   H , D  & 0.632 & 4.759 & $<$ 0.005 \nl 
  &  FIR, D  &-0.235 & -1.410 &0.087   &   &   B , D  & 0.671 & 5.271 & $<$ 0.005 \nl 
  &   12, D  & 0.025 & 0.144 & $>$ 0.400   &   &   X , D  & 0.811 & 8.072 & $<$ 0.005 \nl 
  &   H , X , D  & -0.035 & -0.198 & $>$ 0.400   &   &  6cm, H , D  & 0.539 & 3.681 & $<$ 0.005 \nl 
  &   H ,FIR, D  & -0.002 & -0.013 & $>$ 0.400   &   &  6cm, B , D  & 0.595 & 4.249 & $<$ 0.005 \nl 
  &   H , 12, D  & 0.097 & 0.560 & 0.290   &   &  6cm, X , D  & 0.773 & 6.998 & $<$ 0.005 \nl 
  &   X ,FIR, D  & -0.231 & -1.363 & 0.093   &   &   H , B , D  & 0.640 & 4.785 & $<$ 0.005 \nl 
  &   X , 12, D  & -0.010 & -0.060 & $>$ 0.400   &   &   H , X , D  & 0.559 & 3.873 & $<$ 0.005 \nl 
  &  FIR, 12, D  & -0.205 & -1.206 & 0.125   &   &   B , X , D  & 0.630 & 4.666 & $<$ 0.005 \nl 
  &   H , X ,FIR, D  & -0.034 & -0.193 & $>$ 0.400   &   &  6cm, H , B , D  & 0.548 & 3.710 & $<$ 0.005 \nl 
  &   H , X , 12, D  & 0.001 & 0.004 & $>$ 0.400   &   &  6cm, H , X , D  & 0.504 & 3.299 & $<$ 0.005 \nl 
  &   H ,FIR, 12, D  & -0.007 & -0.039 & $>$ 0.400   &   &  6cm, B , X , D  & 0.580 & 4.031 & $<$ 0.005 \nl 
  &   X ,FIR, 12, D  & -0.202 & -1.168 & 0.134   &   &   H , B , X , D  & 0.562 & 3.844 & $<$ 0.005 \nl 
 H , 12&  D & 0.803& 7.958 & $<$ 0.005  & 6cm, 12&  D & 0.565& 4.046 & $<$ 0.005 \nl
  &  6cm, D  & 0.747 & 6.555 & $<$ 0.005   &   &   H , D  &0.393 & 2.492 &0.009 \nl 
  &   B , D  &0.396 & 2.515 &0.009   &   &   B , D  &0.392 & 2.482 &0.010 \nl 
  &   X , D  & 0.762 & 6.863 & $<$ 0.005   &   &   X , D  &0.404 & 2.578 &0.008 \nl 
  &  FIR, D  &0.399 & 2.538 &0.009   &   &  FIR, D  &-0.138 & -0.810 &0.219 \nl 
  &  6cm, B , D  & 0.400 & 2.509 & 0.009   &   &   H , B , D  & 0.396 & 2.477 & 0.010 \nl 
  &  6cm, X , D  & 0.734 & 6.213 & $<$ 0.005   &   &   H , X , D  & 0.283 & 1.697 & 0.050 \nl 
  &  6cm,FIR, D  & 0.380 & 2.357 & 0.014   &   &   H ,FIR, D  & -0.035 & -0.204 & $>$ 0.400 \nl 
  &   B , X , D  & 0.455 & 2.935 & $<$ 0.005   &   &   B , X , D  & 0.310 & 1.874 & 0.037 \nl 
  &   B ,FIR, D  & 0.309 & 1.866 & 0.038   &   &   B ,FIR, D  & -0.074 & -0.426 & 0.339 \nl 
  &   X ,FIR, D  & 0.399 & 2.503 & 0.009   &   &   X ,FIR, D  & -0.134 & -0.776 & 0.227 \nl 
  &  6cm, B , X , D  & 0.438 & 2.758 & $<$ 0.005   &   &   H , B , X , D  & 0.281 & 1.659 & 0.055 \nl 
  &  6cm, B ,FIR, D  & 0.303 & 1.797 & 0.043   &   &   H , B ,FIR, D  & -0.036 & -0.204 & $>$ 0.400 \nl 
  &  6cm, X ,FIR, D  & 0.382 & 2.336 & 0.014   &   &   H , X ,FIR, D  & -0.041 & -0.233 & $>$ 0.400 \nl 
  &   B , X ,FIR, D  & 0.316 & 1.881 & 0.037   &   &   B , X ,FIR, D  & -0.071 & -0.404 & 0.347 \nl 
 H ,FIR&  D & 0.785& 7.495 & $<$ 0.005  & 6cm,FIR&  D & 0.710& 5.969 & $<$ 0.005 \nl
  &  6cm, D  & 0.746 & 6.540 & $<$ 0.005   &   &   H , D  & 0.654 & 5.046 & $<$ 0.005 \nl 
  &   B , D  &0.261 & 1.574 &0.066   &   &   B , D  & 0.646 & 4.940 & $<$ 0.005 \nl 
  &   X , D  & 0.749 & 6.591 & $<$ 0.005   &   &   X , D  & 0.578 & 4.127 & $<$ 0.005 \nl 
  &   12, D  &0.305 & 1.869 &0.038   &   &   12, D  & 0.535 & 3.694 & $<$ 0.005 \nl 
  &  6cm, B , D  & 0.280 & 1.677 & 0.053   &   &   H , B , D  & 0.651 & 4.933 & $<$ 0.005 \nl 
  &  6cm, X , D  & 0.739 & 6.298 & $<$ 0.005   &   &   H , X , D  & 0.558 & 3.858 & $<$ 0.005 \nl 
  &  6cm, 12, D  & 0.377 & 2.336 & 0.014   &   &   H , 12, D  & 0.570 & 3.983 & $<$ 0.005 \nl 
  &   B , X , D  & 0.359 & 2.210 & 0.019   &   &   B , X , D  & 0.564 & 3.926 & $<$ 0.005 \nl 
  &   B , 12, D  & -0.007 & -0.042 & $>$ 0.400   &   &   B , 12, D  & 0.562 & 3.905 & $<$ 0.005 \nl 
  &   X , 12, D  & 0.346 & 2.119 & 0.022   &   &   X , 12, D  & 0.467 & 3.031 & $<$ 0.005 \nl 
  &  6cm, B , X , D  & 0.345 & 2.081 & 0.024   &   &   H , B , X , D  & 0.557 & 3.799 & $<$ 0.005 \nl 
  &  6cm, B , 12, D  & 0.057 & 0.324 & 0.376   &   &   H , B , 12, D  & 0.564 & 3.865 & $<$ 0.005 \nl 
  &  6cm, X , 12, D  & 0.398 & 2.452 & 0.010   &   &   H , X , 12, D  & 0.502 & 3.283 & $<$ 0.005 \nl 
  &   B , X , 12, D  & 0.104 & 0.594 & 0.279   &   &   B , X , 12, D  & 0.500 & 3.263 & $<$ 0.005 \nl 
6cm, H &  D & 0.441& 2.909 & $<$ 0.005  & & & & & \nl
  &   B , D  &0.073 & 0.428 &0.338   & & & & & \nl
  &   X , D  &0.301 & 1.840 &0.040   & & & & & \nl
  &  FIR, D  &-0.266 & -1.612 &0.061   & & & & & \nl
  &   12, D  & -0.024 & -0.140 & $>$ 0.400   & & & & & \nl
  &   B , X , D  & 0.136 & 0.788 & 0.224   & & & & & \nl
  &   B ,FIR, D  & -0.129 & -0.748 & 0.234   & & & & & \nl
  &   B , 12, D  & -0.097 & -0.559 & 0.290   & & & & & \nl
  &   X ,FIR, D  & -0.244 & -1.442 & 0.083   & & & & & \nl
  &   X , 12, D  & -0.012 & -0.069 & $>$ 0.400   & & & & & \nl
  &  FIR, 12, D  & -0.233 & -1.375 & 0.092   & & & & & \nl
  &   B , X ,FIR, D  & -0.087 & -0.492 & 0.314   & & & & & \nl
  &   B , X , 12, D  & -0.006 & -0.035 & $>$ 0.400   & & & & & \nl
  &   B ,FIR, 12, D  & -0.112 & -0.638 & 0.264   & & & & & \nl
  &   X ,FIR, 12, D  & -0.209 & -1.210 & 0.124   & & & & & \nl
\enddata
\end{deluxetable}


==> table2.tex <==
\begin{deluxetable}{l}
\tablenum{2}
\small
\tablewidth{0pc}
\tablecaption{References to Table1}
\tablehead{
%\colhead{}
}

\startdata
1. X-ray data from HRI \nl
2. X-ray source may not be associated with galaxy. \nl
3. X-ray data are from the previous works  \nl
   LMC and SMC (compilation of Fabbiano 1989)\nl
   M31 and M32 (Trinchieri and Fabbiano 1991)\nl
   M33 (Trinchieri et al. 1988)\nl
   M101 (Trinchieri et al. 1990)\nl
4. N523 : no morphological type in RC2 (peculiar galaxy). Assigned to late sample. \nl
5. N4236, N4258 : combined x-ray flux of two sources (see FKT). \nl
6. IRAS data from Knapp et al. (1989) \nl
7. Galaxies not observed by IRAS from Lonsdale et al. (1985) \nl
\nl
8. IRAS fluxes from Rice et al. (1988) \nl
9. IRAS fluxes from Gallagher et al. (1991) \nl
10. IRAS fluxes from the IRAS Extragalactic Catalog (Fullmer \& Lonsdale 1989) \nl
11. IRAS fluxes from the IRAS Extragalactic Catalog (Fullmer \& Lonsdale 1989) \nl
   blended in the IR: \nl
   NGC 1512 with NGC 1510; \nl
   NGC 3395 with NGC 3396; \nl
   NGC 3690 with IC   694; \nl
   NGC 3994 with NGC 3995; \nl
   NGC 4038 with NGC 4039; \nl
   IC  3528 with NGC 4540; \nl
   NGC 4567 with NGC 4568; \nl
   NGC 4861 with IC  3961; \nl
   NGC 5683 with NGC 5682; \nl
   NGC 7320 with NGC 7319; \nl
   NGC 7469 with IC  5283; \nl
   NGC 7771 with NGC 7770;\nl 
12. IRAS fluxes from Helou et al. (1988) (NED)\nl
13. IRAS fluxes from Knapp et al. (1990) (NED)\nl
14. IRAS fluxes from Corbelli et al. (1991) (NED)\nl
15. FIR detection by Telesco \& Harper (1980) \nl
16. FIR from NGC 7682 confused by emission from NGC 7679. \nl
17. IRAS fluxes from "1990IRASF.C...0000M" (NED) \nl
\nl
18. 6cm from Fabbiano et al. (1989) \nl
19. 6cm from Gioia \& Fabbiano (1987) \nl
20. 6cm from Roberts et al. (1991) \nl
21. 6cm from Ekers \& Ekers (1973) \nl
22. 6cm from Wright (1974) \nl
23. 6cm from Sulentic (1976) \nl
24. 6cm from Sramek (1975) \nl
25. 6cm from Sramek (1975) blended with NGC 7770 \nl
26. 6cm from Whiteoak (1970) \nl
27. 6cm from Whiteoak, blended with NGC 4039 \nl
28. 6cm from Condon et al. (1982)  \nl
29. 6cm from Hummel et al (1984)  \nl
30. 6cm from Ulvestad et al. (1981)  \nl
31. 6cm from Jones et al. (1981) \nl
32. 6cm from Wilson \& Ulvestad (1982) \nl
33. 6cm from Stocke et al. (1978) \nl
34. 6cm from Condon, (1980) \nl
35. 6cm from Haynes et al. (1975) \nl
36. 6cm from Wunderlich, Klein \& Wielebinski (1987) \nl
37. 6cm from Disney \& Wall (1977) \nl
38. 6cm from Calvani et al. (1989) \nl
39. 6cm from Ulvestad and Wilson (1989) (NED)\nl
40. 6cm from Ulvestad and Wilson (1984) \nl
41. 6cm from Klein (1986) \nl
42. 6cm from Wunderlich and Klein (1991) (NED) \nl
43. 6cm from Condon et al. (1991) (NED). \nl
44. 6cm from Becker et. al. (1991) \nl
\nl
45. H-band data from Tormen and Burstein (1996) \nl
46. H-band data from Aaronson et al. (1981) \nl     
47. H-band data from Aaronson et al. (1982) \nl     
48. H-band data from Allen (1976) \nl
49. H-band data from Balzano and Weedman (1981) \nl
50. H-band data from Becklin et al. (1980) \nl     
51. H-band data from Bothun et al. (1984) \nl     
52. H-band data from Bothun et al. (1985) \nl     
53. H-band data from Cutri and McAlary (1985) \nl
54. H-band data from Frogel et al. (1978) \nl     
55. H-band data from Glass (1976) \nl
56. H-band data from Glass (1984) \nl
57. H-band data from Glass and Moorwood (1985) \nl
58. H-band data from Griersmith, Hyland, Jones (1982) \nl
59. H-band data from Heckman et al. (1983) \nl     
60. H-band data from Hunter and Gallagher (1985) \nl
61. H-band data from Mould, Aaronson, Huchra (1980) \nl
62. H-band data from Mould (1981) \nl
63. H-band data from Persson, Frogel, Aaronson (1979) \nl
64. H-band data from Penston et al. (1974) \nl     
65. H-band data from Rieke (1978) \nl
66. H-band data from Thuan (1983) \nl
67. H-band data from Ward et al. (1982) \nl     
68. H-band data from Willner et al. (1985) \nl     

\enddata
\end{deluxetable}



==> table3.tex <==
\begin{deluxetable}{rcrr}
\tablenum{3}
\tablewidth{0pc}
\tablecaption{Photometric Systems for Magnitude to Flux Conversion}
\tablehead{
\colhead{System} &
\colhead{$\lambda_{eff}$ ($\mu$m) } & 
\colhead{$F_{\nu}(0)$ (mJy)} &
\colhead{References\tablenotemark{a} }\\
}

\startdata
Cal Tech - Harvard College Observatory& 1.65 & 980 & 46,47,50,51,52,54,60,61,62,63,64,68\nl
Johnson& 1.65 & 1075 & 48,53,59,65\nl
Anglo-Australian Observatory& 1.64& 1030 & 56\tablenotemark{b},57 \tablenotemark{b},58,67\nl
Royal Greenwich Observatory& 1.60& 1075 & 55\nl
Kitt Peak National Observatory & 1.66 & 1010 & 49\nl
\nodata  & 1.64  & \nodata &  66 \tablenotemark{c}\nl

\tablenotetext{a}{ Reference codes as in Table 2.}
\tablenotetext{b}{The $H$ magnitudes in Refs. 56 and 57 
from the South African Astronomical Observatory, were
first converted to the AAO system via $H_{AAO} =  H_{SAAO} / 1.01$).}
\tablenotetext{c}{To convert the $H$ magnitude from Ref. 66 we used their conversion of 
$F_{\nu} = 1.02 Jy$ for $H = 15.0$ mag.}

\enddata
\end{deluxetable}



==> table4.tex <==
\begin{deluxetable}{lrrrrrrrrr}
\tablenum{4}
\small
\tablewidth{0pc}
\tablecaption{Luminosity Data}
\tablehead{
\colhead{Name} & 
\colhead{$log(L_X)$} &
\colhead{$log(L_B)$} & 
\colhead{$log(L_H)$} &
\colhead{$log(L_{12})$} &
\colhead{$log(L_{25})$} & 
\colhead{$log(L_{60})$} &
\colhead{$log(L_{100})$} & 
\colhead{$log(L_{FIR})$} & 
\colhead{$log(L_{6cm})$} \\
\colhead{}     & \colhead{erg/sec} & \colhead{erg/sec} &
\colhead{erg/sec} & \colhead{erg/sec} &
\colhead{erg/sec} &
\colhead{erg/sec} & \colhead{erg/sec} & \colhead{erg/sec}
& \colhead{erg/sec} \\
 }

\startdata

 
N0125  &$<$ 41.44 &   43.35 &  &  &  &  &  &  &$<$ 37.29 \nl
 N0224  &   39.55 &   43.33 &   43.91 &   42.27 &   41.63 &   41.99 &   42.32 &   42.59 &   34.94 \nl
 N0247  &   39.17 &   42.29 &   42.36 &$<$ 40.31 &$<$ 39.99 &   41.34 &   41.47 &   41.81 &  \nl
 N0253  &   39.90 &   43.05 &   43.62 &   43.01 &   43.00 &   43.47 &   43.33 &   43.81 &   36.08 \nl
   SMC  &   37.96 &   41.55 &  &   39.66 &   39.82 &   40.87 &   40.81 &   41.24 &  \nl
 N0309  &$<$ 41.31 &   43.83 &  &$<$ 43.47 &$<$ 43.11 &   43.55 &   43.65 &   44.01 &  \nl
 I1613  &   38.18 &   40.74 &  &$<$ 38.82 &$<$ 38.74 &   39.40 &   39.41 &   39.81 &  \nl
 N0449  &$<$ 41.42 &   42.79 &   43.08 &$<$ 44.20 &   43.39 &   43.51 &   43.20 &   43.79 &   36.89 \nl
 N0520  &$<$ 40.72 &   43.35 &   43.89 &   43.33 &   43.44 &   44.14 &   43.92 &   44.45 &   36.79 \nl
 N0521   \tablenotemark{b}&$<$ 41.40 &   43.67 &  &$<$ 43.87 &$<$ 43.04 &   42.90 &   43.30 &   43.55 &  \nl
 N0524   \tablenotemark{b}&   41.01 &   43.52 &   44.17 &   42.73 &$<$ 42.08 &   42.47 &   42.42 &   42.85 &   35.47 \nl
 N0523  &$<$ 41.12 &   43.58 &   43.85 &$<$ 43.33 &   42.91 &   43.45 &   43.40 &   43.83 &$<$ 36.68 \nl
 N0578  &$<$ 40.31 &   43.13 &   43.24 &   42.34 &$<$ 42.03 &   42.67 &   42.87 &   43.19 &  \nl
 N0598  &   39.25 &   42.45 &   42.58 &   41.64 &   41.28 &   41.96 &   42.03 &   42.40 &   34.74 \nl
 N0625  &$<$ 38.91 &   41.80 &  &$<$ 41.08 &   41.16 &   41.62 &   41.40 &   41.93 &  \nl
 N0628  &   39.34 &   42.73 &   42.95 &   42.32 &   41.83 &   42.54 &   42.62 &   42.98 &   35.08 \nl
 I1727   \tablenotemark{b}&$<$ 39.15 &   42.13 &  &$<$ 41.44 &$<$ 40.99 &   40.84 &   41.12 &   41.40 &  \nl
 N0672  &$<$ 39.20 &   42.50 &  &$<$ 41.47 &   41.19 &   41.81 &   41.80 &   42.21 &$<$ 34.25 \nl
 N0772   \tablenotemark{b}&$<$ 40.89 &   43.72 &   44.20 &   42.78 &   42.59 &   43.22 &   43.45 &   43.75 &   36.24 \nl
 N0871  &$<$ 40.91 &   43.12 &  &$<$ 43.11 &   42.76 &   43.51 &   43.39 &   43.86 &   36.83 \nl
 N0877  &   40.93 &   43.59 &   43.97 &   43.32 &   43.04 &   43.92 &   43.94 &   44.33 &   36.85 \nl
 N0936  &   40.29 &   43.08 &   43.81 &$<$ 41.70 &$<$ 41.53 &$<$ 41.18 &$<$ 41.08 &$<$ 41.54 &   34.92 \nl
 N0941  &$<$ 40.97 &   42.56 &  &$<$ 42.40 &$<$ 41.95 &   42.13 &   42.20 &   42.57 &  \nl
 N0945  &$<$ 40.85 &   43.43 &  &$<$ 43.25 &$<$ 42.79 &   43.03 &   43.23 &   43.54 &  \nl
 N0985  \tablenotemark{a}&   43.86 &   43.83 &  &$<$ 44.19 &   44.05 &   44.13 &   43.86 &   44.41 &  \nl
 N1042  &   40.41 &   42.93 &  &$<$ 42.25 &$<$ 41.81 &   42.13 &   42.46 &   42.73 &  \nl
 N1068  \tablenotemark{a} &   41.83 &   43.55 &   44.35 &   44.30 &   44.20 &   44.19 &   43.90 &   44.47 &   37.55 \nl
 N1073  &   40.15 &   42.85 &  &$<$ 42.17 &$<$ 41.72 &   42.04 &   42.35 &   42.63 &   36.31 \nl
 N1087  &$<$ 40.60 &   43.18 &  &   42.72 &   42.41 &   43.12 &   43.21 &   43.57 &   36.10 \nl
 N1090  &$<$ 40.87 &   43.33 &   43.60 &$<$ 42.84 &$<$ 42.51 &   42.59 &   42.82 &   43.12 &  \nl
 N1097  &   41.00 &   43.37 &   44.11 &   43.18 &   43.15 &   43.60 &   43.58 &   43.99 &   36.33 \nl
 N1218  \tablenotemark{a}&   42.62 &   43.77 &   44.42 &$<$ 43.32 &   43.00 &$<$ 42.48 &   42.84 &$<$ 43.10 &$<$ 39.39 \nl
 N1300  &   39.93 &   43.23 &   43.46 &$<$ 42.32 &$<$ 41.94 &   42.51 &   42.76 &   43.06 &  \nl
 N1313  &   39.66 &   42.50 &  &   41.57 &   41.68 &   42.35 &   42.35 &   42.75 &   34.86 \nl
 N1317  &$<$ 40.03 &   42.71 &  &   42.26 &   41.79 &   42.59 &   42.59 &   42.99 &  \nl
 N1350  &$<$ 40.29 &   43.09 &   43.64 &$<$ 42.21 &$<$ 41.76 &$<$ 41.78 &   42.21 &$<$ 42.44 &  \nl
 N1358   \tablenotemark{b}&   40.69 &   43.29 &   43.93 &$<$ 42.67 &$<$ 42.39 &   42.53 &   42.51 &   42.92 &   35.32 \nl
 N1365  &   40.84 &   43.46 &   44.12 &   43.46 &   43.48 &   43.95 &   43.88 &   44.31 &   36.63 \nl
 N1380  &   40.31 &   42.93 &   43.74 &   41.91 &   41.07 &   41.92 &   41.96 &   42.34 &   34.45 \nl
 N1386  &   40.38 &   42.59 &   43.39 &   42.54 &   42.54 &   42.77 &   42.56 &   43.08 &   35.78 \nl
 N1398  &   40.15 &   43.26 &   44.00 &$<$ 42.19 &$<$ 41.74 &   41.97 &   42.48 &   42.70 &  \nl
 N1421  &   40.77 &   43.39 &   43.47 &   42.74 &   42.32 &   43.25 &   43.31 &   43.68 &  \nl
 I0342  &   39.88 &   43.60 &   44.47 &   42.77 &   42.60 &   43.01 &   43.01 &   43.41 &   34.79 \nl
 N1512  &$<$ 39.67 &   42.54 &   43.20 &$<$ 41.90 &$<$ 41.24 &   41.46 &   41.15 &   41.73 &$<$ 34.90 \nl
 N1533  &   39.90 &   42.59 &  &$<$ 41.63 &   40.99 &   41.39 &   41.55 &   41.88 &$<$ 35.58 \nl
 N1559  &   40.48 &   42.99 &   43.21 &   42.64 &   42.46 &   43.28 &   43.25 &   43.67 &   36.27 \nl
 N1566  \tablenotemark{a}&   41.38 &   43.22 &   43.75 &   42.39 &   42.16 &   42.98 &   43.09 &   43.44 &   36.04 \nl
 N1569  &   38.83 &   41.60 &   42.23 &   40.57 &   41.13 &   41.62 &   41.25 &   41.88 &   34.68 \nl
 N1614  &   41.50 &   43.20 &   43.81 &   44.03 &   44.31 &   44.62 &   44.19 &   44.86 &  \nl
 N1625  &$<$ 41.11 &   43.67 &  &$<$ 43.27 &$<$ 42.82 &   43.11 &   43.25 &   43.59 &  \nl
 N1672  &   40.33 &   43.17 &   43.66 &   42.82 &   42.80 &   43.40 &   43.29 &   43.75 &   36.15 \nl
 N1784  &$<$ 40.45 &   43.21 &   43.66 &$<$ 42.64 &$<$ 42.33 &   42.84 &   43.00 &   43.33 &  \nl
   LMC  &   38.41 &   42.07 &  &   41.12 &   41.12 &   41.81 &   41.74 &   42.18 &  \nl
 N1961   \tablenotemark{b}&   41.28 &   44.26 &   44.75 &   43.74 &   43.26 &   44.07 &   44.18 &   44.53 &   37.34 \nl
 U3691  &$<$ 40.54 &   43.25 &   42.73 &$<$ 42.60 &$<$ 42.15 &   42.55 &   42.58 &   42.96 &  \nl
 N2276  &$<$ 40.38 &   42.67 &  &   42.51 &   42.35 &   43.03 &   43.01 &   43.42 &   36.26 \nl
 N2366  &$<$ 38.52 &   41.59 &   41.15 &$<$ 40.74 &   40.75 &   41.07 &   40.80 &   41.36 &   34.14 \nl
 N2403  &   39.37 &   42.54 &   42.86 &   41.82 &   41.64 &   42.21 &   42.26 &   42.64 &   34.51 \nl
 N2441  &$<$ 41.11 &   43.38 &  &$<$ 43.18 &$<$ 42.73 &   42.91 &   43.14 &   43.44 &$<$ 36.04 \nl
 N2525  &$<$ 40.07 &   42.82 &  &$<$ 42.22 &   42.12 &   42.81 &   42.84 &   43.23 &  \nl
 N2608  &   40.04 &   42.79 &  &$<$ 42.58 &   42.13 &   42.75 &   42.76 &   43.16 &   36.11 \nl
 N2642  &$<$ 41.11 &   43.19 &  &$<$ 43.17 &$<$ 42.73 &   42.89 &   43.07 &   43.39 &  \nl
 N2683   \tablenotemark{b}&$<$ 39.46 &   42.52 &   43.11 &   41.71 &   41.01 &   41.88 &   42.08 &   42.39 &   34.54 \nl
 N2763  &$<$ 40.13 &   42.66 &  &$<$ 42.44 &$<$ 41.94 &   42.50 &   42.55 &   42.93 &  \nl
 N2773  &   41.19 &   42.89 &  &$<$ 43.41 &   43.11 &   43.64 &   43.49 &   43.97 &  \nl
 N2775  &   40.17 &   43.05 &   43.66 &$<$ 42.15 &$<$ 41.74 &   42.20 &   42.57 &   42.82 &$<$ 35.24 \nl
 N2777  &$<$ 39.76 &   41.82 &  &$<$ 42.15 &$<$ 41.80 &   41.83 &   41.66 &   42.15 &$<$ 35.24 \nl
 N2782  &$<$ 40.89 &   43.18 &   43.58 &   43.06 &   43.07 &   43.49 &   43.29 &   43.81 &   36.59 \nl
 N2835  &   39.25 &   42.64 &   42.62 &$<$ 41.54 &$<$ 41.09 &   41.76 &   42.10 &   42.36 &  \nl
 N2848  &$<$ 40.16 &   42.89 &  &$<$ 42.44 &$<$ 41.99 &   42.33 &   42.54 &   42.85 &  \nl
 N2841   \tablenotemark{b}&   40.54 &   43.87 &   44.42 &   43.03 &   42.54 &   42.93 &   43.26 &   43.52 &   35.72 \nl
 N2903  &   39.85 &   42.87 &   43.33 &   42.59 &   42.32 &   42.82 &   42.86 &   43.24 &   35.56 \nl
 N2914  &$<$ 40.89 &   42.63 &  &$<$ 42.41 &$<$ 42.07 &   42.16 &   42.04 &   42.50 &$<$ 36.54 \nl
 N2992  \tablenotemark{a}&   42.30 &   42.95 &   43.64 &   42.96 &   42.87 &   43.23 &   43.15 &   43.59 &   35.61 \nl
 N2993  &$<$ 40.99 &   42.75 &   42.87 &   42.86 &   42.94 &   43.41 &   43.18 &   43.71 &  \nl
 N3031   \tablenotemark{b}&   40.16 &   43.06 &   43.77 &   42.16 &   41.68 &   42.25 &   42.43 &   42.75 &   34.96 \nl
 N3034  &   40.56 &   42.49 &   43.57 &   43.22 &   43.40 &   43.71 &   43.32 &   43.96 &   36.50 \nl
 N3067  &$<$ 40.34 &   42.59 &  &   42.68 &   42.41 &   43.02 &   42.93 &   43.38 &$<$ 36.75 \nl
 N3081  &   40.88 &   42.76 &   43.29 &  &  &  &  &  &   34.63 \nl
 N3066  &$<$ 40.93 &   42.54 &   42.70 &$<$ 42.78 &   42.50 &   42.91 &   42.78 &   43.25 &  \nl
 N3079   \tablenotemark{b}&$<$ 40.71 &   43.32 &   43.85 &   42.95 &   42.71 &   43.70 &   43.60 &   44.06 &   36.87 \nl
 N3077  &$<$ 38.68 &   41.85 &   42.16 &   41.11 &   41.22 &   41.77 &   41.59 &   42.09 &$<$ 34.27 \nl
 N3125  &$<$ 39.96 &   41.71 &   41.84 &$<$ 41.73 &$<$ 41.78 &   42.24 &   41.94 &   42.52 &  \nl
 N3166   \tablenotemark{b}&   39.45 &   42.39 &  &   41.66 &   41.34 &   42.15 &   42.10 &   42.53 &$<$ 34.67 \nl
 N3169   \tablenotemark{b}&$<$ 39.58 &   42.41 &  &   41.91 &   41.50 &   42.21 &   42.27 &   42.64 &   35.03 \nl
 N3175  &$<$ 39.96 &   42.50 &  &   42.21 &   42.00 &   42.67 &   42.67 &   43.07 &  \nl
 N3184  &$<$ 40.47 &   42.48 &  &$<$ 41.39 &$<$ 41.28 &   41.58 &   41.98 &   42.23 &   34.61 \nl
 N3227  \tablenotemark{a} &   41.53 &   42.74 &   43.31 &   42.41 &   42.37 &   42.70 &   42.63 &   43.06 &   35.61 \nl
 I2574  &   38.35 &   41.89 &   41.45 &$<$ 40.10 &   39.85 &   40.99 &   41.22 &   41.52 &  \nl
 N3281  &$<$ 41.18 &   43.38 &   43.87 &   43.47 &   43.48 &   43.57 &   43.21 &   43.82 &   36.45 \nl
 N3310  &   40.42 &   42.83 &   42.99 &   42.68 &   42.80 &   43.32 &   43.00 &   43.59 &   36.25 \nl
 N3346  &$<$ 39.74 &   42.37 &  &$<$ 42.04 &$<$ 41.75 &   41.98 &   42.18 &   42.50 &  \nl
 N3351  &$<$ 39.98 &   42.81 &   43.42 &   42.05 &   42.12 &   42.74 &   42.64 &   43.09 &   35.40 \nl
 N3353  &   39.60 &   41.99 &   42.13 &$<$ 41.97 &   42.08 &   42.49 &   42.19 &   42.77 &  \nl
 N3368   \tablenotemark{b}&$<$ 39.93 &   43.09 &   43.75 &   41.96 &$<$ 41.68 &   42.56 &   42.62 &   42.99 &$<$ 35.26 \nl
 N3389  &$<$ 40.86 &   43.12 &  &  &  &  &  &  &  \nl
 N3395  &   40.30 &   42.72 &   42.45 &$<$ 42.33 &   42.19 &   43.06 &   42.96 &   43.41 &   36.04 \nl
 N3430  &$<$ 40.17 &   42.85 &   43.17 &$<$ 42.47 &$<$ 41.86 &   42.58 &   42.64 &   43.01 &  \nl
 N3445  &$<$ 40.51 &   42.67 &  &$<$ 42.58 &$<$ 42.15 &   42.74 &   42.63 &   43.09 &  \nl
 N3448  &   40.23 &   42.74 &  &   42.39 &   42.16 &   42.81 &   42.69 &   43.16 &   35.94 \nl
 N3455  &$<$ 39.75 &   42.15 &  &$<$ 42.01 &$<$ 41.67 &   41.75 &  &   41.85 &  \nl
 N3489   \tablenotemark{b}&$<$ 39.87 &   42.57 &  &  &  &  &  &  &   34.08 \nl
 N3504  &   40.28 &   42.84 &   43.50 &   42.89 &   42.99 &   43.37 &   43.19 &   43.69 &   36.43 \nl
 N3512  &$<$ 40.14 &   42.25 &  &$<$ 42.17 &$<$ 41.93 &   42.12 &   42.18 &   42.56 &  \nl
 N3593  &   39.09 &   41.96 &  &   42.04 &   41.79 &   42.41 &   42.27 &   42.74 &   35.24 \nl
 N3628   \tablenotemark{b}&   40.45 &   43.33 &   43.79 &   42.92 &   42.70 &   43.33 &   43.32 &   43.72 &   36.28 \nl
 N3690  &   41.03 &   43.44 &   43.90 &   44.12 &   44.43 &   44.79 &   44.40 &   45.03 &   37.59 \nl
 N3718   \tablenotemark{b}&$<$ 40.33 &   42.74 &   43.62 &   41.77 &   41.18 &   41.68 &   41.79 &   42.14 &$<$ 36.04 \nl
 N3729  &$<$ 40.01 &   42.52 &  &$<$ 42.12 &   41.78 &   42.30 &   42.35 &   42.73 &  \nl
 N3783  \tablenotemark{a}&   42.79 &   43.18 &   43.66 &   43.26 &   43.31 &   43.11 &   42.88 &   43.41 &   35.98 \nl
 N3884   \tablenotemark{b}&   42.07 &   43.52 &   44.08 &  &  &  &  &  &  \nl
 N3887  &$<$ 39.67 &   42.64 &  &$<$ 41.96 &$<$ 41.67 &   42.36 &   42.50 &   42.83 &  \nl
 N3888  &$<$ 40.38 &   42.93 &   43.35 &   42.83 &   42.55 &   43.22 &   43.18 &   43.60 &$<$ 36.30 \nl
 N3893  &$<$ 39.93 &   43.01 &   43.25 &   42.58 &   42.26 &   43.01 &   43.00 &   43.41 &   35.81 \nl
 N3896  &$<$ 39.76 &   41.79 &  &  &  &  &  &  &$<$ 35.54 \nl
 N3991  &   41.01 &   42.83 &   42.70 &$<$ 42.93 &$<$ 42.54 &   43.15 &   43.01 &   43.49 &   36.58 \nl
 N3994  &$<$ 40.86 &   42.88 &  &$<$ 42.96 &$<$ 42.79 &   43.18 &   43.35 &   43.67 &   36.42 \nl
 N3995  &$<$ 40.85 &   43.23 &  &  &  &  &  &  &   36.64 \nl
 I0749  &$<$ 39.72 &   42.16 &  &  &  &  &  &  &$<$ 35.59 \nl
 I0750  &$<$ 39.73 &   42.33 &  &  &  &  &  &  &   35.96 \nl
 N4036   \tablenotemark{b}&$<$ 40.31 &   42.92 &   43.73 &   41.94 &$<$ 41.32 &   41.87 &   41.86 &   42.26 &   34.87 \nl
 N4038  &   40.96 &   43.39 &  &   43.10 &   43.16 &   43.82 &   43.69 &   44.16 &   36.84 \nl
 N4041  &$<$ 40.36 &   42.72 &  &   42.72 &   42.50 &   43.15 &   43.10 &   43.53 &   35.88 \nl
 N4051  \tablenotemark{a} &   41.80 &   42.99 &   43.06 &   42.55 &   42.36 &   42.79 &   42.78 &   43.19 &   35.81 \nl
 N4151  \tablenotemark{a} &   41.33 &   42.88 &   43.51 &  &  &  &  &  &   36.24 \nl
 N4156  &   41.72 &   43.30 &  &  &  &  &  &  &  \nl
 N4178  &$<$ 39.73 &   42.57 &   42.59 &$<$ 42.14 &   41.75 &   42.32 &   42.28 &   42.70 &  \nl
 N4190  &   38.94 &   40.65 &  &$<$ 40.45 &$<$ 40.01 &   40.18 &   40.34 &   40.67 &   33.57 \nl
 N4192   \tablenotemark{b}&   39.53 &   43.22 &   43.64 &   42.42 &   41.71 &   42.67 &   42.77 &   43.12 &   35.62 \nl
 N4206  &$<$ 39.98 &   42.80 &   42.97 &$<$ 42.35 &$<$ 42.04 &   42.14 &   42.06 &   42.51 &  \nl
 N4212  &   39.90 &   42.91 &  &   42.71 &   42.44 &   42.91 &   42.85 &   43.28 &  \nl
 N4214  &$<$ 39.91 &   42.07 &   42.14 &   41.10 &   41.30 &   41.88 &   41.71 &   42.20 &   34.67 \nl
 N4216   \tablenotemark{b}&   39.59 &   43.38 &   43.96 &$<$ 41.81 &$<$ 41.58 &   42.30 &   42.64 &   42.90 &  \nl
 N4224  &$<$ 40.99 &   43.22 &  &$<$ 42.90 &$<$ 42.40 &   42.04 &   42.33 &   42.61 &  \nl
 N4236  &   38.20 &   42.21 &   41.98 &   40.44 &   40.70 &   41.20 &   41.19 &   41.60 &  \nl
 N4235  \tablenotemark{a} &   41.28 &   42.74 &   43.18 &$<$ 41.92 &$<$ 41.74 &   41.59 &   41.48 &   41.94 &   35.10 \nl
 N4244  &   38.73 &   42.50 &   42.26 &$<$ 40.30 &$<$ 39.98 &   41.42 &   41.59 &   41.92 &  \nl
 N4245  &$<$ 39.66 &   42.21 &  &$<$ 41.44 &$<$ 41.02 &   41.51 &   41.62 &   41.97 &  \nl
 N4246  &$<$ 40.76 &   42.87 &   42.96 &  &  &  &  &  &  \nl
 N4254  &   39.96 &   43.09 &  &   43.11 &   42.71 &   43.36 &   43.28 &   43.72 &   36.13 \nl
 N4258   \tablenotemark{b}&   40.45 &   43.21 &   43.66 &   42.35 &   41.99 &   42.54 &   42.69 &   43.02 &   35.88 \nl
 N4260  &$<$ 41.10 &   43.24 &  &$<$ 43.23 &$<$ 42.45 &   42.05 &   42.31 &   42.60 &  \nl
 N4298  &   39.84 &   42.67 &  &   42.48 &   42.19 &   42.44 &   42.55 &   42.90 &  \nl
 N4303  &   40.10 &   42.91 &   43.25 &   42.89 &   42.58 &   43.15 &   43.02 &   43.49 &   35.91 \nl
 N4321   \tablenotemark{b}&   40.42 &   43.33 &   43.62 &   43.15 &   42.78 &   43.40 &   43.34 &   43.77 &   36.11 \nl
 N4351  &$<$ 39.89 &   42.01 &  &$<$ 41.50 &$<$ 41.31 &   41.58 &   41.61 &   42.00 &  \nl
 N4378   \tablenotemark{b}&   40.98 &   43.40 &  &$<$ 42.96 &$<$ 42.66 &$<$ 42.83 &   42.63 &$<$ 43.14 &  \nl
 N4385  &$<$ 40.79 &   42.58 &   43.01 &   42.55 &   42.73 &   42.99 &   42.69 &   43.26 &  \nl
 N4388   \tablenotemark{b}&   40.34 &   43.03 &   43.38 &   42.78 &   42.82 &   43.00 &   42.78 &   43.30 &   36.21 \nl
 N4394   \tablenotemark{b}&$<$ 40.01 &   43.07 &   43.62 &   42.50 &   42.03 &   42.32 &   42.55 &   42.85 &  \nl
 N4424  &   37.93 &   41.33 &  &   40.74 &   40.60 &   41.17 &   41.02 &   41.51 &  \nl
 N4429   \tablenotemark{b}&   39.81 &   42.74 &   43.56 &   41.81 &$<$ 41.14 &   41.92 &   41.97 &   42.35 &$<$ 34.93 \nl
 N4438   \tablenotemark{b}&   40.03 &   42.89 &   43.43 &   41.69 &$<$ 41.19 &   42.30 &   42.34 &   42.72 &   35.84 \nl
 N4449  &   39.11 &   41.85 &   42.02 &  &  &  &  &  &   34.84 \nl
 N4450   \tablenotemark{b}&   40.44 &   42.91 &   43.45 &   41.76 &$<$ 41.57 &   42.05 &   42.28 &   42.58 &  \nl
 N4461  &$<$ 39.77 &   42.28 &  &   41.55 &$<$ 40.99 &$<$ 40.35 &$<$ 40.59 &$<$ 40.89 &$<$ 34.84 \nl
 N4464  &$<$ 40.26 &   42.08 &   42.75 &$<$ 41.93 &$<$ 41.51 &$<$ 40.99 &   41.10 &$<$ 41.45 &  \nl
 N4477   \tablenotemark{b}&   40.36 &   42.81 &   43.54 &   41.92 &$<$ 41.38 &   41.69 &   41.61 &   42.05 &$<$ 33.64 \nl
 N4501   \tablenotemark{b}&   40.44 &   43.44 &   43.98 &   43.13 &   42.79 &   43.29 &   43.33 &   43.72 &   36.13 \nl
 N4503  &$<$ 39.33 &   42.22 &  &$<$ 41.29 &$<$ 40.89 &$<$ 40.71 &$<$ 40.92 &$<$ 41.23 &$<$ 34.79 \nl
 N4522  &$<$ 40.29 &   42.53 &   42.61 &$<$ 42.03 &   41.62 &   42.15 &   42.10 &   42.53 &  \nl
 N4527   \tablenotemark{b}&$<$ 40.09 &   42.91 &  &   42.56 &   42.37 &   43.18 &   43.16 &   43.57 &   36.23 \nl
 N4535  &$<$ 39.71 &   42.96 &   43.08 &   42.54 &   42.20 &   42.82 &   42.77 &   43.20 &   35.54 \nl
 N4536  &   40.29 &   43.11 &   43.53 &   42.87 &   42.81 &   43.41 &   43.17 &   43.71 &   36.15 \nl
 I3528  \tablenotemark{a}&   43.02 &   43.38 &  &$<$ 44.26 &$<$ 44.01 &   44.14 &   44.36 &   44.67 &  \nl
 N4548   \tablenotemark{b}&$<$ 40.09 &   42.91 &  &   42.20 &   41.58 &   42.26 &   42.44 &   42.76 &  \nl
 N4565   \tablenotemark{b}&   40.02 &   43.32 &   43.89 &   42.52 &   42.11 &   42.53 &   42.80 &   43.09 &   35.48 \nl
 N4567  &   40.45 &   42.89 &   42.90 &   42.74 &   42.52 &   43.38 &   43.45 &   43.82 &   36.14 \nl
 N4569   \tablenotemark{b}&   39.77 &   42.90 &   43.31 &   42.06 &   41.85 &   42.36 &   42.42 &   42.80 &   35.30 \nl
 N4571  &$<$ 39.96 &   42.56 &  &$<$ 42.03 &$<$ 41.57 &   41.81 &   42.24 &   42.48 &  \nl
 N4579   \tablenotemark{b}&   41.58 &   43.39 &   44.02 &   42.86 &   42.29 &   42.92 &   42.96 &   43.34 &   36.14 \nl
 N4594   \tablenotemark{b}&   40.49 &   43.50 &   44.06 &   42.10 &   41.47 &   42.07 &   42.38 &   42.66 &   35.95 \nl
 N4603  &   40.39 &   43.26 &   43.59 &$<$ 42.64 &$<$ 42.19 &   42.80 &   43.10 &   43.38 &  \nl
 N4631  &   39.31 &   42.55 &   42.95 &   42.11 &   41.90 &   42.50 &   42.49 &   42.89 &   35.09 \nl
 N4639   \tablenotemark{b}&   40.99 &   42.96 &  &$<$ 42.56 &$<$ 42.06 &   42.56 &   42.53 &   42.94 &  \nl
 N4643   \tablenotemark{b}&   39.86 &   42.70 &   43.50 &$<$ 41.59 &$<$ 41.40 &   41.71 &   41.75 &   42.13 &$<$ 33.94 \nl
 N4647  &$<$ 40.55 &   42.77 &   42.76 &   42.86 &   42.38 &   42.87 &   42.86 &   43.27 &$<$ 35.33 \nl
 N4651   \tablenotemark{b}&$<$ 40.25 &   43.12 &   43.55 &   42.71 &   42.32 &   42.92 &   42.86 &   43.29 &  \nl
 N4654  &$<$ 39.81 &   42.83 &   43.08 &   42.61 &   42.30 &   42.89 &   42.84 &   43.27 &   35.69 \nl
 N4665  &$<$ 39.98 &   42.77 &  &$<$ 41.49 &$<$ 41.40 &$<$ 40.81 &$<$ 40.61 &$<$ 41.12 &$<$ 33.70 \nl
 N4689  &   40.32 &   42.65 &  &   42.26 &   41.70 &   42.38 &   42.36 &   42.77 &  \nl
 N4698   \tablenotemark{b}&   40.58 &   43.53 &   44.11 &   42.85 &$<$ 42.61 &   42.41 &   42.48 &   42.85 &  \nl
 N4736   \tablenotemark{b}&   39.93 &   42.95 &   43.81 &   42.50 &   42.21 &   42.83 &   42.75 &   43.19 &   35.27 \nl
 N4826   \tablenotemark{b}&   39.30 &   42.70 &   43.26 &   41.84 &   41.46 &   42.35 &   42.29 &   42.72 &   34.87 \nl
 N4845  &$<$ 40.45 &   43.31 &  &   42.89 &   42.63 &   43.43 &   43.42 &   43.83 &  \nl
 N4861  &   40.06 &   42.15 &   42.26 &$<$ 41.79 &   41.53 &   41.87 &   41.57 &   42.15 &$<$ 35.37 \nl
 I4182  &$<$ 39.74 &   41.56 &  &$<$ 40.59 &$<$ 40.05 &   40.59 &   40.65 &   41.02 &  \nl
 N5033   \tablenotemark{b}&   41.13 &   42.98 &   43.55 &   42.58 &   42.24 &   42.88 &   42.95 &   43.32 &   35.67 \nl
 N5037  &$<$ 40.52 &   42.49 &  &$<$ 42.29 &$<$ 41.89 &   41.95 &   42.15 &   42.46 &  \nl
 N5068  &$<$ 39.42 &   42.41 &  &$<$ 41.30 &$<$ 41.35 &   41.40 &   41.85 &   42.09 &  \nl
 N5088  &$<$ 39.85 &   42.40 &  &$<$ 42.11 &$<$ 41.92 &   42.17 &   42.12 &   42.55 &  \nl
 N5101  &$<$ 40.51 &   43.09 &  &   41.99 &   41.54 &   42.05 &   42.49 &   42.73 &  \nl
 N5135  &   41.03 &   43.38 &   43.94 &   43.53 &   43.65 &   44.12 &   43.99 &   44.46 &   36.97 \nl
 N5204  &   39.78 &   42.03 &   41.98 &$<$ 41.39 &$<$ 41.01 &   41.58 &   41.52 &   41.95 &  \nl
 N5194   \tablenotemark{b}&   40.46 &   43.29 &   43.57 &   43.17 &   42.92 &   43.38 &   43.39 &   43.79 &   36.18 \nl
 N5236  &   40.09 &   43.02 &   43.34 &   43.01 &   42.81 &   43.22 &   43.19 &   43.61 &   35.77 \nl
 N5248  &   39.87 &   42.95 &   43.47 &   42.56 &   42.29 &   43.03 &   43.01 &   43.42 &   35.96 \nl
 N5253  &   38.66 &   41.96 &   42.06 &   41.94 &   42.16 &   42.23 &   41.76 &   42.46 &   34.84 \nl
I4329A  \tablenotemark{a}&   43.34 &   43.00 &   43.96 &   43.87 &   43.75 &   43.37 &   42.86 &   43.58 &  \nl
 N5313  &$<$ 40.48 &   42.98 &  &$<$ 42.89 &   42.30 &   43.06 &   43.18 &   43.52 &  \nl
 N5326  &$<$ 40.45 &   42.94 &  &  &  &  &  &  &$<$ 36.14 \nl
 N5350  &$<$ 40.59 &   43.11 &  &$<$ 43.08 &   42.36 &   42.84 &   43.01 &   43.33 &  \nl
 N5364  &$<$ 40.32 &   42.95 &  &$<$ 42.04 &$<$ 42.09 &   42.16 &   42.49 &   42.76 &  \nl
 N5410  &$<$ 41.05 &   42.90 &   42.87 &$<$ 43.12 &$<$ 42.64 &   42.80 &   42.77 &   43.18 &  \nl
 N5457  &   40.08 &   43.34 &   43.50 &   42.79 &   42.62 &   43.15 &   43.20 &   43.58 &   35.67 \nl
 N5474  &$<$ 39.03 &   42.10 &   41.64 &$<$ 41.39 &$<$ 40.94 &   41.25 &   41.47 &   41.78 &$<$ 33.97 \nl
 N5477  &$<$ 39.12 &   40.94 &  &$<$ 40.70 &$<$ 40.47 &   40.66 &   40.50 &   40.99 &$<$ 33.97 \nl
 N5506  \tablenotemark{a}&   41.83 &   42.70 &   43.37 &   43.10 &   43.14 &   43.14 &   42.70 &   43.37 &   36.60 \nl
 N5548  \tablenotemark{a} &   43.31 &   43.45 &   43.92 &   43.51 &   43.38 &   43.18 &   42.99 &   43.50 &   36.35 \nl
 N5566   \tablenotemark{b}&   40.09 &   43.14 &   43.85 &$<$ 42.23 &$<$ 41.82 &   42.07 &   42.38 &   42.65 &  \nl
 N5585  &$<$ 39.29 &   42.20 &   42.06 &$<$ 41.39 &$<$ 40.94 &   41.13 &   41.37 &   41.67 &   34.19 \nl
 N5645  &$<$ 40.19 &   42.40 &  &$<$ 42.28 &$<$ 41.70 &   42.27 &   42.22 &   42.65 &  \nl
 N5643  &   40.31 &   43.02 &   43.23 &   42.42 &   42.56 &   42.97 &   42.93 &   43.35 &   35.79 \nl
 N5674  &   41.47 &   43.46 &  &$<$ 43.67 &$<$ 43.37 &   43.65 &   43.61 &   44.03 &  \nl
 N5683  \tablenotemark{a}&   43.10 &   43.23 &   43.85 &$<$ 44.00 &$<$ 43.55 &   43.48 &   43.53 &   43.91 &  \nl
 N5689  &$<$ 40.59 &   43.06 &  &$<$ 42.64 &$<$ 42.19 &   42.10 &   42.19 &   42.55 &$<$ 36.74 \nl
 N5728  &   40.90 &   43.33 &   43.83 &$<$ 42.87 &   42.82 &   43.50 &   43.35 &   43.83 &   35.53 \nl
 N5850   \tablenotemark{b}&   40.08 &   43.39 &  &$<$ 42.72 &$<$ 42.26 &   42.39 &   42.76 &   43.02 &  \nl
 N5879   \tablenotemark{b}&$<$ 39.86 &   42.54 &   42.87 &   41.92 &   41.41 &   42.20 &   42.23 &   42.62 &  \nl
 N5907  &$<$ 39.70 &   43.17 &   43.53 &   42.51 &   42.10 &   42.58 &   42.88 &   43.16 &   35.40 \nl
 N5985   \tablenotemark{b}&$<$ 41.12 &   43.47 &  &$<$ 42.79 &$<$ 42.34 &   42.59 &   42.98 &   43.23 &  \nl
 N6052  &$<$ 41.70 &   43.15 &   43.33 &   43.27 &   43.37 &   43.94 &   43.69 &   44.24 &   37.06 \nl
 N6300  &$<$ 39.95 &   42.98 &  &   42.31 &   42.32 &   42.80 &   42.84 &   43.22 &   35.56 \nl
 N6454  \tablenotemark{a}&   42.31 &   43.48 &   44.22 &$<$ 43.23 &$<$ 42.50 &$<$ 42.63 &$<$ 42.55 &$<$ 42.99 &   38.74 \nl
 N6503   \tablenotemark{b}&$<$ 39.25 &   42.29 &   42.70 &   41.49 &   40.91 &   41.78 &   41.92 &   42.25 &   34.53 \nl
 N6744  &   39.83 &   43.28 &   43.47 &   42.64 &   42.35 &   42.74 &   42.91 &   43.23 &  \nl
 N6814  \tablenotemark{a}&   41.20 &   43.06 &   43.55 &   42.48 &   42.28 &   42.93 &   43.02 &   43.38 &   34.80 \nl
 N6822  &   37.41 &   40.95 &  &   39.08 &   39.62 &   40.57 &   40.46 &   40.92 &   33.03 \nl
 N6872  &   41.60 &   43.89 &  &$<$ 43.60 &$<$ 42.81 &   43.27 &   43.54 &   43.82 &   36.94 \nl
 N6890  &$<$ 40.69 &   42.79 &   43.42 &   42.91 &   42.72 &   43.07 &   43.04 &   43.46 &   35.41 \nl
 N6946  &   40.07 &   43.27 &   43.47 &   42.85 &   42.64 &   43.11 &   43.10 &   43.50 &   35.37 \nl
 N6951   \tablenotemark{b}&$<$ 40.56 &   43.34 &   43.84 &   42.65 &   42.61 &   43.34 &   43.36 &   43.75 &   36.05 \nl
 N6962  &$<$ 41.09 &   43.46 &  &$<$ 43.21 &$<$ 42.76 &$<$ 42.62 &   42.92 &$<$ 43.20 &  \nl
 I5063  &$<$ 41.30 &   43.15 &   43.81 &   43.64 &   43.71 &   43.58 &   42.95 &   43.77 &   37.69 \nl
 N7213  \tablenotemark{a}&   42.78 &   43.18 &   43.91 &   42.73 &   42.48 &   42.63 &   42.72 &   43.08 &   36.87 \nl
 N7314  &$<$ 40.70 &   43.06 &   43.30 &$<$ 42.31 &   42.24 &   42.61 &   42.85 &   43.15 &  \nl
 N7320  &   40.37 &   42.24 &   42.26 &$<$ 42.04 &$<$ 41.65 &   41.65 &   41.92 &   42.21 &  \nl
 N7331   \tablenotemark{b}&   40.38 &   43.51 &   44.26 &   43.17 &   42.81 &   43.40 &   43.50 &   43.85 &   36.11 \nl
 N7339  &$<$ 40.37 &   42.53 &  &  &  &  &  &  &  \nl
 N7469  \tablenotemark{a}&   42.61 &   42.79 &   43.35 &   43.33 &   43.51 &   43.86 &   43.57 &   44.14 &   36.61 \nl
 I5283  &$<$ 40.37 &   42.11 &   42.74 &  &  &  &  &  &$<$ 36.24 \nl
 N7496  &$<$ 40.38 &   42.82 &   43.09 &   42.36 &   42.66 &   43.07 &   42.91 &   43.40 &  \nl
 N7552  &   40.67 &   43.10 &   43.67 &   43.40 &   43.56 &   44.00 &   43.73 &   44.29 &   36.57 \nl
 N7582  \tablenotemark{a}&   40.77 &   43.22 &   43.73 &   43.06 &   43.28 &   43.82 &   43.59 &   44.12 &   36.47 \nl
 N7590  &   40.18 &   42.97 &   43.32 &   42.65 &   42.40 &   43.01 &   42.98 &   43.40 &  \nl
 N7599  &   40.04 &   43.07 &   43.23 &   42.65 &   42.27 &   42.93 &   42.99 &   43.36 &  \nl
 N7611  &$<$ 41.01 &   42.88 &   43.68 &$<$ 42.65 &$<$ 42.41 &$<$ 41.99 &$<$ 42.30 &$<$ 42.57 &$<$ 38.30 \nl
 N7673  &   40.90 &   43.14 &  &$<$ 43.06 &   42.91 &   43.59 &   43.30 &   43.87 &  \nl
 N7677  &$<$ 41.06 &   42.96 &  &   43.14 &   43.12 &   43.49 &   43.28 &   43.80 &  \nl
 N7679  &   41.81 &   43.45 &   44.02 &   43.68 &   43.57 &   44.09 &   43.81 &   44.37 &$<$ 37.26 \nl
 N7682  &$<$ 41.85 &   43.14 &  &  &  &  &  &  &   36.90 \nl
 N7714  &   40.73 &   43.06 &   43.39 &   43.18 &   43.48 &   43.74 &   43.33 &   43.99 &   36.32 \nl
 N7769  &$<$ 41.12 &   43.42 &   43.87 &$<$ 43.44 &   43.15 &   43.72 &   43.69 &   44.11 &$<$ 36.76 \nl
 N7771  \tablenotemark{a}&   41.50 &   43.47 &   44.09 &   43.68 &   43.63 &   44.31 &   44.23 &   44.68 &   37.02 \nl
 N7793  &   39.12 &   42.36 &   42.41 &   41.67 &   41.35 &   41.99 &   42.03 &   42.41 &  \nl


\tablenotetext{a} {Galaxies known as AGN,
and excluded from the statistical analysis.}
\tablenotetext{b} {Galaxies exhibiting evidence
for some kind of non-stellar ionizing continuum giving rise to
nuclear emission, but at a lower level than those flagged with 
``a'' (Ho et al. 1997). These galaxies were included in the statictical analysis.}

\enddata
\end{deluxetable}




==> table9.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{llrrr}
\tablenum{9}
\tablewidth{0pc}
\tablecaption{Six-variable Partial Ranks Plus Fixed Distance
$({\rm Total \ Sample} : N = 94)$
}
\tablehead{
\colhead{Test } & \colhead{Held } &
\colhead{Partial } &
\colhead{Test Stat.} & \colhead{Prob.}  \\
\colhead{Pair} & \colhead{Parameters} &
\colhead{Rank} &
\colhead{(T)} & \colhead{}  \\
}
\startdata



6cm, H &  B , X ,FIR, 12 & -0.089 & -0.840 & 0.211 \nl
6cm, H &  B , X ,FIR, 12, D  & -0.108 & -1.009 & 0.170 \nl 
& & & & \nl
6cm, B &  H , X ,FIR, 12 & -0.016 & -0.147 & $>$ 0.400 \nl
6cm, B &  H , X ,FIR, 12, D  & -0.012 & -0.114 & $>$ 0.400 \nl 
& & & & \nl
6cm, X &  H , B ,FIR, 12 & 0.301 & 2.964 & $<$ 0.005 \nl
6cm, X &  H , B ,FIR, 12, D  & 0.250 & 2.404 & 0.010 \nl 
& & & & \nl
6cm,FIR&  H , B , X , 12 & 0.411 & 4.233 & $<$ 0.005 \nl
6cm,FIR&  H , B , X , 12, D  & 0.359 & 3.589 & $<$ 0.005 \nl 
& & & & \nl
6cm, 12&  H , B , X ,FIR & 0.215 & 2.064 & 0.023 \nl
6cm, 12&  H , B , X ,FIR, D  & 0.241 & 2.318 & 0.013 \nl 
& & & & \nl
 H , B & 6cm, X ,FIR, 12 & 0.823 & 13.578 & $<$ 0.005 \nl
 H , B & 6cm, X ,FIR, 12, D  & 0.819 & 13.307 & $<$ 0.005 \nl 
& & & & \nl
 H , X & 6cm, B ,FIR, 12 & 0.247 & 2.392 & 0.010 \nl
 H , X & 6cm, B ,FIR, 12, D  & 0.210 & 2.005 & 0.025 \nl 
& & & & \nl
 H ,FIR& 6cm, B , X , 12 & -0.236 & -2.282 & 0.015 \nl
 H ,FIR& 6cm, B , X , 12, D  & -0.255 & -2.464 & 0.009 \nl 
& & & & \nl
 H , 12& 6cm, B , X ,FIR & 0.122 & 1.158 & 0.134 \nl
 H , 12& 6cm, B , X ,FIR, D  & 0.143 & 1.352 & 0.093 \nl 
& & & & \nl
 B , X & 6cm, H ,FIR, 12 & -0.012 & -0.115 & $>$ 0.400 \nl
 B , X & 6cm, H ,FIR, 12, D  & -0.007 & -0.068 & $>$ 0.400 \nl 
& & & & \nl
 B ,FIR& 6cm, H , X , 12 & 0.296 & 2.911 & $<$ 0.005 \nl
 B ,FIR& 6cm, H , X , 12, D  & 0.293 & 2.863 & $<$ 0.005 \nl 
& & & & \nl
 B , 12& 6cm, H , X ,FIR & 0.012 & 0.109 & $>$ 0.400 \nl
 B , 12& 6cm, H , X ,FIR, D  & 0.007 & 0.069 & $>$ 0.400 \nl 
& & & & \nl
 X ,FIR& 6cm, H , B , 12 & 0.032 & 0.296 & 0.384 \nl
 X ,FIR& 6cm, H , B , 12, D  & -0.021 & -0.197 & $>$ 0.400 \nl 
& & & & \nl
 X , 12& 6cm, H , B ,FIR & 0.014 & 0.130 & $>$ 0.400 \nl
 X , 12& 6cm, H , B ,FIR, D  & 0.060 & 0.563 & 0.289 \nl 
& & & & \nl
FIR, 12& 6cm, H , B , X  & 0.615 & 7.315 & $<$ 0.005 \nl
FIR, 12& 6cm, H , B , X , D  & 0.632 & 7.602 & $<$ 0.005 \nl 
& & & & \nl
\enddata
\end{deluxetable}

